Piecewise Deterministic Markov Processes and their invariant measures

Piecewise Deterministic Markov Processes (PDMPs) are studied in a general framework. First, different constructions are proven to be equivalent. Second, we introduce a coupling between two PDMPs following the same differential flow which implies quantitative bounds on the total variation between the marginal distributions of the two processes. Finally two results are established regarding the invariant measures of PDMPs. A practical condition to show that a probability measure is invariant for the associated PDMP semi-group is presented. In a second time, a bound on the invariant probability measures in $V$-norm of two PDMPs following the same differential flow is established. This last result is then applied to study the asymptotic bias of some non-exact PDMP MCMC methods.

==> constructions_D.tex <==
\section{Alternative constructions}
\label{sec:alternative-constructions}


Consider PDMP characteristics   $( \varphi,(\lambda_i,Q_i)_{i\in \iintLigne{1,\ell}})$, an initial distribution $\mu_0 \in \mcp(\msm)$ and the associated process $(X_t)_{t \geq 0}$ defined in \Cref{sec:framework}. The goal of this Section is to construct another process $(Y_t)_{t \geq 0}$  on the same probability space $(\Omega,\mcf,\mathbb{P})$ with the same distribution on $\mrd(\rset_+,\msm \cup \{\infty\})$  as $(X_t)_{t \geq 0}$. \tcr{This alternative construction will turn out to be interesting to obtain a characterization of the distribution of the first jump time of type $i \in \{1,\ldots,\ell\}$; see \Cref{prop:premier_bounce} below. Simply put, the differences between the two constructions are the following: in Construction~\ref{const:1}, the exponential clocks $(E_{j,k})_{j\in \iintLigne{1,\ell}}$ are only used after the $(k-1)^{th}$ jump to define the time of the $k^{th}$ one, and they are all discarded afterwards. In contrast, in Construction~\ref{const:2}, only the exponential clock that has lead to the $k^{th}$ jump (i.e. with index $j\in \iintLigne{1,\ell}$ such that $S_k=S_{j,k}$) is refreshed to a new value, the others are kept in the next step, taking advantage of the memoryless property of the exponential law. This requires the definition of a counter variable ($\tilde N_{j,k}$ below) that keeps track of how many jumps of type $j$ have already occurred before the $k^{th}$ jump. The second difference is that, in Construction~\ref{const:1}, the randomness involved in the position after the $k^{th}$ jump is simply given by a variable $U_k$ while, in Construction~\ref{const:2}, each jump type $j$ has its own stock of variables $(U_{j,k})_{k\in\nsets}$ so that $U_{j,k}$ is consumed only at the $k^{th}$ jump of type $j$. }

\noindent\hfil\rule{\textwidth}{.4pt}\hfil
\begin{construction}
\label{const:2}
 Let $W_0$ be a \rv~ with distribution $\mu_0 \in \mcp(\msm)$ and $(E_{j,k},U_{j,k})_{j\in\iintLigne{1,\ell},k\in \nsets}$ be  an i.i.d. family, independent of $W_0$, such that for all $k\in \nset$ and $j\in \iintLigne{1,\ell}$, $U_{j,k}$ is uniformly distributed on $[0,1]$  and $E_{j,k}$ is an exponential \rv~ with parameter $1$, independent of $U_{j,k}$.\\
  Set $\tS_0 = 0$, $Y_0' = W_0$, $\bN_{0} = 1$, $\tH_{j,1} = E_{j,1}$ and $\tN_{j,1} = 1$, for $j\in \cco 1,\ell\ccf$. Suppose that $(Y_t)_{t \leq \S_k}$ and  $(Y_{k}',\tS_k,\bN_{k},(\tH_{j,k+1},\tN_{j,k+1})_{j \in \iint{1,\ell}})$ have been defined for some $k\in \mathbb N$. Set 
\begin{equation*}
\tS_{j,k+1}   =  \inf \ensemble{ t>\tS_k}{ \tH_{j,k+1} < \int_{\tS_k}^t \lambda_j\parenthese{s, \varphi_{\tS_k,s}(Y_{k}')} \rmd s }\eqsp, \, \tS_{k+1}  =  \underset{j\in\iint{1,\ell}}\min \tS_{j,k+1} \eqsp.
\end{equation*}
\begin{itemize}
\item If $\tS_{k+1} = +\infty$, set $\tS_m=+\infty$, $Y'_{m} = \infty$, $\tI_m = 1$ for all $m>k$ and $Y_t = \varphi_{\tS_k,t}(Y'_k)$ for $t \geq \tS_k$.
\item  If $\tS_{k+1} < +\infty$, set
  \[
    \begin{array}{rclcrcl}
      \tI_{k+1} & =  & \min \{j\in \cco 1,\ell \ccf,\ \tS_{j,k+1} = \tS_{k+1}\} &\eqsp, \, & \bN_{k+1} =  \tN_{\tI_{k+1},k+2}&  =&  \tN_{\tI_{k+1},k+1}+1 \eqsp, \\
      Y_{k+1}' &= &
\bfG_{\tI_{k+1}} (  \tS_{k+1}, \varphi_{\tS_k,\tS_{k+1}}(Y_{k}'),U_{\tI_{k+1},\bN_{k+1}})
 & \eqsp, \, & \tH_{\tI_{k+1},k+2}  &= &  E_{\tI_{k+1},\bN_{k+1}} \eqsp, 
  \end{array}
\]
and for $j\neq \tI_{k+1}$,
\begin{equation*}
  \tH_{j,k+2}  =  \tH_{j,k+1} - \int_{\tS_k}^{\tS_{k+1}} \lambda_j\parenthese{s, \varphi_{\tS_k,s}(Y_{k}')} \rmd s \eqsp, \quad \tN_{j,k+2} = \tN_{j,k+1} \eqsp. 
\end{equation*}
Set $Y_t =  \varphi_{\tS_k,t}(Y'_k)$ for $t \in \ooint{\tS_k,\tS_{k+1}}$ and  $Y_{\tS_{k+1}} = Y'_{k+1}$.
\end{itemize}
For $t \geq \sup_{k \in \nset} \tS_k$, set $Y_t = \infty$.
\end{construction}
\noindent\hfil\rule{\textwidth}{.4pt}\hfil
\bigskip

We show in the following result that the two constructions we consider define the same distribution on $\rmD(\rset_+,\msm\cup\{\infty\})$.
 \begin{proposition}
   \label{propo:eg_deux_proc_1}
The two Markov chains $(X'_k,S_k,I_k)_{k \in \nset}$ and
   $(Y'_k,\tS_k,\tI_k)_{k \in \nset}$ have the same distribution on
   $((\msm\cup\{\infty\}) \times (\rset_+\cup\{+\infty\}))^{\nset}$. Therefore, $(X_t)_{t \geq 0}$ and $(Y_t)_{t \geq 0}$ have the same distribution on $\mrd(\rset_+,\msm\cup\{\infty\})$.
 \end{proposition}
 We preface the proof by a lemma.
 Denote by $(\tmcf_{k})_{k\in \nset}$ and $(\tmcf_{k}')_{k\in \nset}$ the
filtration associated with the sequence of random variables $(Y_{k}',\tS_k,\tI_k)_{k \in \nset}$ and $(Y_{k}',\tS_k)_{k \in \nset}$.  

% Before showing that $(\bX_t,\bY_t)_{t \geq 0}$ has the same
% distribution as $(\tX_t,\tY_t)_{t \geq 0}$, we need to derive some
% properties on the distributions associated with the sequence of random
% variables $(\bH_n)_{n \in \nset^*}$. 
\begin{lemma}
  \label{lem:prop_bH}
  For all $k \in \nset$, given $\{\tS_k < \plusinfty\}$,
  $(\tH_{j,k+1})_{j \in \iint{1,\ell}}$ are \iid~exponential random
  variables with parameter $1$, independent of $\tmcf'_{k}$. In
  addition, for all $i \in \iint{1,\ell}$, given
  $\{\tI_{k} = i \}\cap \{\tS_k < \plusinfty\}$,
  $(\tH_{j,k+1})_{j \in \iint{1,\ell}\setminus\{i\}}$
  % $(\tH_{j,k}-\int_{0}^{\tT_{k+1}} \lambda_j( \tS_k+s, \varphi_{\tS_k,\tS_k+s}(Y_{k}')) \rmd s)_{j \in \iint{1,\ell}\setminus\{i\}}$
  are
  \iid~exponential random variables with parameter $1$, independent of
  $\tmcf'_k$. 
\end{lemma}
\begin{proof}
  Set for all $k \in \nsets$ and $j \in \iint{1,\ell}$, $B_{j,k} = \1_{\rset_+} (\tS_k)\int_{\tS_{k-1}}^{\tS_{k}} \defEnsLigne{\lambda_j(s,
  \varphi_{\tS_{k-1},s}(Y_{{k-1}}'))} \rmd s$.
  Note that the second statement is equivalent to for all
  $k \in \nsets$ and $i \in \iint{1,\ell}$,
  $(\tH_{j,k}-B_{j,k})_{j \in \iint{1,\ell}\setminus\{i\}}$ are
  \iid~exponential random variables with parameter $1$,  independent of $\sigma(\tmcf'_{k-1},\tS_{i,k})$ given
  $\{\tS_{k} = \tS_{i,k}\}$ since for all $\msa \in \tmcf'_k$,
  $\{\tS_{k} = \tS_{i,k}\} \cap \msa \in
  \sigma(\tmcf'_{k-1},\tS_{i,k})$, which is the result that we will
  show.

  The proof is by induction on $k \in \nsets$. For $k=1$, by
  definition the first  statement holds. The second part follows
  from the memoryless property of the exponential distribution and
  because for all $i \in \iint{1,\ell}$, $(\tH_{1,j} = E_{1,j})_{j \in \iint{1,\ell}\setminus\{i\}}$, is  independent of
  $\sigma(\tmcf'_{0},\tS_{1,i})$.

Assume now that the result holds for $k \in \nsets$. Then for all $t_1,\ldots,t_\ell \geq 0$, we have using the induction hypothesis, the definition of $(\tH_{j,k+1})_{j \in \iint{1,\ell}}$, the memoryless property of the exponential distribution and since given $\{\tS_{k} = \tS_{i,k}\}$, $E_{i,\bN_{k+1}}$ is independent of $\sigma(\tmcf'_{k},\tS_k, (\tH_{j,k})_{j \in \iint{1,\ell}})$ for all $i \in \iint{1,\ell}$,
\begin{align*}
  &  \1_{\rset_+} (\tS_k) \CPP{\bigcap_{j=1}^{\ell}\{\tH_{j,k+1} \geq t_j \}}{\tmcf'_{k}} &\\
&   \qquad \qquad =   \1_{\rset_+} (\tS_k) \sum_{i=1}^\ell  \CPP{\bigcap_{j=1}^{\ell}\{\tH_{j,k+1} \geq t_j \} \cap\{ \tS_{k} = \tS_{i,k}\}}{\tmcf'_{k}} \\
&\qquad \qquad =    \1_{\rset_+} (\tS_k) \sum_{i=1}^\ell  \CPP{\bigcap_{j=1, j \not = i}^{\ell}\{\tH_{j,k+1} \geq t_j \} \cap\{ \tS_{k} = \tS_{i,k}\} \cap \{\bE_{i,\bN_{k+1}} \geq t_i\}}{\tmcf'_{k}}\\
  &\qquad  \qquad  =\1_{\rset_+} (\tS_k) \exp\parenthese{-\sum_{j=1}^{\ell} t_j}\eqsp.
\end{align*}
which shows the first part of the statement. Finally we show the second statement of the induction.
Note that $(\tH_{j,k+1})_{j \in \iint{1,\ell}\setminus\{i\}}$ is an independent
family of random variables, independent of $\tmcf'_k$ and
$\tS_{i,k+1}$, for $i \in \iint{1,\ell}$ and therefore given $\{\tI_{k+1} = i\}$, $(\tH_{j,k+1})_{j \in \iint{1,\ell}\setminus\{i\}}$ is independent of $(B_{j,k+1})_{j \in \iint{1,\ell}\setminus\{i\}}$. Then,  using the first statement and
the memoryless property of the exponential distributions, we have for
all $t_1,\ldots,t_\ell \geq 0$,
\begin{align*}
& \1_{\rset_+}(\tS_{k+1}) \CPP{\bigcap_{j=1,j\not= i}^{\ell} \{\tH_{j,k+1}-B_{j,k+1} \geq t_j\}\cap \{\tS_{k+1} = \tS_{i,k+1}\} }{\sigma(\tmcf'_{k},\tS_{i,k+1})}\\
&      = \1_{\rset_+}(\tS_{k+1}) \CPP{\bigcap_{j=1,j\not= i}^{\ell} \defEns{\{\tH_{j,k+1}-B_{j,k+1} \geq t_j\}\cap \{\tH_{j,k+1} > B_{j,k+1}\}} }{\sigma(\tmcf'_{k},\tS_{i,k+1})}
  \\
&   
  =  \1_{\rset_+}(\tS_{k+1}) \exp\parenthese{-\sum_{j=1,j \not = i}^{\ell} t_j}  \eqsp. 
  % &  \CPP{\bigcap_{j=1,j\not= i}^{\ell} \{\tH_{j,k+1}-\int_{0}^{\tT_{k+1}} \defEns{\lambda_j( \tS_k+s, \varphi_{\tS_k,\tS_k+s}(Y_{k}'))} \rmd s \geq t_j\}\cap \{\tT_{k+1} = \tT_{i,k+1}\} }{\sigma(\tmcf_{k},\tT_{i,k+1})}\\
% & \quad \qquad  \quad \qquad \\
%   &= \CPP{\bigcap_{j=1,j\not= i}^{\ell} \defEns{\{\tH_{j,k+1}-\int_{0}^{\tT_{k+1}} \defEns{\lambda_j( \tS_k+s, \varphi_{\tS_k,\tS_k+s}(Y_{k}'))} \rmd s \geq t_j\}\cap \{\tH_{j,k+1} > \int_{0}^{\tT_{k+1}} \defEns{\lambda_j( \tS_k+s, \varphi_{\tS_k,\tS_k+s}(Y_{k}'))} \rmd s\}} }{\sigma(\tmcf_{k},\tT_{j,k+1})}  \\
%  = \rme^{-\lambdab t } \CPP{  \tH_{n+1} > \tT^2_{n+1} }{\sigma(\tmcf_{n},\tT^2_{n+1})}
\end{align*}

% Assume now that the result holds for $k \in \nsets$. Let $i\in \iint{1,\ell}$. Then for all $t \geq 0$, we have using the induction hypothesis, the definition of $\tH_{i,k+1}$, the memoryless property of the exponential distribution and since given $\{\tT_{k+1} = \tT_{i,k+1}\}$, $E_{i,\tN_{k+2}}$ is independent of $\sigma(\tmcf_{k},\tT_k)$
% \begin{align*}
% &
%   \CPP{\tH_{i,k+1} \geq t}{\tmcf_{k}} =  \sum_{j=1, j\not = i}^\ell  \CPP{\tH_{i,k+1} \geq t, \tT_{k} = \tT_{j,k}}{\tmcf_{k}} + 
% \CPP{\tH_{i,k+1} \geq t, \tT_{k} = \tH_{i,k}}{\tmcf_{k}} \\
% &=  \sum_{j=1, j\not = i}^\ell \CPP{\tH_{i,k} - \tT_{j,k} \geq t, \tT_{k} = \tT_{j,k}}{\tmcf_{k}} + 
% \CPP{\bE_{i,\bN_{n+2}} \geq  t, \tT_{k} = \tH_{i,k}}{\tmcf_{k}} \\
% &=  \rme^{- t}  \sum_{j=1, j\not = i}^\ell \CPP{\tT_{k} = \tT_{j,k}}{\tmcf_{k}} + 
% \rme^{- t} \CPP{ \tT_{k} = \tH_{i,k}}{\tmcf_{k}} = \rme^{-t} \eqsp,
% \end{align*}
% which shows the first part of the statement. Finally since $\tH_{i,k+1}$ is
% independent of $\tmcf_k$ and $\tT_{j,k+1}$, for $j \in \iint{1,n}$, $j \not = i$, using the first statement
% and the memoryless property of the exponential distributions, we have
% \begin{align*}
% &  \CPP{\tH_{i,k+1}-\tT_{i,k+1} \geq t, \tT_{k+1} = \tT_{j,k+1} }{\sigma(\tmcf_{k},\tT_{j,k+1})}\\
% & \quad \qquad  \quad \qquad  =  \CPP{\tH_{i,k+1}-\tT_{j,k+1} \geq t, \tH_{i,k+1} > \tT_{j,k+1} }{\sigma(\tmcf_{k},\tT_{j,k+1})} \\
% %  = \rme^{-\lambdab t } \CPP{  \tH_{n+1} > \tT^2_{n+1} }{\sigma(\tmcf_{n},\tT^2_{n+1})}
% & \quad \qquad   \quad \qquad = \rme^{-\lambdab t } \CPP{ \tT_{k+1} = \tT_{j,k+1} }{\sigma(\tmcf_{n},\tT^2_{j,k+1})} \eqsp.
% \end{align*}
\end{proof}

\begin{proof}[Proof of \Cref{propo:eg_deux_proc_1}]
  We show that the two processes $(X'_k,S_k,I_k)_{k \in \nset}$ and
  $(Y'_k,\tS_k,\tI_k)_{k \in \nset}$ have the same distribution.  Note
  that, since   $(X'_0,S_0,I_0)$ and $(Y'_0,\tS_0,\tI_0)$ have the same distribution,
  this result is equivalent  to show that
  $(Y'_k,\tS_k,\tI_k)_{k \in \nset}$ is also a Markov chain with a
  Markov kernel characterized by \eqref{eq:carac_chaine_markov_1}.
  %Let $(\tmcf_k)_{k \in\nsets}$ be the filtration associated with $(Y'_k,\tS_k,\tI_k)_{k \in \nset}$.
% \begin{multline}
% \label{eq:carac_chaine_markov_1}
%   \CPP{X'_{k+1}\in \msa, S_{k+1} \leq t, i_{k+1} = j}{\mcf_k} \\
% = \int_0^{t-S_k} \rmd s \parentheseDeux{\lambda_j(S_k+s,\varphi_{S_k,S_k+s}(X_k')) \, \exp\defEns{-\sum_{i=1}^\ell \int_0^s \rmd u \lambda_i(S_k+u,\varphi_{S_k,S_k+u}(X_k')) }}\eqsp.
% \end{multline}
Let $k \in \nsets$, $\msa \in \mcb{\msm}$, $t \geq \tS_k$,
$i\in \iint{1,\ell}$. By \Cref{lem:prop_bH} and definition of
$(Y'_{\tilde{k}},\tS_{\tilde{k}},\tI_{\tilde{k}})_{\tilde{k} \in \nset}$, since, given $\{\tI_{k+1}=i\} \cap \{\tS_{k+1} < \plusinfty\}$,
$Y'_{k+1} = \bfG(\tS_{i,k+1}, \varphi_{\tS_k,\tS_{i,k+1}}(Y'_k),U_{i,\bN_{k+1}})$ and $U_{i,\bN_{k+1}}$ is independent of $\tmcf_k$, then setting
$\mcg_{i,k+1} =\sigma(\tmcf_k,\tH_{i,k+1},U_{i,\bN_{k+1}})$ and $B_{j,k+1} = \1_{\rset_+}(\tS_{i,k+1})\int_{\tS_k}^{\tS_{i,k+1}} \lambda_j( s,
\varphi_{\tS_k,s}(Y_{k}')) \rmd s$, for $j \in \iint{1,\ell}\setminus\{i\}$, we have
\begin{align*}  
  &\CPP{Y'_{k+1}\in \msa, \tS_{k+1} \leq t, \tI_{k+1} = i}{\tmcf_k} \\
  &     =   \CPP{Y'_{k+1} \in \msa, \tS_{i,k+1} \leq t , \tS_{i,k+1} < \tS_{j,k+1}, \text{ for all $j \in \iint{1,\ell}\setminus\{i\}$}, \tI_{k+1} = i}{\tmcf_k}    \\
  &     =   \CPE{\1_\msa(Y'_{k+1})  \1_{\ccint{\tS_k,t}}(\tS_{i,k+1}) \CPP{ \bigcap_{j \in \iint{1,\ell}, j \not = i} \{\tS_{i,k+1} \leq \tS_{j,k+1}\}}{\mcg_{i,k+1}}}{\tmcf_k}   \\
&     =   \CPE{\1_\msa(Y'_{k+1}) \1_{\ccint{\tS_k,t}}(\tS_{i,k+1}) \CPP{  \bigcap_{j \in \iint{1,\ell}, j \not = i} \{ B_{j,k+1} < \tH_{j,k+1}\}}{\mcg_{i,k+1}}}{\tmcf_k}\\
  &=  \CPE{\1_\msa(Y'_{k+1}) \1_{\ccint{\tS_k,t}}(\tS_{i,k+1}) \exp\defEns{-\sum_{j=1,j \not = i}^\ell \int_t^{\tS_{i,k+1}}  \lambda_j(u,\varphi_{\tS_k,u}(Y_k'))\rmd u }}{\tmcf_k} \eqsp. 
  % &\CPP{Y'_{k+1}\in \msa, \tS_{k+1} \leq t, \tI_{k+1} = j}{\tmcf_k} \\
  % &     =   \CPP{\bfG(\tT_{j,k+1}+ \tS_k, \varphi_{\tS_k,\tT_{j,k+1}+ \tS_k}(Y'_k),U_{k+1}) \in \msa, \tT_{j,k+1} \leq t - \tS_k, \tT_{j,k+1} \leq \tT_{i,k+1}, \text{ for all $i \in \iint{1,\ell}\setminus\{j\}$}}{\tmcf_k}    \\
  % &     =   \CPE{\1_\msa(\bfG(\tT_{j,k+1}+ \tS_k, \varphi_{\tS_k,\tT_{j,k+1}+ \tS_k}(Y'_k),U_{k+1})) \1_{\ccint{0,t-S_k}}(\tT_{j,k+1}) \CPP{ \tT_{j,k+1} \leq \tT_{i,k+1}, \text{ for all $i \in \iint{1,\ell}\setminus\{j\}$}}{\sigma(\tmcf_k,\tH_{j,k+1},U_{k+1})}}{\tmcf_k}   \\
  % &     =   \CPE{\1_\msa(\bfG(\tT_{j,k+1}+ \tS_k, \varphi_{\tS_k,\tT_{j,k+1}+ \tS_k}(Y'_k),U_{k+1})) \1_{\ccint{0,t-S_k}}(\tT_{j,k+1}) \CPP{ B_{i,k+1} < \tH_{i,k+1}, \text{ for all $i \in \iint{1,\ell}\setminus\{j\}$}}{\sigma(\tmcf_k,\tH_{i,k+1},U_{k+1})}}{\tmcf_k}\\
  % &=  \CPE{\1_\msa(\bfG(\tT_{j,k+1}+ \tS_k, \varphi_{\tS_k,\tT_{j,k+1}+ \tS_k}(Y'_k),U_{k+1})) \1_{\ccint{0,t-S_k}}(\tT_{j,k+1}) \exp\defEns{-\sum_{i=1,i \not = j}^\ell \int_0^{\tT_{j,k+1}} \rmd u \lambda_i(S_k+u,\varphi_{S_k,S_k+u}(X_k')) }}{\tmcf_k} \eqsp. 
\end{align*}
The proof then follows from the definition of $\tS_{i,k+1}$ and $Y'_{k+1}$, and \Cref{lem:prop_bH}.
\end{proof}

%The only  difference between $(X_t)_{t \geq 0}$ and $Y$ is the following: in the first case, for $k\geqslant 1$, at time $T_k$, if $j\neq i_k$, then the variable $E_{j,k}$ is thrown away and a new variable $E_{j,k+1}$ is used to defined $T_{j,k+1}$. In the second case, at time $S_k$, if $i\neq j_k$, then $E_{j,N_{j,k}}$ is kept.
For $k\geqslant 1$ with $S_k <\infty$, we say that, at time $S_k$, the process $(X_t)_{t \geq 0}$ given by \Cref{const:1} has made a jump of type $I_k$, or equivalently that $S_k$ is a jump time of type $I_k$. Denote
\begin{equation}
  \label{eq:def_t_j}
  T^{(j)}\ = \ \inf\ensemble{S_k}{\ k\geqslant 1,\ I_k = j}
\end{equation}
 the first jump time of type $j$. Then, one example of application of \Cref{propo:eg_deux_proc_1} is the following result.
 \begin{proposition}
   \label{prop:premier_bounce}
Let $\ell=\ell_1+\ell_2$ with $\ell_1,\ell_2\in\nsets$. Let $(X_t)_{t \geq 0}$ be a PDMP on $\msm$ with characteristics $(\varphi,(\lambda_i,Q_i)_{i \in \iint{1,\ell}})$ given by \Cref{const:1} and initial distribution $\mu_0$. Define $T = \min\ensembleLigne{T^{(i)}}{i\in \iint{\ell_1+1,\ell} }$, where $T^{(j)}$ is given by \eqref{eq:def_t_j} for all $j \in \iint{1,\ell}$ . Then the cumulative distribution function of $T$ is given for all $u\geqslant 0$ by
\begin{equation}
   \label{eq:premier_bounce}
\proba{ T \leq u}  =  \proba{ E <  \sum_{i\in \iint{\ell_1+1}}^{\ell}\int_0^{u \wedge \tau_\infty(Z)}\lambda_{i}\po s,Z_s\pf \rmd s }\eqsp,
 \end{equation}
 where $ (Z_t)_{t \geq 0}$ is a PDMP with characteristics $(\varphi,(\lambda_i,Q_i)_{i\in \iint{1,\ell_1}})$  and initial distribution $\mu_0$, and $E$ is a standard exponential \rv~independent of $ (Z_t)_{t \geq 0}$.
 \end{proposition}

 \begin{proof}
   Let $(Y_t)_{t \geq 0}$ be a PDMP defined by  \Cref{const:2} with characteristics  $(\varphi,(\lambda_i,$ $Q_i)_{i\in \iint{1,\ell}})$  and initial distribution $\mu_0$. Define similarly to $(X_t)_{t \geq 0}$ for all $j \in \iint{1,\ell}$,
%    \begin{equation}
%   \label{eq:def_t_j_y}
% \eqsp,
% \end{equation}
$  \tT^{(j)}\ = \ \inf\ensembleLigne{\tS_k}{\ k\geqslant 1,\ \tI_k = j} $ and $\tT = \min\ensembleLigne{\tT^{(i)}}{i \in \iint{\ell_1+1,\ell_2} }$. Note that since by \Cref{propo:eg_deux_proc_1}, $(X'_k,S_k,I_k)_{k \in \nset}$ and $(Y'_k,\tS_k,\tI_k)_{k \in \nset}$ has the same distribution, $T$ and $\tT$ have the same distribution and it suffices to show that the cumulative distribution function of $\tT$ is given by \eqref{eq:premier_bounce}.

Let $(Z_t)_{t \geq 0}$ be a PDMP with characteristics $(\varphi,(\lambda_i,Q_i)_{i \in \iint{1,\ell_1}})$ and initial distribution $\mu_0$ defined by \Cref{const:2} and based on the \rvs~$W_0$, $(E_{j,k},U_{j,k})_{j \in \iint{1,\ell_1}, k \in \nset}$, and let $(Z_k',R_k,J_k)_{k \in \nset}$ be the corresponding embedded chain. By construction, for all $t \leq \tT \wedge \tau_{\infty}(Z)$, $Y_t =Z_t$. In addition, define
\begin{equation*}
  N = \inf\ensemble{k \in \nsets}{\text{ there exists } i \in \iint{\ell_1+1,\ell}, \tI_k = i} \eqsp.
\end{equation*}
By definition, $\tT= \tS_N$ on $\{ \tT <  \plusinfty\}$ and for all $k \in \nsets$, on $\{N=k\}$ for all $t \in \ccintLigne{0,\tS_k}$, $Y_t = Z_t$, and for all $n \leq k$, $Y'_n = Z_n'$, $\tS_n = R_n$. Therefore, for all $k\in \nsets$, on $\{N\geq k\}\cap\{\tau_{\infty}(Z) \geq t\}$, for all $i \in \iint{\ell_1+1,\ell}$, we have by induction
\begin{equation*}
  \tS_{i,k} = \inf \ensemble{ t>R_{k-1}}{ \tH_{i,k} < \int_{R_{k-1}}^t \lambda_i\parenthese{s, \varphi_{R_{k-1},s}(Z_{k}')} \rmd s }
   = \inf \ensemble{ t> 0 }{ E_{i,0} < \int_{0}^t \lambda_i\parenthese{s, Z_s} \rmd s } \eqsp.
 \end{equation*}
Since $\{\tT < \tau_{\infty}(Z)\} \subset \{\tT < \plusinfty\}$, we thus obtain
\begin{align}
  \nonumber
  \{\tT < \tau_{\infty}(Z)\} \cap   \{\tT \geq t\} &=  \{\tT < \tau_{\infty}(Z)\} \cap \defEns{ \bigcap_{k \in \nsets, \, i \in \iint{\ell_1+1,\ell}} \{ \tS_{i,k} \geq t\} \cap \{N = k\}}\\
  \label{eq:premier_bounce_1}
  &=  \{\tT < \tau_{\infty}(Z)\} \cap \defEns{  \bigcap_{  i \in \iint{\ell_1+1,\ell}} \defEns{ E_{i,0} \geq \int_{0}^t \lambda_i\parenthese{s, Z_s} \rmd s } }\eqsp.
\end{align}

In addition, since $\{ \tT = \plusinfty\} \subset \{ \tau_{\infty}(Z) = \tau_{\infty}(Y)\} \subset \{\tT \geq \tau_{\infty}(Z)\}$, we have
\begin{align}
  \nonumber
  \{\tT \geq \tau_{\infty}(Z) \vee t \}  = \{\tT = \plusinfty\} &= \bigcap_{i \in \iint{\ell_1+1,\ell}, \, k \in \nsets} \{ \tS_{i,k} \geq R_k \} \\
  \label{eq:premier_bounce_2}
                                                         & =    \bigcap_{  i \in \iint{\ell_1+1,\ell}} \defEns{ E_{i,0} \geq \int_{0}^{\tau_{\infty}(Z)} \lambda_i\parenthese{s, Z_s} \rmd s }  \eqsp.
\end{align}
Combining \eqref{eq:premier_bounce_1} and \eqref{eq:premier_bounce_2} and since $(E_{i,0})_{i \in \iint{\ell_1+1,\ell_2}}$ is independent of $(Z_s)_{s \geq 0}$, we get
\begin{equation*}
  \proba{\tT \geq t } = \proba{\bigcap_{  i \in \iint{\ell_1+1,\ell}} \defEns{ E_{i,0} \geq \int_{0}^{\tau_{\infty}(Z) \wedge t } \lambda_i\parenthese{s, Z_s} \rmd s }} = \expe{\exp\parenthese{- \sum_{i=\ell_1+1}^{\ell} \int_0^{\tau_{\infty}(Z)\wedge t}  \lambda_i\parenthese{s, Z_s} \rmd s   }}\eqsp,
\end{equation*}
which concludes the proof.
% \begin{align*}
%   \proba{\tT > t} & = \sum_{k \in \nsets} \proba{\{N=k\} \cap \bigcap_{i\in \iint{\ell_1+1}}^{\ell} 
% \end{align*}
% Let $ (X_t)_{t \geq 0}\sim \PDMP\po \varphi,(\lambda_i,Q_i)_{i\in \cco 1,{\ell_1+\ell_2}\ccf},\mu_0\pf$ be defined through Construction 2 from some r.v.  $W_0$  and $(E_{j,k},U_{j,k})_{j\in\iintLigne{1,\ell_1+\ell_2},k\in \nset}$, and let $(X_k',T_k,i_k)_{k\in\nset}$ be its associated embedded chain. Let $ (\bar X_t)_{t \geq 0}\sim \PDMP\po \varphi,(\lambda_i,Q_i)_{i\in \cco 1,{\ell_1}\ccf},\mu_0\pf$ be defined through Construction 2 from  $W_0$  and $(E_{j,k},U_{j,k})_{j\in\iintLigne{1,\ell_1},k\in \nset}$. Then, by construction, $X_t=\bX_t$ for all $t\in[0,R\wedge \tau_\infty(\bX))$, and in particular if $\tau_\infty(\bX)<R$ then necessarily $\tau_\infty(X) = \tau_\infty(\bX)$ and $R=+\infty$ (there are infinitely many jumps of type in $\cco 1,\ell_1\ccf$ before any jump of type in $\cco \ell_1+1,\ell_1+\ell_2\ccf$). As a consequence, for all $j\in\cco \ell_1 + 1,\ell_1+\ell_2\ccf$,
% \[ T^{(j)} \ = \ \inf\ensemble{t>0}{E_{j,0} > \int_0^{t\wedge \tau_\infty(\bX)} \lambda_j\po s,\bX_s\pf \rmd s}\eqsp.\]
% Since $ (\bar X_t)_{t \geq 0}$ is a deterministic function of $W_0$  and $(E_{j,k},U_{j,k})_{j\in\iintLigne{1,\ell_1},k\in \nset}$, it is independent of $E_{j,0}$ for all $j>\ell_1$. Hence, for all $t\geqslant 0$,
% \begin{eqnarray*}
% \mathbb P(R > t) & = & \mathbb E \po \mathbb P \Big( \bigcap_{j=\ell_1+1 }^{\ell_1+\ell_2} \{ E_{j,0} > \int_0^{t\wedge \tau_\infty(\bX)} \lambda_j\po s,\bX_s\pf \rmd s\}\ \Big|\ (\bX_s)_{s\geqslant 0} \Big) \pf\\
% & = & \mathbb E \po \exp\left\{- \sum_{j=\ell_1+1 }^{\ell_1+\ell_2} \int_0^{t\wedge \tau_\infty(\bX)} \lambda_j\po s,\bX_s\pf \rmd s \right\}\pf
% \eqsp,
% \end{eqnarray*}
% which concludes.
\end{proof}

%  For $k\geqslant 1$ with $T_k <\infty$, we say that, at time $T_k$, the process $(X_t)_{t \geq 0}$ has made a jump of type $i_k$, or equivalently that $T_k$ is a jump time of type $i_k$. Denote
%  \[T^{(j)}\ = \ \inf\ensemble{T_k}{\ k\geqslant 1,\ i_k = j}\]
%  the first jump time of type $j$. Then, one example of application of \Cref{propo:eg_deux_proc_1} is the following:
%  \begin{proposition}
%    \label{prop:premier_bounce}
% Suppose $\ell=\ell_1+\ell_2$ with $\ell_1,\ell_2\in\nsets$ and set $R = \min\ensemble{T^{(\ell_1+j)}}{j\in\cco 1,\ell_2\ccf }$ . Then the repartition function of $R$ is given for all $t\geqslant 0$ by
%  \begin{eqnarray*}
%  \mathbb P \po R < t \pf & = & \mathbb P \po E <  \sum_{j=1}^{\ell_2}\int_0^{t\wedge \tau_\infty(\bX)}\lambda_{\ell_1 + j}\po s,\bX_s\pf \rmd s\pf\eqsp,
%  \end{eqnarray*}
%  where $ (\bar X_t)_{t \geq 0}\sim \PDMP \po \varphi,(\lambda_i,Q_i)_{i\in \cco 1,{\ell_1}\ccf},\mu_0\pf$ and $E$ is a standard exponential r.v. independent of $ (\bar X_t)_{t \geq 0}$.
%  \end{proposition}

% \begin{proof}
% Let $ (X_t)_{t \geq 0}\sim \PDMP\po \varphi,(\lambda_i,Q_i)_{i\in \cco 1,{\ell_1+\ell_2}\ccf},\mu_0\pf$ be defined through Construction 2 from some r.v.  $W_0$  and $(E_{j,k},U_{j,k})_{j\in\iintLigne{1,\ell_1+\ell_2},k\in \nset}$, and let $(X_k',T_k,i_k)_{k\in\nset}$ be its associated embedded chain. Let $ (\bar X_t)_{t \geq 0}\sim \PDMP\po \varphi,(\lambda_i,Q_i)_{i\in \cco 1,{\ell_1}\ccf},\mu_0\pf$ be defined through Construction 2 from  $W_0$  and $(E_{j,k},U_{j,k})_{j\in\iintLigne{1,\ell_1},k\in \nset}$. Then, by construction, $X_t=\bX_t$ for all $t\in[0,R\wedge \tau_\infty(\bX))$, and in particular if $\tau_\infty(\bX)<R$ then necessarily $\tau_\infty(X) = \tau_\infty(\bX)$ and $R=+\infty$ (there are infinitely many jumps of type in $\cco 1,\ell_1\ccf$ before any jump of type in $\cco \ell_1+1,\ell_1+\ell_2\ccf$). As a consequence, for all $j\in\cco \ell_1 + 1,\ell_1+\ell_2\ccf$,
% \[ T^{(j)} \ = \ \inf\ensemble{t>0}{E_{j,0} > \int_0^{t\wedge \tau_\infty(\bX)} \lambda_j\po s,\bX_s\pf \rmd s}\eqsp.\]
% Since $ (\bar X_t)_{t \geq 0}$ is a deterministic function of $W_0$  and $(E_{j,k},U_{j,k})_{j\in\iintLigne{1,\ell_1},k\in \nset}$, it is independent of $E_{j,0}$ for all $j>\ell_1$. Hence, for all $t\geqslant 0$,
% \begin{eqnarray*}
% \mathbb P(R > t) & = & \mathbb E \po \mathbb P \Big( \bigcap_{j=\ell_1+1 }^{\ell_1+\ell_2} \{ E_{j,0} > \int_0^{t\wedge \tau_\infty(\bX)} \lambda_j\po s,\bX_s\pf \rmd s\}\ \Big|\ (\bX_s)_{s\geqslant 0} \Big) \pf\\
% & = & \mathbb E \po \exp\left\{- \sum_{j=\ell_1+1 }^{\ell_1+\ell_2} \int_0^{t\wedge \tau_\infty(\bX)} \lambda_j\po s,\bX_s\pf \rmd s \right\}\pf
% \eqsp,
% \end{eqnarray*}
% which concludes.
% \end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



==> invariant_D.tex <==

\section{Regularity estimates for PDMP semigroups}
\label{sec:stab_c1c}

In this section, only homogeneous processes are
considered. Nevertheless, our result can be applied to inhomogeneous
PDMP since if $(X_t)_{t\geq 0}$ is such a process on $\msm$ with
characteristics $(\varphi,Q,\lambda)$, then the process
$(X_t,t)_{t \geq 0}$ is a homogeneous PDMP on
$(\msm \times \rset_+, \mcbb(\msm \times \rset_+))$ with
characteristics $(\bar{\varphi},\bar{Q},\lambda)$
defined for all $t,s \in \rset_+$, $x \in \msm$ and $\msa \in \mcbb(\msm \times \rset_+)$ by
\begin{equation*}
  \bar{\varphi}_{s}((x,t)) = (\varphi_{t,t+s}(x),t+s)  \eqsp, \qquad \qquad \bar{Q}((x,t),\msa) = \int_{\msm\times \rset_+} \1_{\msa}((y,u))  Q(x,\rmd y) \otimes \updelta_t(\rmd u) \eqsp.
\end{equation*}

For our next result, we need the following definition.
\begin{definition}
We say that a
differential flow $\varphi$ on $\msm$ and a Markov kernel $Q$ are
compactly compatible if for all compact set $\msk \subset \msm$ and $T \geq 0$,
there exists a compact set $\tilde \msk \subset \msm$ satisfying for
all $N \in \nset$, $(t_i)_{i \in \{1,\ldots,N+1\}} \in \rset_+^n$,
$\sum_{i=1}^{N+1} t_i \leq T$,
\begin{equation}
\label{def:prop_tmsk}
\cup_{i=0}^{N} \msk_i \subset \tilde \msk \eqsp, \text{ and } \varphi_{s_i}( \msk_{i-1}) \subset \tilde \msk  \eqsp,
\end{equation}
for all $i \in \{1,\ldots,N+1\}$ and $s_i \in \ccint{0,t_i}$ setting
$t_0=0$, where $(\msk_i)_{i \in \{0,\ldots,N\}}$ is a sequence of
compact sets of $\msm$, satisfying
\begin{equation}
  \label{def:msk_i}
\msk \subset \msk_0 \text{  and for all $i\in \{0,\ldots,N-1\}$, } \bigcup_{x \in \msk_i} \supp \{ Q(\varphi_{t_{i+1}}(x),\cdot) \} \subset
\msk_{i+1} \eqsp.  
\end{equation}  
\end{definition}
Note that by definition, if $\varphi$ and $Q$ are compactly compatible
and the PDMP semigroup with local characteristics $(\varphi, \lambda,Q)$ is
non-explosive, for all $t \geq 0$ and all
compact set $\msk \subset \msm$, there exists a compact set
$\tilde \msk \subset \msm$, such that
$\PP (X_s \in \tilde{\msk}, \text{ for all $s \in \ccint{0,t}$} ) =1$,
where $(X_t)_{t \geq 0}$ is a PDMP process with local characteristics $(\varphi, \lambda,Q)$.

\begin{assumption}
  \label{ass:stability}
The local characteristics $(\varphi,\lambda,Q)$ satisfy
\begin{enumerate}[label = (\roman*)]
\item \label{item_1_lem:stab_c1c} the flow  $\varphi$ and the Markov kernel $Q$ are compactly compatible;
\item \label{item_2_lem:stab_c1c} $\lambda\in\mrc^{1}(\msm)$ and for
  all $f \in \mrc^1(\msm)$, $\lambda Qf \in \mrc^1(\msm)$ and there
  exists a function $\Psi :\msm \to \rset_+$ such that for all compact set $\msk \subset \msm$, $\sup_{y \in \msk} \Psi(y) < \plusinfty$ and for all 
  $x \in \msk$,
  \begin{equation*}
    \label{eq:1}
 \norm{\diff (\lambda Qf)(x)} \leq   \sup_{y \in \msk}\{ \Psi(y) \} \sup \ensemble{\abs{f(y)} + \norm{\diff f(y)}}{y \in \supp \{Q(x,\cdot)\}};
  \end{equation*}
\item \label{item_3_lem:stab_c1c} for all $t \in \rset_+$, we have $x \mapsto \varphi_t(x)$ is continuously differentiable  and for all compact $\msk \subset \msm$, 
  \begin{equation*}
    \sup \ensemble{\norm{\diff \varphi_s(x)}}{s \in \ccint{0,t}, x \in \msk} < \plusinfty \eqsp.
  \end{equation*}
\end{enumerate}  
\end{assumption}
\begin{lemma}
  \label{lem:stab_c1c}
  Let $(P_t)_{t\geqslant 0}$ be a non-explosive PDMP semigroup on $\msm$ with corresponding characteristics $(\varphi,\lambda,Q)$ satisfying \Cref{ass:stability}. 
  Then for all $f \in \mrc^1(\msm)$, $T \in \rset_+$, $P_Tf \in \mrc^1(\msm)$  and for all compact set $\msk \subset \msm$, there exists $C \geq  0$  such that for all $t \in \ccint{0,T}$,
  \begin{equation}
    \label{eq:lem_stab_clc}
  \sup_{x \in \msk}\{ \abs{P_t f}(x) + \norm{\diff (P_tf)(x)}\} \leq C \eqsp.  
  \end{equation}
%   In particular $\mrc^1(\msm)$ is a  core for $(P_t)_{t \geq 0}$. 
% that  and $(x,t)\in\msm\times\rset_+ \mapsto \norm{\na \varphi_t (x)}$ is locally bounded, and that there exist locally bounded functions $C_1:\msm \rightarrow \rset_+$ and $C_2:\rset_+\rightarrow \rset_+$  such that for all $f\in \rmc^1_c(\msm)$, $\lambda Qf\in \rmc^1_c(\msm)$ and for all $x\in\msm$, 
% \[\norm{\na (\lambda Q f)(x)}\ \leqslant  \ C_1(x)\sup\{|f(y)| + \norm{\na f(y)},\ y\in \supp Q(x,\cdot)\}\eqsp,\]
%  and for all $t\geqslant 0$,  $X_s \in \msb(X_0,C_2(t))$ for all $s\in[0,t]$ almost surely. Then, if $f\in \mrc^1_c(\msm)$, $ P_t f\in \mrc^1_c(\msm)$ for all $t \geq 0$. %Therefore, $\mrc^1_c(\msm)$ is a core for $(P_t)_{t \geq 0}$.
 
 
% More precisely, if $f\in \mrc^1_c(\msm)$ and $t\geqslant0$, then there exist $C>0$ and a compact $\msk$ of $\msm$  such that,  for all $s\in [0,t]$, the support of $P_s f$ is included in $\msk$ and  $\norm{\na P_s f}_\infty \leqslant C$.
\end{lemma}
\begin{remark}
  \Cref{lem:stab_c1c} can be generalized  under the condition that
for some $k \in \nsets$,  the local characteristics $(\varphi,\lambda,Q)$ satisfy
\begin{enumerate}[label = (\roman*)]
\item \label{item_1_lem:stab_c1c_b} the flow  $\varphi$ and the Markov kernel $Q$ are compactly compatible;
\item \label{item_2_lem:stab_c1c_b} $\lambda\in\mrc^{k}(\msm)$ and for all $f \in \mrc^k(\msm)$, $\lambda Qf \in \mrc^k(\msm)$ and there exists a function $\Psi :\msm \to \rset_+$ such that for all compact set $\msk \subset \msm$, $\sup_{y \in \msk} \Psi(y) < \plusinfty$ and for all $x \in \msk$, $i \in\{1,\ldots,k\}$,
  \begin{equation*}
    \label{eq:1}
  \norm{\diff^i (\lambda Qf)(x)} \leq    \sup_{y \in \msk} \{ \Psi(y)\} \sup \ensemble{ \norm{\diff^i f(y)}}{y \in \supp \{Q(x,\cdot)\} \eqsp,i \in\{1,\ldots,k\} };
  \end{equation*}
\item \label{item_3_lem:stab_c1c_b} for all $t \in \rset_+$, we have $x \mapsto \varphi_t(x)$ is $k$-times continuously differentiable  and for all compact $\msk \subset \msm$, 
  \begin{equation*}
    \sup \ensemble{\norm{\diff^i \varphi_s(x)}}{s \in \ccint{0,t}, x \in \msk\eqsp, i \in \{1,\ldots,k\}} < \plusinfty \eqsp.
  \end{equation*}
\end{enumerate}
Then for all function $f \in \mrc^k(\msm)$, and $T \in \rset_+$,
$P_Tf \in \mrc^k(\msm)$. In addition, for all compact set
$\msk \subset\msm$, and $T \in \rset_+$, there exists $C \geq 0$ such
that for all $t \in \ccint{0,T}$,
$\sup_{x \in \msk} \absLigne{P_t f}(x) + \sup_{x \in \msk, i
  \in\{1,\ldots,k\}} \norm{\diff^i P_t f(x)} \leq C$.
\end{remark}
% \begin{remark}
%   Note that in the case where the condition $\inf_{x \in \msm} \lambda(x) >0$ is not satisfied, we can simply consider a modified characteristics $(\varphi,\bar \lambda, \bar Q)$ which defines the same PDMP semigroup $(P_t)_{t \geq 0}$ where $\bar Q$ and $\bar \lambda$ are given for all $x \in \msm$ and $\msa \in \mcb{\msm}$ by
%   \begin{equation*}
%     \bar \lambda(x) = \lambda(x) + \rate \eqsp, \, \bar Q(x,\msa) = \bar \lambda^{-1}(x)\lambda(x) Q(x,\msa) + \parenthese{1-\bar \lambda^{-1}(x)\lambda(x)} \updelta_x(\msa) \eqsp,
%   \end{equation*}
%   for $\rate >0$. Then, if the other conditions of \Cref{lem:stab_c1c} are satisfied, the modified characteristics $(\varphi,\bar \lambda, \bar Q)$ satisfy these conditions as well and $\inf_{x \in \msm} \bar \lambda(x) \geq \rate$. 
% \end{remark}
\begin{proof}
  If the first statement of the Lemma holds, then the fact that $\mrc^1(\msm)$ is a  core for $(P_t)_{t \geq 0}$ is a consequence of \cite[Proposition 3.3]{ethier:kurtz:1986}. 
 
  We now show the first statement of the Lemma.  For all $x \in \msm$
  denote by $(X_t^x)_{t \geq 0}$ a PDMP starting from $x$ associated
  with the characteristics $(\varphi,\lambda,Q)$.  Let
  $(S_n^x)_{n \in \nset}$ be the jump times of $(X_t^x)_{t \geq 0}$
  for all $x \in \msm$. Let $f\in \mrc^1(\msm) $, $T\geqslant 0$ and a
  compact set $\msk \subset \msm$. For $T =0$, the result is
  straightforward so we consider $T >0$. Let $\tilde \msk$ satisfying for all $n \in \nset$,
$(t_i)_{i \in \{1,\ldots,n+1\}} \in \rset_+^n$,
$\sum_{i=1}^{n+1} t_i \leq T$, \eqref{def:prop_tmsk}.
% $\cup_{i=0}^{n} \msk_i \subset \tilde \msk$,
% $\varphi_{s_i}( \msk_{i-1}) \subset \tilde \msk$, for all
% $i \in \{1,\ldots,n+1\}$ and $s_i \in \ccint{0,t_i}$ setting
% $t_0=0$, where $(\msk_i)_{i \in \{0,\ldots,n\}}$ are given by \eqref{def:msk_i}. 

Since for all $x  \in \msk$, 
  $\PP (X_t^x \in \tilde \msk, \text{ for all } t \in \ccint{0,T}) = 1$,
  for all $t \in \ccint{0,T}$ and $x \in \msm$,
  \begin{equation*}
    \label{eq:core_proof_1}
    \abs{P_tf(x)} = \abs{\expe{f(X_t)}} \leq \sup_{y \in \tilde \msk} \abs{f}(y) \eqsp.
  \end{equation*}
  
Furthermore,  $(P_t)_{t \geq 0}$
  is assumed to be non-explosive. Therefore
  $\sup_{n \in \nset} \S^{x}_n = \plusinfty$ and we can consider the
  following decomposition for all $t \in \ccint{0,T}$ and $x \in \msk$
  \begin{equation}
    \label{eq:decomposition_regular_pDMP}
  P_tf(x)  = \sum_{n=0}^{\plusinfty} \expeMarkov{}{\1_{\coint{S^{x}_n,S^{x}_{n+1}}}(t) f(X^{x}_t)} \eqsp.
\end{equation}
  By induction on $n \in \nset$, we show that
  \begin{equation}
    \label{eq:def_F_n}
   F_{n,t} : x \mapsto
  \expeMarkov{}{\1_{\cointLigne{S^{x}_n,S^{x}_{n+1}}}(t)
    f(X^{x}_t)}  \eqsp,
  \end{equation}
 is continuously
  differentiable and in addition there exists $C \geq 0$ such that for all
  $n \in \nset$, $t \in \ccint{0,T}$
  \begin{equation}
    \label{eq:estimate_gradient_n}
\sup_{x \in \msk}   \norm{ \diff  F_{n,t} (x)} \leq C^n  /n!\eqsp.%       \expeMarkov{(x,y)}{\1_{\coint{\bS_n^{\epsilon},\bS_n^{\epsilon}}}(t) } \eqsp,
   \end{equation}
   %where $(\bS_n^{\epsilon})_{n \in \nset}$ are the event times of a Poisson process with constant jump rate $\rate$.
   Assume for the moment that this result holds. Then, we have for all $t \in \ccint{0,T}$,
    \begin{equation*}
      \lim_{N \to \plusinfty}   \sum_{n=N}^{\infty} \sup_{x \in \msk}  \norm{ \diff F_{n,t}(x) } = 0 \eqsp. 
    \end{equation*}
    By \eqref{eq:decomposition_regular_pDMP}, it implies that
    $x \mapsto P_T f(x)$ is continuously differentiable. In
    addition, for all compact set $\msk \subset\msm$, there exists $C$ such that for all $t \in \ccint{0,T}$
    \begin{equation*}
        \label{eq:core_proof_0}
      \sup_{x \in \msk} \norm{\diff P_tf(x)} \leq C \eqsp.
    \end{equation*}
This result and \eqref{eq:core_proof_1} imply \eqref{eq:lem_stab_clc}.
  
    We now turn in showing that for all $n \in \nset$, $F_n$ is
    continuously differentiable and \eqref{eq:estimate_gradient_n}
    holds. We first show this result for $n = 0$. In a second time, we
    make an induction on $n \in \nsets$. 

For all $x \in \msk$ and $t \in \ccint{0,T}$, we have
    \begin{equation*}
      F_{0,t}(x) =  f(\phi_t(x)) \exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \eqsp. 
    \end{equation*}
Therefore, for all $x\in \msk$ and $t \in \ccint{0,T}$, we obtain by \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c}
    \begin{multline*}
      \diff F_{0,t}(x) = \defEns{\diff f (\phi_t(x))} \diff (\phi_t)(x) \exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \\
+        f(\phi_t(x))   \parentheseDeux{\int_0 ^t \defEns{\diff  \lambda (\phi_s(x)) \cdot \diff(\phi_s)(x) }\rmd s}\exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \eqsp.
\end{multline*}
Since for all $x \in \msk$ and $t \in \ccint{0,T}$, $\varphi_t(x) \in \tilde \msk$, $f \in \mrc^1(\msm)$ and using \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c}, we get there exists $C_0 \geq 0$ such that 
\begin{equation*}
\sup_{x \in \msk} [     \abs{F_0(x)}+    \norm{\diff F_0(x)}  ]\leq C_0 \eqsp.
    \end{equation*}
%    where we have used that for all $x \in \msm$, $\lambda(x) \geq \rate$.

We now show the result for $n \in \nsets$. We give first an explicit expression of $F_n$ for all $n \in \nsets$. Indeed, we have conditioning successively on $\mcf_{S_{n+1}^x}, \cdots, \mcf_{S_1^x}$, for all $x \in \msk$ and $t \in \ccint{0,T}$
\begin{multline}
  \label{eq:forme_loimarkov_chain}
  % \expeMarkov{(x,y)}{\1_{\coint{S^{(\epsilon)}_n,S^{(\epsilon)}_{n+1}}}(t) f(X^{(\epsilon)}_t,Y^{(\epsilon)}_t)}
  F_{n,t}(x)  = \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
  \int_0^{t-t_1} \rmd t_2 \exp\parenthese{-\int_0^{t_2} \lambda\defEns{\phi_{s_2}(x_1)} \rmd s_2}  \int_{\msm } \opK(\phi_{t_2}(x_1),\rmd x_2) \\
  \cdots   \int_0^{t-\sum_{i=1}^{n-1}t_i} \rmd t_n \exp\parenthese{-\int_0^{t_n} \lambda\defEns{\phi_{s_n}(x_{n-1})} \rmd s_n} \\
  \int_{\msm } \opK(\phi_{t_n}(x_{n-1}),\rmd x_n) f(\phi_{t-\sum_{i=1}^n t_i} (x_n))   \\  \exp\parenthese{-\int_0^{t-\sum_{i=1}^n t_i} \lambda\defEns{\phi_{s_{n+1}}(x_{n})} \rmd s_{n+1}} \eqsp,
\end{multline}
where $\opK$ is the kernel defined on $(\msm, \mcb{\msm})$  for all $x \in \msm$ and $\msa \in \mcb{\msm}$ by
  \begin{equation*}
    \opK(x,\msa) = \lambda(x) Q(x,\msa)  \eqsp.
  \end{equation*}

%   For the case $n=1$, we get for all $x \in \msk$ and $t \in \ccint{0,T}$,
%   \begin{multline}
%     \label{eq:first_estimate_gradient} 
%     F_{1,t}(x) =
%     \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1}  \lambda\defEns{\phi_{s_1}(x)} \rmd s_1}    \\
%       \times\left\lbrace \int_{\msm}  \lambda\parenthese{\phi_{t_1}(x)} Q(\phi_{t_1}(x),\rmd x_1) f\parenthese{\phi_{t-t_1}(x_1)} \exp\parenthese{-\int_0^{t-t_1} \lambda\defEns{\phi_{s_{2}}(x_1)} \rmd s_{2}} \right \rbrace
%   \eqsp.
% \end{multline}
% Since $f \in \mrc^1(\msm)$ and by \ref{item_1_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
% \begin{equation*}
%   x_1 \mapsto g(t_1,x_1) =  f\parenthese{\phi_{t-t_1}(x_1)} \exp\parenthese{-\int_0^{t-t_1} \lambda\defEns{\phi_{s_{2}}(x_1)} \rmd s_{2}} \eqsp,
% \end{equation*}
% is continuously differentiable for $t \in \ccint{0,T}, t_1 \in \ccint{0,t}$. In addition, for all $t \in \ccint{0,T}, t_1 \in \ccint{0,t}$ and for all $x_1 \in \supp \{Q(\varphi_{t_1}(x),\cdot)\}$, by \eqref{def:prop_tmsk}-\eqref{def:msk_i} $\varphi_{s_1}(x_1) \in\tilde K$ for all $s_1\in\ccint{0,t-t_1}$ and therefore
% \begin{equation*}
%   \abs{g}(t_1,x_1)  + \norm{\diff_x g(t_1,x_1)} < 2 \defEnsLigne{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{\diff \lambda }  \sup_{s \in \ccint{0,T}, y \in  \tmsk} \norm{\diff \varphi_{s}(y)}}\rme^{-\rate(t-t_1)} \eqsp.
% \end{equation*}
% Then by \ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
% $x \mapsto \lambda Qg(t_1,\varphi_{t_1}(x))$ is continuously differentiable for all
% $t \in \ccint{0,T}$, $t_1 \in \ccint{0,t}$ and for all $x \in \msk$,
% \begin{multline*}
%   \abs{\lambda Qg(t_1,\varphi_{t_1}(x))}  + \norm{\diff_x \lambda Qg(t_1,\varphi_{t_1}(x))}\\
%   \leq   4  \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}^2\rme^{-\rate(t-t_1)} \eqsp.
% \end{multline*}
%  In addition, since $\varphi_{t_1}(x) \subset \tilde \msk$, for all $t_1 \in \ccint{0,t}$, $t\in\ccint{0,T}$ and $x\in \msk$, by \ref{item_2_lem:stab_c1c}, we have
% \begin{multline*}
%   \sup_{x \in \msk} [\abs{F_1(x)} + \norm{\diff F_1(x) }] \\
%   \leq   8  \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}^3  t  \rme^{-\rate t} \eqsp.
% \end{multline*}

 We introduce a sequence of operator
$( Q^{(n)})_{n \in \nset^*}$, defined for all
$g : \rset_+ \times \msm \to \rset$, bounded on all compact of
$\rset_+ \times \msm$ and measurable, $t \in \ccint{0,T}$ and
$x \in \msm$ by
  \begin{multline}
\label{eq:def_q_n}
    Q^{(n)}_t g (x) = \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
    \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n  \exp\parenthese{-\int_0^{t_n} \lambda\defEns{\phi_{s_n}(x_{n-1})} \rmd s_n} \\\int_{\msm } \opK(\phi_{t_n}(x_{n-1}),\rmd x_n) g(t-\sum_{i=1}^n t_i ,x_n) \eqsp.
  \end{multline}
  Taking for $g$ the function
  $g_F : (s,y) \mapsto f(\varphi_s(y)) \exp(-\int_0^s \rmd u
  \lambda(\varphi_u(y)))$, we have $F_{n,t} = Q^{(n)}_t g_F$. Since
  $f \in \mrc^1(\msm)$ and by \Cref{ass:stability}-\ref{item_3_lem:stab_c1c}, $g_F$ is
  measurable, for all $s \in \rset_+$, $y \mapsto g_F(s,y)$ is
  differentiable on $\msm$ and satisfies for all $T' \geq 0$,
  $\msk' \subset \msm$ compact,
  $\sup_{s \in \ccint{0,T'}, y \in \msk'} \abs{g_F(s,y)} +
  \norm{\diff_x g_F(s,y)} < \plusinfty$. Therefore if we show that for
  all measurable function $g :\rset_+ \times \msm \to \rset_+$ such
  that for all $s \in \rset_+$, $y \mapsto g_F(s,y)$ is differentiable
  on $\msm$ satisfying for all $T' \geq 0$, $\msk' \subset \msm$
  compact,
  $\sup_{s \in \ccint{0,T'}, y \in \msk'} \abs{g_F(s,y)} +
  \norm{\diff_x g_F(s,y)} < \plusinfty$: 1) for all
  $t \in \ccint{0,T}$ and $x \in \msk$, $Q^n_t g$ is differentiable at $x$ 2) there exists $C \geq 0$ such that for all
  $x \in \msk$ and $t \in \ccint{0,T}$,
  \begin{equation}
    \label{eq:objectif_g}
    \abs{Q_t^{(n)} g(x)} + \norm{\diff_x Q_t^{(n)} g(x)} \leq C^n/(n!) \eqsp,
  \end{equation}
then \eqref{eq:estimate_gradient_n} holds which will conclude the proof.

  Note the following relation between $Q^{n-1}$ and $Q^1$ which will be essential in our next reasonings: for all
$g : \rset_+ \times \msm \to \rset$, bounded on all compact of
$\rset_+ \times \msm$ and measurable, $t \in \ccint{0,T}$ and
$x \in \msm$ 
  \begin{multline}
\label{eq:q_n_prop_q_1}
    Q^{(n)}_t g (x) = \int_{0}^t \rmd t_1  \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) Q_{t-t_1}^{n-1}g(x_1) \\
    = Q^{(1)}_t g_{n-1}(x)\eqsp,
  \end{multline}
where $g_{n-1}(s,y) = Q_{s}^{n-1}g(y)$ for all $s \in \rset_+$ and $y \in \msm$.
  
First, we make an induction on $i \in \{1,\ldots,n\}$ to show that for
all  $i \in \{1,\ldots,n\}$ and
$g : \rset_+ \times \msm \to \rset$, measurable, $y \mapsto g(s,y)$ is continuously
differentiable on $\msm$, for all $T' \in \rset_+$ and compact $\msk' \subset \msm$,
$\sup_{s \in \ccint{0,T'}, y \in \msk'} \norm{\diff_x g(s,y)} +
\abs{g}(s,y) < \plusinfty$, that $(s,x) \mapsto Q^{(i)}_s g $ is measurable, $y \mapsto Q^{(i)}_s g$ is continuously
differentiable on $\msm$, for all $T' \in \rset_+$ and compact $\msk' \subset \msm$,
$\sup_{s \in \ccint{0,T'}, y \in \msk'} \normLigne{\diff_x Q^{(i)}_s g(y)} +
\absLigne{Q^{(i)}_s g}(y) < \plusinfty$. For $i =1$, note that for all $s \in \rset_+$ and $y \in \msm$,
  \begin{equation}
  \label{eq:def_q_1}
    Q^{(1)}_sg(y) = \int_0^s \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(y)} \rmd s_1}  \int_{\msm } \opK(\phi_{t_1}(y),\rmd y_1) g(s-t_1 ,y_1) \eqsp.
  \end{equation}
  Let $T' \in \rset_+$, $\msk' \subset \msm$ be compact and $\tilde \msk'$ satisfying \eqref{def:prop_tmsk} associated with
  $\msk'$. Then for all $s \in \ccint{0,T'}$, $t_1\in\ccint{0,s}$, $\varphi_{t_1}(y) \in \tilde \msk '$ for all $y \in \msk'$. Therefore we have 
 by assumption on $g$, \ref{item_2_lem:stab_c1c} and \ref{item_3_lem:stab_c1c},
  $y \mapsto  \int_{\msm } \opK(\phi_{t_1}(y),\rmd y_1) g(s-t_1 ,y_1)$ for all $s \in \ccint{0,T'}$, $t_1 \in \ccint{0,s}$, is differentiable and there exists $C \geq 0$ such that for all $s \in \ccint{0,T'}$, $t_1 \in \ccint{0,s}$
  \begin{equation*}
    \sup_{y \in \msk'} \defEns{ \abs{\opK g(s-t_1 \cdot)(\phi_{t_1}(y))} + \norm{\diff_x  \opK g(s-t_1 \cdot)(\phi_{t_1}(y))}} < C \eqsp
  \end{equation*}
  By \eqref{eq:def_q_1}, we get then the result for $i=1$. The result for $i \in \{2,\ldots,n\}$ is then a straightforward consequence of \eqref{eq:q_n_prop_q_1} and the case $i=1$.

  We now show that for all $g : \rset_+ \times \msm \to \rset$, for
  all $s \in \rset_+$, $x \mapsto g(s,x)$ is continuously
  differentiable and for all $T'\in \rset_+$, compact set
  $\msk'\subset \msm$,
  $\sup_{s \in \ccint{0,T'}, y \in \msk'} \abs{g}(s,y) + \norm{\diff_x
    g(s,y)} < \plusinfty$, there exists $C \geq 0$ such that for all
  $x \in \msk$ and $t \in \ccint{0,T}$, \eqref{eq:objectif_g}
  holds. % Note that for all $j \in \{1,\ldots,n-1\}$, by \eqref{eq:def_q_n} we have for all
  % $s \in \rset_+$ and $x \in \msm$,
  % \begin{multline*}
  %   Q^n_tg(x) =  \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
  %   \cdots \int_{\msm } \opK(\phi_{t_{j}}(x_{j-1}),\rmd x_j)  Q_{t-\sum_{i=1}^{j} t_i}^{n-j} g(x_j) \eqsp.
  % \end{multline*}
  By an induction on $N \in \{1,\ldots,n\}$, we show that there exists $C \geq 0$ such that for all
  $N \in \{1,\ldots,n\}$, for all
  $(t_i)_{i \in \{1,\ldots,n-N\}} \in \rset_+^{n-N}$, 
  \begin{multline*}
    \sup_{x_{n-N} \in \msk_{n-N}} \abs{Q^N_{t-\sum_{j=1}^{n-N}t_j} g(x_{n-N}) } + \norm{\diff Q^N_{t-\sum_{j=1}^{n-N}t_j} g(x_{n-N}) } \\
    \leq C^{N} \defEns{\sup_{s \in \ccint{0,T}, y \in \tmsk} \abs{g(s,y)} +\sup_{s \in \ccint{0,T}, y \in \tmsk} \norm{\diff_x g(s,y)} }   \left. \parenthese{t-\sum_{j=1}^{n-N}t_j}^N \middle /(N!) \right .\eqsp,
  \end{multline*}
where $(\msk_j)_{j \in \{1,\ldots,n-N\}}$ are defined by \eqref{def:msk_i} relatively to $\msk$ and $\tmsk$.

%   Indeed, let
%   $x \in \msm$, $t \in \ccint{0,T}$ and
%   $g : \rset_+ \times \msm \to \rset$, bounded on all compact of
%   $\rset_+ \times \msm$, measurable, $y \mapsto g(s,y)$ is
%   continuously differentiable on $msm$, for all $s \in \rset_+$, Since
%   for all $y \in \msm$,

%   Then, an easy induction implies
%   by \eqref{def:prop_tmsk} that for all $i \in \{2,\ldots,n\}$,
%   $(t_j)_{i \in \{1,\ldots,i-1\}} \in \rset_+^n$,
%   $\sum_{j=1}^{i-1} t_j \leq t$, there exists
%   $(\msk_j)_{j \in \{1,\ldots,i-1\}}$ satisfying \eqref{def:msk_i} and
%   \begin{multline*}
%     \sup_{x_i \in \msk_i}      \abs{Q^{(i)}_{t-\sum_{j=1}^{i-1}t_j} g (x_i) } + \norm{\diff_x Q^{(i)}_{t-\sum_{j=1}^{i-1}t_j} g (x_i)}
%     \leq \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}
%   \end{multline*}
%   Note that using the same reasoning as for $F_1$, we get that for all
%   functions
%   $(u,x) \in \rset_+ \times \msm \mapsto g(u,x) \in \rset$,
%    measurable, continuously differentiable with respect to $x$, for all $u >0$, $x \mapsto Q^{(1)}_u g(x,y)$ is continuously differentiable. In addition, for all   $u \in \ccint{0,t}$, there exists $C \geq 0$ such that 

%   \begin{multline}
%     \label{eq:estimate_nabla_G_1}
% \sup_{x \in \msk}      \abs{Q^{(1)}_t g(x)} + \norm{\nabla Q^{(1)}_t g(x)} \\\leq C  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \defEns{
%       \sup_{\substack{x \in \msk}} \abs{g}(t-t_1,x) +  \sup_{\substack{x \in \msk}} \norm{\diff_{x}g}(t-t_1,x)} \eqsp.
%   \end{multline}

%   By an easy induction using that for all $t \geq 0$,
%   $g : \rset_+ \times \msm \to \rset$, bounded and measurable, $x \in \msm$
%   and $n \in \nsets$, $n >1$,
%   \begin{equation*}
%      Q^{(n)}_t g (x,y) =      Q^{(1)}_t [\tilde{g}_t] (x,y)  \eqsp, \quad \text{with }  \tilde{g} (t_1,w,z) = Q^{(n-1)}_{t_1} g (w,z) \eqsp,
%    \end{equation*}
%    for all $t_1 \in \ccint{0,t}$ and \eqref{eq:estimate_nabla_G_1}, we
%    have that for all functions
%    $(t,x,y) \rset_+ \times \msm \mapsto g(t,x,y) \in \rset$,
%    bounded and measurable, differentiable with respect to the space
%    variables $(x,y)$, for all $t >0$ and $n \in \nsets$,
%    $(x,y) \mapsto Q^{(n)}_t g(x,y)$ is continuously differentiable. In
%    addition, for all $R \geq 0$, $n \in \nsets$ and $T >0$, there
%    exists $C \geq 0$ such that for all $t \in \ccint{0,T}$,
%    $x \in \msm$, $\norm{x} + \norm{y} \leq R$,
%   \begin{multline*}
%     \label{eq:estimate_nabla_G_n}
%      \abs{Q^{(n)}_t g(x,y)} + \norm{ \nabla Q^{(n)}_t g(x,y)} \leq C^n  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n \rme^{-\rate t_n }  \\\defEns{
%        \sup_{\substack{x \in \msm\\ \norm{x} + (1+t) \norm{y} \leq R}} \abs{g}\parenthese{t-\sum_{i=1}^n t_i,x,y} +     \sup_{\substack{x \in \msm\\ \norm{x} + (1+t) \norm{y} \leq R}}  \norm{\nabla_{x,y}g}\parenthese{t-\sum_{i=1}^n t_i,x,y}} \eqsp.
%   \end{multline*}

%   Applying this result to the function
%   \begin{equation*}
%   (t,x,y) \mapsto     f(\phi_{t} (x_n,y_n))     \exp\parenthese{-\int_0^{t} \lambda\defEns{\phi_{s_{n+1}}(x_{n},y_{n})} \rmd s_{n+1}} \eqsp,
%   \end{equation*}
%   and using \eqref{eq:def_F_n}, we get that for all $n \in \nsets$,
%   $F_n$ is continuously differentiable. In addition, using that for
%   all $(z,w) \in \msm$, $\lambda(z,w) \geq \rate$, we
%   get for all $R \geq 0$, $n \in \nsets$ and $T >0$, there exists
%   $C \geq 0$ such that for all $t \in \ccint{0,T}$,
%   $x \in \msm$, $\norm{x} + \norm{y} \leq R$,
%   \begin{align*}
%     \label{eq:estimate_nabla_F_n}
%     &\abs{F_n(x,y)} + \norm{ \nabla F_n(x,y)} \\
%     &\qquad     \qquad  \leq C^n  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n \rme^{-\rate t_n }  \rme^{-(t-\sum_{i=1}^n t_i)\rate} \defEns{ \norm{f}_\infty + \norm{\nabla f}_\infty}  \\
%     &\qquad     \qquad   \leq  C^n \rme^{-t \rate } \int_0^t \rmd t_1  \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n   \defEns{ \norm{f}_\infty + \norm{\nabla f}_\infty}\eqsp,
%   \end{align*}
%   which shows that \eqref{eq:estimate_gradient_n} holds and concludes the proof. 
  

%   For all $s\in[0,t]$, we have by \eqref{item_4_lem:stab_c1c} for all $x \in \msm$,
%   \begin{equation*}
%    P_s f(x) = \int_{\msm} \1_{\msk_{x,t}}(y) f(y) P_s(x,\rmd y)   \eqsp.
%  \end{equation*}
%  Therefore $P_sf(x) = 0$ for all $x \in \msm$, 
%   $P_s f(x) = 0$ for all $x$ with $dist(x,\supp f) > \sup\{C_2(s),\ s\in[0,t]\}$. In particular, $P_t f$ is compactly supported. For any $x_0 \in \msm$, let us prove that $P_t f$ is $\rmc^1$ on $\msb(x_0,1)$. Let $\lambda_* = 1+ \sup\{\lambda(x),\ x\in\msb(x_0,1+C_2(t))\}$, and $(\bar P_t)_{t\geqslant 0}$ be the PDMP semigroup with characteristics $( \varphi,\lambda_*,Q_*)_{i\in \iintLigne{1,n}})$ with for all $x\in\msm$,
% \[Q_*(x,\cdot) \ = \  \frac{1 - (\lambda(x)\wedge \lambda_*)}{\lambda_*} \delta_x(\cdot) +  \frac{\lambda(x)\wedge \lambda_*}{\lambda_*} Q(x,\cdot) \eqsp.\]
% Then, for all $x\in \msb(x_0,1)$, $\bar P_t f(x) = P_t f(x)$.

%  Conditioning by the jump times of the process (which are jump times of an homogeneous Poisson process with intensity $\lambda_*$),
%  \begin{eqnarray*}
%  \bar P_t f(x) & = & \sum_{k\in\nset} \frac{(\lambda_* t)^k}{k!}\int_{\Delta_{k,t}} T_{s_1} Q_* T_{s_2} \dots Q_* T_{s_{k-1}} Q_* T_{s_k} f(x) \rmd s_1,\dots,\rmd s_k
%  \end{eqnarray*}
%  where, for $k\in\nset$, $\Delta_{k,t} = \{s\in \rset_+^k, \sum_{i=1}^k s_i = t\}$ and $T_r f(x) = f( \varphi_r(x))$. For a given $x\in \msb(x_0,1)$, $k\in\nset$ and $s\in \Delta_{k,t}$, let $E_0=\{x\}$, $E_{i} = \cup\{ \supp Q_*( \varphi_{s_i}(y),\cdot),\ y\in E_{i-1}\}$ for $i\in \iintLigne{1,k-1}$ and $E_k = \cup\{ \varphi_{s_k}(y),\ y\in E_{k-1}\}$. By assumption, for almost every $s\in \Delta_{k,t}$, $E_i \subset \msb(x,C_2(t))\subset \msb(x_0,1+C_2(t))$ for all $i\in \iintLigne{0,k}$ (otherwise, this would be in contradiction with the fact that almost surely $X_u \in \msb(X_0,C_2(t))$ for all $u\in[0,t]$). Hence, there exists $C>0$ such that, for all $x\in \msb(x_0,1)$, $k\in\nset$, $i\in \iintLigne{1,k-1}$ and almost every $s\in \Delta_{k,t}$,
%  \[\sup\{|T_{s_i}Q_*f(y)| + \norm{\na T_{s_i}Q_* f(y)},\ y\in E_{i-1}\} \ \leqslant \ C \sup\{|f(y)| + \norm{\na f(y)},\ y\in E_{i}\}\eqsp,\]
%   \[\sup\{|T_{s_k} f(y)| + \norm{\na T_{s_k}  f(y)},\ y\in E_{k-1}\} \ \leqslant \ C \sup\{|f(y)| + \norm{\na f(y)},\ y\in E_{k}\}\eqsp,\]
% and in particular
% \[\norm{\na (T_{s_1} Q_*  \dots  Q_* T_{s_k} f)(x)} \ \leqslant \ C^k ( \|f\|_\infty + \norm{\na f}_\infty) \eqsp.\]
%  Hence, $\bar P_t f$ is $\rmc^1$ on $\msb(x_0,1)$, on which it is equal to $P_t f$, which concludes.
\end{proof}

\begin{assumption}
  \label{ass:compact_sup}
    Let $(P_t)_{t \geq 0}$ be a non-explosive PDMP semi-group with local
    characteristics $(\varphi,\lambda,Q)$. Assume that for all $T \geq 0$, there exists $M \geq 0$ such that for all $x \in \msm$ and $t \in \ccint{0,T}$, $\supp\{P_t(x,\cdot)\} \subset \cball{x}{M}$.
\end{assumption}
\begin{lemma}
  \label{lem:compact_sup}
  Assume \Cref{ass:compact_sup}.
 Then for all $f \in \rmc_c(\msm)$, $T \in \rset_+$, there exists a compact $\msk$ such that  $P_t^{\veps} f (x) = 0$, for all $x \not \in \msk$ and $t \in \ccint{0,T}$.
\end{lemma}
\begin{proof}
Let $f \in \rmc_c(\msm)$, $T \in \rset_+$. Then by assumption, there exist $M_f,M_T \in \rset_+$ such that $\supp(f) \subset \ball{x_0}{M_f}$, $x_0 \in \msm$, and $\supp\{P_t(x,\cdot) \subset \cball{x}{M}$ for all $t \in \ccint{0,T}$, $x \in \msm$. Therefore, we get for all  $x \not \in \cball{x_0}{M_T+M_f+1}$, $P_tf(x) = \int_{\msm}\1_{\cball{x}{M_T}\cap \ball{x_0}{M_f}}(y) f(y) P_t(x,\rmd y) = 0$. Indeed by construction $\cball{x}{M_T}\cap \ball{x_0}{M_f} = \emptyset$ since by the triangle inequality,  $\dist(x,y) \leq M_T$ implies that $\dist(x_0,y) \geq M_f+1$. 
\end{proof}


By \Cref{lem:stab_c1c}, \Cref{lem:compact_sup} and \cite[Proposition 3.3, Chapter 1]{ethier:kurtz:1986}, we obtain the following result. 
\begin{corollary}
\label{coro:core_generator}
  Assume \Cref{ass:stability} and \Cref{ass:compact_sup}. Then, $\rmc^1_c(\msm)$ is a core for the (strong) generator of $(P_t)_{t \geq 0}$. 
\end{corollary}


\begin{definition}
  We say that the PDMP semi-group $(P_t)_{t \geq 0}$ with local  characteristics $( \varphi,\lambda,Q)$ is smoothly and compactly approximable if
  for all $\varepsilon>0$ there exists local characteristics  $( \varphi,\lambda^\varepsilon,Q^\varepsilon)$ satisfying \Cref{ass:stability}-\Cref{ass:compact_sup} and 
\begin{equation}
\label{eq:def_sm_comp_approx}
  \sup_{\substack{x \in \msm\\ \msa \in \mcbb(\msm)}} \defEns{\lambda^\varepsilon (x) \wedge \lambda (x) \abs{  Q^\varepsilon(x,\msa)  -  Q (x,\msa) } + \abs{\lambda^\varepsilon (x) - \lambda (x)} } \leq \veps \eqsp.
\end{equation}
\end{definition}



\begin{proposition}\label{prop:approx-BPS}
  Let $U\in\rmc^2(\rset^d)$, $\rate>0$ and $\loiy\in\mcp(\msv)$ with $\msv \subset \rset^d$ bounded. Then the associated BPS on $\rset^d \times \msv$, given by \Cref{ex:BPS}, is smoothly and compactly  approximable.
\end{proposition}

\begin{proof}
  Let $(\varphi,\lambda,Q)$ be the local characteristics of the BPS given by \Cref{ex:superposition:bps}. Let $\veps > 0$, $\lambda^{\veps}: \msm \to \rset_+$ and $Q^{\veps}$ be  a Markov kernel on $(\rset^d\times \msv,\mcbb(\rset^d\times \msv))$ defined for all $(x,y)\in \rset^d \times \msv$ and $\msa \in \mcbb(\rset^d)$ by
    \begin{equation*}
    \lambda^{\veps}(x,y) = \lambda_1^{\veps}(x,y) + \lambdab \eqsp, \, \lambda_1^{\veps}(x,y) = (\ps{y}{\nabla U(x)}-\veps)^2_+ / (\veps + (\ps{y}{\nabla U(x)}-\veps)_+) \eqsp,
  \end{equation*}
  \begin{equation*}
    Q^{\veps}((x,y),\msa) =    (1/\lambda^{\veps}(x,y))\defEns{\lambda_1^{\veps} \updelta_{(x,\Refl(x,y))}(\msa) + \rate (\updelta_x \otimes \loiy)(\msa)} \eqsp,
  \end{equation*}
  where $\Refl$ is defined by \eqref{eq:def_refl} for $g = \nabla U$. Then, similarly to the BPS process, $(\varphi,\lambda^{\veps},Q^{\veps})$ defines a non-explosive semi-group $(P_t^{\veps})_{t\geq 0}$ on $(\rset^d \times \msv) \times \mcbb (\rset^d \times \msv)$. In addition we have
     \begin{equation}
     \label{eq:bound_distance_lambda_lambda_eps}
    \sup_{x \in \msm } \abs{ \lambda^{(\epsilon)}(x,y) -
    \lambda(x,y) } \leq 2 \epsilon  \eqsp.
   \end{equation}
   Therefore, using \Cref{rem:sync}, we get
   \begin{multline*}
\sup_{\substack{x \in \msm\\ \msa \in \mcbb(\msm)}} \defEns{\lambda^\varepsilon (x) \wedge \lambda (x) \abs{  Q^\varepsilon(x,\msa)  -  Q (x,\msa) } + \abs{\lambda^\varepsilon (x) - \lambda (x)} } \\ \leq 2 \sup_{\substack{x \in \msm\\ \msa \in \mcbb(\msm)}}  \abs{\lambda^\varepsilon (x)   Q^\varepsilon(x,\msa)  -  \lambda (x)  Q (x,\msa) } \leq 4 \veps   \eqsp,
\end{multline*}
which shows \eqref{eq:def_sm_comp_approx}.

Since $\msv$ is assumed to be  bounded, $\msv \subset\cball{0}{M_{\msv}}$, with $M_\msv \in \rset_+$. Therefore by definition,  for all $t \in \rset_+$ and $(x,y) \in \rset^d \times \msv$, we have $P^{\veps}_t((x,y),\cball{x}{t M_\msv} \times \msv) = 1$ and $P^{\veps}_t$ satisfies \Cref{ass:compact_sup}.

Finally, we show that \Cref{ass:stability} is satisfied. \Cref{ass:stability}-\ref{item_3_lem:stab_c1c_b} trivially holds by definition of $\varphi$. 

For all closed ball, $\cball{0}{M} \subset \rset^d$, $M \in \rset_+$, $Q^{\veps}((x,y),\cball{0}{M} \times \msv) = 1$ for all $x \in \cball{0}{M}$. Therefore, for all compact set $\msk \subset \ball{0}{M} \times \msv \subset \rset^d \times \msv$, $M \geq 0$, $T \in \rset_+$, $N \in \nset$, $(t_i)_{i \in \{1,\ldots,N+1\}} \in \rset_+^n$,
$\sum_{i=1}^{N+1} t_i \leq T$, \eqref{def:prop_tmsk} is satisfied for $\tilde{K} = \ball{0}{M+TR} \times \msv$, with  $R = \sup_{y \in \msv} \norm{y}$,
for all $i \in \{1,\ldots,N+1\}$ and $s_i \in \ccint{0,t_i}$ setting
$t_0=0$,  $(\msk_i)_{i \in \{0,\ldots,N\}}$ are given by
\begin{equation*}
  \msk_0 = \ball{0}{M} \times \msv\eqsp, \, \msk_i =  \ball{0}{R_i } \times \msv \eqsp, \, R_i =M+R \sum_{j=0}^i t_j \eqsp,
\end{equation*}
and \eqref{def:msk_i} holds. Thus, $\varphi$ and $Q^{\veps}$ are compactly compatible.

    Then note that for all  $\lambda^{\veps}$ is
  continuously differentiable on $\msm$ since
  $t \mapsto (t-\veps)_+^2/(\veps+(t-\veps)_+)$ is on $\rset$; and its gradient is given for all $x \in \msm$ by
  \begin{equation}
    \label{eq:gradient_lambda_eps}
    \nabla(\lambda^{(\epsilon)})(x,y) =
    \begin{cases}
      \frac{(\ps{y}{\nabla U(x)}-\epsilon)(\ps{y}{\nabla U(x)}+\epsilon)}{\ps{y}{\nabla U(x)}^2} \begin{pmatrix}  \nabla^2 U(x) y , \nabla U(x)
      \end{pmatrix} & \text{ if $\ps{y}{\nabla U(x)} \geq \epsilon$}\\
      0 & \text{ otherwise} \eqsp.
    \end{cases}
  \end{equation}
  In addition, for all continuously differentiable function $f: \rset^d \times \msv \to \rset$,  $(x,y) \in \rset^d \times \msv$, we have
  $    \lambda^{\veps}(x,y)  Q^{\veps}f(x,y) = A_1(x,y) + A_2(x,y)$  where
  \begin{equation*}
    A_1(x,y) = \lambda_1^{\veps}(x,y) f(x,\Refl(x,y)) \eqsp, \, A_2(x,y) =  \rate \int_{\msv} f(x,\tilde y) \loiy(\rmd \tilde y) \eqsp.
  \end{equation*}
  We show that $A_1$ and $A_2$ are continuously differentiable and satisfy for $i=1,2$, for all compact set $\msk \in \rset^d \times \msv$, for all $(x,y) \in \msk$,
  \begin{equation}
    \label{eq:bound_bps_A_1_2} 
    \norm{\diff A_i(x,y)} \leq \sup_{(w,z) \in \msk} \{\Psi_i(w,z)\}\sup\ensemble{\abs{f}(x,\tilde{y}) + \norm{\diff f(x,\tilde{y})}}{y \in \msv}   \eqsp,
  \end{equation}
  where $\Psi_i : \rset^d \times \msv \to \rset_+$, $i=1,2$, are
  bounded on compact sets of $\rset^d \times \msv$. Note that if we
  show \eqref{eq:bound_bps_A_1_2}, since for all
  $(x,y) \in \rset^d \times \msv$,
  $\supp \{Q((x,y),\cdot)\} = \{x\} \times \msv$, this result concludes the proof that \Cref{ass:stability}-\ref{item_2_lem:stab_c1c_b} holds.
  
  First, for all $(x,y) \in \rset^d \times \msv$, $\Refl$ is
  continuously differentiable at $(x,y)$ is
  $\ps{y}{\nabla U(x)} \not =0$. Since $f$, $\lambda_1^{\veps}$ are
  continuously differentiable and $\lambda_1^{\veps}(x,y) = 0$ if
  $\ps{y}{\nabla U(x)} \leq \veps$, $A_1$ is continuously
  differentiable and satisfies for all $(x,y) \in \rset^d \times y$,
  $\ps{y}{\nabla U(x)} \geq \veps$
  \begin{equation}
    \label{eq:bound_bps_A_1}
\norm{\diff A_1(x,y)} \leq  \norm{\diff \lambda_1^{\veps}(x,y)} \abs{f}(x,\Refl(x,y)) + \lambda_1^{\veps}(x,y) (1+\norm{\diff \Refl(x,y)})\norm{\diff f(x,\Refl(x,y))} \eqsp. 
\end{equation}
Regarding $A_2$, we have for all $(x,y) \in \rset^d \times \msv$, since $\diff f$ is bounded on all compact sets of $\rset^d \times \msv$ and the Lebesgue dominated convergence theorem,
\begin{equation*}
\norm{\diff A_2(x,y)} \leq \rate \int_\msv \norm{\diff_x f(x,\tilde y)} \loiy(\tilde y) \leq \rate \sup_{y \in \msv}\norm{\diff f(x,\tilde y)}\eqsp,
\end{equation*}
where $\diff_x$ is the differential operator with respect to the $x$-variable. Combining this result and \eqref{eq:bound_bps_A_1}, we get that \eqref{eq:bound_bps_A_1_2} holds and therefore \Cref{ass:stability}-\ref{item_2_lem:stab_c1c_b} as well.

\end{proof}


\begin{lemma}
  \label{lem:dist_generator}
  Let $(P_t^1)_{t \geq 0}$ and $(P_t^2)_{t \geq 0}$ be  non-explosive PDMP semigroups with local characteristics $(\varphi,\lambda^1,Q^1)$ and $(\varphi,\lambda^2,Q^2)$ respectively. Assume that there exists $\eta \geq 0$, such that 
  \begin{equation*}
    \sup_{\substack{x \in \msm \\ \msa \in \mcbb(\msm) }} \defEns{\lambda^1(x) Q^1(x,\msa) - \lambda^2(x) Q^2(x,\msa)} \leq \eta \eqsp.
  \end{equation*}
 Then for all  $f \in \rmc^1_c(\msm)$,
  \begin{equation*}
    \sup_{x \in \msm} \abs{\generator f(x) - \generator^{\veps} f(x)} \leq \eta \sup_{x \in \msm}\abs{f}(x) \eqsp,
  \end{equation*}
  where $\generator^1$, $\generator^2$ are the (weak) generator of $(P_t^1)_{t \geq 0}$,   $(P_t^{2})_{t \geq 0}$ respectively.
\end{lemma}

\begin{proof}
  Let $\veps >0$ and $f \in \rmc^1_c(\msm)$. 
  Since $\rmc^1_c(\msm)$ belongs to the domain of $\generator^1$ and $\generator^{2}$, we have for all $x \in \msm$ by \eqref{eq:def_generator} and \cite[Section III.1]{dunford:schwartz:1958} \alain{mettre bon label}
  \begin{multline*}
    \abs{\generator^1f(x) - \generator^2f(x)} = \abs{\lambda^1(x) Q^1f(x)-\lambda^2(x) Q^2f(x)} \\\leq  \sup_{x \in \msm} \{\abs{f}(x) \}\sup_{\msa \in \mcb{\msm}} \abs{\lambda^1(x) Q^1(x,\msa)-\lambda^2(x) Q^2(x,\msa)} \leq \eta \sup_{x \in \msm}\abs{f}(x)  \eqsp, 
  \end{multline*}
  which concludes the proof.
\end{proof}

\begin{proposition}\label{lem:critere-invariant}
  Let $(P_t)_{t \geq 0}$ be a non-explosive PDMP semigroup with local characteristics $(\varphi,\lambda,Q)$. Assume that $(P_t)_{t \geq 0}$ is smoothly and compactly approximable and $\int_{\msm} \abs{\lambda} (x) \mu(\rmd x) < \plusinfty$. In addition, assume that the (weak) generator $\generator$ associated with $(P_t)_{t \geq 0}$ satisfies for all $f \in \mrc^1_c(\msm)$,
  \begin{equation}
    \label{eq:critere_inv}
    \int_{\msm} \generator f(x) \mu (\rmd x) = 0 \eqsp.
  \end{equation}
  Then $\mu$ is invariant for $(P_t)_{t \geq 0}$. 
  % Let $\generator$ be the generator of the semigroup $(P_t)_{t\geqslant 0}$ of a homogeneous PDMP with characteristics $( \varphi,(\lambda_i,Q_i)_{i\in \iintLigne{1,n}})$, and let $\mu\in \mcp(\msm)$. Suppose the PDMP is nicely approximable  and $\int_{\msm} \lambda_i \rmd \mu < \infty$ for all $i\in \iintLigne{1,n}$.
%that satisfies
%\begin{eqnarray*}
%\sum_{i=1}^n \int_{\msm} |\lambda_i^\varepsilon - \lambda_i| \rmd \mu & \underset{\varepsilon\rightarrow 0}\longrightarrow & 0\eqsp .
%\end{eqnarray*}
% Suppose moreover that
% \begin{eqnarray*}
% \int_{\msm} \generator f(x) \mu( \rmd x) & = & 0
% \end{eqnarray*}
% for all $f\in \mrc^{1}_c(\msm)$. Then $\mu$ is invariant for $(P_t)_{t\geqslant 0}$.
\end{proposition}

\begin{proof}
Since $\mrc^{1}_c(\msm)$ is dense in $\mrl^\infty(\mu)$, it is sufficient to show that 
\[\int_\msm P_t f (x) \mu(\rmd x) \ = \ \int_\msm   f(x)  \mu(\rmd x) \]
for all $t\geqslant 0$ and $f\in \mrc^{1}_c(\msm)$.
Let $\veps >0$, a PDMP semi-group $(P^{\veps}_s)_{s \geq 0}$ with local characteristics  $(\varphi,\lambda^{\veps}, Q^{\veps})$ satisfying \Cref{ass:stability}-\Cref{ass:compact_sup} and \eqref{eq:def_sm_comp_approx}, and $t \geq 0$ . 
By \Cref{prop:synchrone}, we have for all $x \in \msm$, $\tvnorm{\updelta_x P_t - \updelta_x P^{\veps}_t} \leq 2(1-\rme^{-t \veps})$, therefore we get for all  $f \in \mrc^1_c(\msm)$
\begin{align}
\nonumber
  &   \abs{  \int_{\msm} P_tf(x) \mu(\rmd x)-     \int_{\msm} f(x) \mu(\rmd x)} \leq \abs{\int_{\msm} \defEns{P_t f(x) -P_t^{\veps} f(x)}\mu(\rmd x)} \\
  \nonumber
& \qquad \qquad  \qquad   \qquad \qquad \qquad   \qquad \qquad  +\abs{ \int_{\msm} \{P_t^{\veps} f(x) - f(x) \} \mu(\rmd x)  } \\%[-0.5cm]
  \label{eq:preuve_invariance_bounded_support_1} 
 &      \qquad   \qquad \qquad \qquad   \qquad \qquad  \leq 2(1-
    \rme^{-\veps t}) \sup_{x \in \msm} \abs{f(x)} +\abs{ \int_{\msm} \{ P_t^{\veps} f(x) - f(x) \} \mu(\rmd x)  } \eqsp.
\end{align}

Furthermore, by \Cref{coro:core_generator}, $\mrc^1_c(\msm)$ is a
core for the strong generator associated with $(P_s^{\veps})_{s \geq 0}$. Thus, it belongs to the
domain of the strong generator of $(P_t^{\veps})_{t \geq 0}$ and by Dynkin formula \cite[Proposition 1.5-(c)]{ethier:kurtz:1986}, we get
\begin{equation*}
   \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)=  \int_{\msm} f(x)\mu(\rmd x)- \int_{\msm} \int_0^t \generator^{\veps}P_s^{\veps}f(x) \rmd s\,\mu(\rmd x)\eqsp.
\end{equation*}
Therefore,
\begin{multline}
    \label{eq:preuve_invariance_bounded_support_2}
  \abs{ \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)- \int_{\msm} f(x) \mu(\rmd x) } \\\leq 
  \abs{\int_{\msm} \int_0^t \defEns{\generator^{\veps}-\generator } P_s^{\veps}f(x) \rmd s\mu(\rmd x)} 
 + \abs{\int_{\msm} \int_0^t \generator P_s^{\veps}f(x) \rmd s\, \mu(\rmd x)} \eqsp.
\end{multline}
In addition, by \eqref{eq:lem_stab_clc} in \Cref{lem:stab_c1c}, \Cref{ass:stability}-\ref{item_3_lem:stab_c1c} and \Cref{lem:compact_sup},  $\int_{\msm} \int_0^t \abs{\generator P_s^{\veps}f(x)} \rmd s\mu(\rmd x) < \plusinfty$. Therefore, by  Fubini's theorem and \eqref{eq:critere_inv}, we get  $\int_{\msm} \int_0^t \generator P_s^{\veps}f(x) \rmd s\mu(\rmd x) = 0$. Combining  this result, \eqref{eq:preuve_invariance_bounded_support_2} becomes 
\begin{equation}
    \label{eq:preuve_invariance_bounded_support_2_5}
  \abs{ \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)- \int_{\msm} f(x) \mu(\rmd x) } \leq 
  \abs{\int_{\msm} \int_0^t \defEns{\generator^{\veps}-\generator } P_s^{\veps}f(x) \rmd s\mu(\rmd x)}  \eqsp.
\end{equation}
Note that by \eqref{eq:rem_syn_3}, \eqref{eq:def_sm_comp_approx} and \Cref{lem:dist_generator}, for all  $f \in \mrc^1_c(\msm)$
\begin{equation*}
%  \label{eq:diff_generator_approximation}
\sup_{x \in \msm}\abs{  \generator f(x) -   \generator^{\veps} f(x)} \leq \veps \sup_{x \in \msm} \abs{f(x)} \eqsp. 
\end{equation*}
Using this result in \eqref{eq:preuve_invariance_bounded_support_2_5}, we obtain 
\begin{equation}
\label{eq:preuve_invariance_bounded_support_3}
\abs{ \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)- \int_{\msm} f(x) \mu(\rmd x) } \leq  \veps t \sup_{\substack{x \in \msm\\
  s \in \ccint{0,t}}} \abs{P_s f(x)} \leq \veps t \sup_{x \in \msm} \abs{f}(x) \eqsp. 
\end{equation}

Plugging 
 \eqref{eq:preuve_invariance_bounded_support_3} in \eqref{eq:preuve_invariance_bounded_support_1}, we finally obtain
\begin{equation*}
   \abs{  \int_{\msm} P_tf(x)\mu(\rmd x)-     \int_{\msm} f(x) \mu(\rmd x)} \leq  (2(1-
    \rme^{-\veps t}) +\veps t  )\sup_{x \in \msm} \abs{f(x)} \eqsp.
\end{equation*}
Taking the limit as $\veps$ goes to $0$ concludes the proof. 
\end{proof}

\begin{proposition}\label{prop:invarince-BPS}
  Let $U\in\rmc^2(\rset^d)$, $\rate>0$ and $\loiy\in\mcp(\msv)$ with
  $\msv \subset \rset^d$, and let $(P_t)_{t\geqslant 0}$ be the
  corresponding BPS Markov semi-group, given by \Cref{ex:BPS}. Assume
  that $\loiy$ is rotation invariant,~\ie~for all
  $O \in \rset^{d\times d}$, $O^{\transpose}O = \Id$,
  $\loiy(O \msa) = \loiy(\msa)$, for all $\msa \in\mcbb(\msv)$. In addition, suppose that
\[\int_{\rset^d} ( 1+\norm{\na U(x)} ) e^{-U(x)}\rmd x \ < \ \infty \eqsp,\quad \int_\msv \norm{y} \loiy(\rmd y)\ < \ \infty \eqsp.\]
Then $\tpi = \pi \otimes \loiy$ is invariant for $(P_t)_{t\geqslant 0}$, where $\pi$ is the probability measure on $(\rset^d,\mcbb(\rset^d))$ with density with respect to the Lebesgue measure proportional to $x \mapsto \rme^{-U(x)}$.  
\end{proposition}

\begin{proof}
  Consider first the case where $\msv$ is bounded. Then, by \Cref{prop:approx-BPS}, $(P_t)_{t \geq 0}$ is smoothly and compactly approximable and the other assumptions of \Cref{lem:critere-invariant} are easily checked.  In particular, for all $f\in\mrc^{1}_c(\rset^d\times\msv) $, 
$   \int \generator f(x)  \pi(\rmd x) = 0$
  follows from an integration by parts and because $\msv$ and $\loiy$ is rotation invariant, see e.g. \cite{MonmarcheRTP} for more details.


Consider the conditional distribution associated with $\loiy$ defined for all $\msa \in \mcb{\msv}$, 
\begin{equation}
  \label{eq:loiy_R}
  \mu^{R}(\msa) = \mu(\ball{0}{R}\cap \msa) / \mu(\ball{0}{R}) \eqsp,
\end{equation}
for $R$ large enough such that $\mu(\ball{0}{R}) \not = 0$.  Consider
a BPS semi-group $(P_t^R)_{t \geq 0}$ associated with $U$ and $\mu^R$,
\ie~with local characteristics $(\varphi,\lambda,Q^R)$ with $\varphi$ given by \eqref{eq:transport_libre}, $\lambda$ by \eqref{eq:def_lambda_total_bps} and
$Q^R$ is defined for all $(x,v) \in \rset^d \times \msv$, $\msa \in \mcbb( \rset^d \times \msv)$ by
\begin{equation*}
    Q^R((x,y),\msa)  =  \lambda^{-1}(x,y)\defEns{\ps{\nabla U(x)}{y} \updelta_{(x,\Refl(x,y))}(\msa) + \rate (\updelta_x \otimes \loiy^R)(\msa)} \eqsp. 
\end{equation*}
Note that since $\msv \cap \ball{0}{R}$ is bounded,  $\tilde{\pi}^{R} = \pi \otimes \loiy^R$ is an invariant measure  for $(P_t^R)_{t \geq 0}$. Therefore for
any $f : \rset^{d} \times \msv \to \rset$, bounded and measurable, $t \geq 0$, we
have for all $R \geq 0$ large enough,
\begin{align}
  \nonumber
  & \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}(x,y) - \int_{\rset^{d} \times \msv} f(x,y) \rmd \tilde{\pi}(x,y)} \\
    \nonumber
  &  \qquad \qquad \leq \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}(x,y) - \int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}^{R}(x,y) } \\
    \nonumber
  & \qquad\qquad\qquad+  \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}^{R}(x,y) - \int_{\rset^{d} \times \msv} P_t^{R} f(x,y) \rmd \tilde{\pi}^{R}(x,y) } \\
    \nonumber
  & \qquad\qquad\qquad+ \abs{\int_{\rset^{d} \times \msv}  f(x,y) \rmd \tilde{\pi}^{R}(x,y) - \int_{\rset^{d} \times \msv} f(x,y) \rmd \tilde{\pi}(x,y) } \\
  % \label{eq:invariance_non_bornee_1}
  \nonumber
  & \qquad\qquad \leq 2 \sup_{\rset^d \times \msv}\abs{f}  \mu\parenthese{\rset^{d} \setminus \ball{0}{R}} +   \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}^{R}(x,y) - \int_{\rset^{d} \times \msv} P_t^{R} f(x,y) \rmd \tilde{\pi}^{R}(x,y) } \eqsp.
\end{align}
Since $\lim_{R \to \plusinfty} \mu\parentheseLigne{\rset^{d} \setminus \ball{0}{R}} = 0$, it
remains to show that the last term in the right-hand side goes to $0$
as $R \to \plusinfty$ and the proof will be finished. Besides, note
that this result holds if for $t >0$, we  show that for all
$(x,y) \in \rset^{d} \times \msv$,
\begin{equation}
  \label{eq:invariance_non_bornee_2}
\lim_{R \to \plusinfty}   \tvnorm{ \updelta_{(x,y)} P_t  -  \updelta_{(x,y)} P_t^R } = 0 \eqsp.
\end{equation}
But by \Cref{prop:synchrone} and definition of local characteristics of $(P_s)_{s \geq 0}$ and $(P_s^R)_{s \geq 0}$, we get for all $t \geq 0$, $(x,y) \in \rset^d \times \msv$, 
\begin{equation*}
  \tvnorm{ \updelta_{(x,y)} P_t  -  \updelta_{(x,y)} P_t^R }  \leq 2 (1-\exp(-\rate \mu(\msv \setminus \ball{0}{R}))) \eqsp,
\end{equation*}
which shows that \eqref{eq:invariance_non_bornee_2} holds. 
\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> invariant_keep.tex <==

\section{Regularity estimates for PDMP semigroups}
\label{sec:stab_c1c}

In this section, only homogeneous processes are
considered. Nevertheless, our result can be applied to inhomogeneous
PDMP since if $(X_t)_{t\geq 0}$ is such a process on $\msm$ with
characteristics $(\varphi,Q,\lambda)$, then the process
$(X_t,t)_{t \geq 0}$ is a homogeneous PDMP on
$(\msm \times \rset_+, \mcbb(\msm \times \rset_+))$ with
characteristics $(\bar{\varphi},\bar{Q},\lambda)$
defined for all $t,s \in \rset_+$, $x \in \msm$ and $\msa \in \mcbb(\msm \times \rset_+)$ by
\begin{equation*}
  \bar{\varphi}_{s}((x,t)) = (\varphi_{t,t+s}(x),t+s)  \eqsp, \qquad \qquad \bar{Q}((x,t),\msa) = \int_{\msm\times \rset_+} \1_{\msa}((y,u))  Q(x,\rmd y) \otimes \updelta_t(\rmd u) \eqsp.
\end{equation*}

For our next result, we need the following definition.
\begin{definition}
We say that a
differential flow $\varphi$ on $\msm$ and a Markov kernel $Q$ are
compactly compatible if for all compact set $\msk \subset \msm$ and $T \geq 0$,
there exists a compact set $\tilde \msk \subset \msm$ satisfying for
all $N \in \nset$, $(t_i)_{i \in \{1,\ldots,N+1\}} \in \rset_+^n$,
$\sum_{i=1}^{N+1} t_i \leq T$,
there exists a sequence $(\msk_i)_{i \in \{0,\ldots,N\}}$ of
compact sets of $\msm$ such that
\begin{equation}
  \label{def:msk_i}
\msk \subset \msk_0 \text{  and for all $i\in \{0,\ldots,N-1\}$, } \bigcup_{x \in \msk_i} \supp \{ Q(\varphi_{t_{i+1}}(x),\cdot) \} \subset
\msk_{i+1} \eqsp,
\end{equation}

and
\begin{equation}
\label{def:prop_tmsk}
\cup_{i=0}^{N} \msk_i \subset \tilde \msk \eqsp, \text{ and } \varphi_{s_i}( \msk_{i-1}) \subset \tilde \msk  \eqsp,
\end{equation}
for all $i \in \{1,\ldots,N+1\}$ and $s_i \in \ccint{0,t_i}$ setting
$t_0=0$.
\end{definition}
Note that by definition, if $\varphi$ and $Q$ are compactly compatible
and the PDMP semigroup with  characteristics $(\varphi, \lambda,Q)$ is
non explosive, for all $t \geq 0$ and all
compact set $\msk \subset \msm$, there exists a compact set
$\tilde \msk \subset \msm$, such that
$\PP (X_s \in \tilde{\msk}, \text{ for all $s \in \ccint{0,t}$} ) =1$,
where $(X_t)_{t \geq 0}$ is a PDMP process with  characteristics $(\varphi, \lambda,Q)$.

\begin{assumption}
  \label{ass:stability}
The  characteristics $(\varphi,\lambda,Q)$ satisfy
\begin{enumerate}[label = (\roman*)]
\item \label{item_1_lem:stab_c1c} the flow  $\varphi$ and the Markov kernel $Q$ are compactly compatible;
\item \label{item_2_lem:stab_c1c} $\lambda\in\mrc^{1}(\msm)$ and for
  all $f \in \mrc^1(\msm)$, $\lambda Qf \in \mrc^1(\msm)$ and there
  exists a function $\Psi :\msm \to \rset_+$ such that for all compact set $\msk \subset \msm$, $\sup_{y \in \msk} \Psi(y) < \plusinfty$ and for all 
  $x \in \msk$,
  \begin{equation*}
    \label{eq:1}
 \norm{\diff (\lambda Qf)(x)} \leq   \sup_{y \in \msk}\{ \Psi(y) \} \sup \ensemble{\abs{f(y)} + \norm{\diff f(y)}}{y \in \supp \{Q(x,\cdot)\}};
  \end{equation*}
\item \label{item_3_lem:stab_c1c} for all compact $\msk \subset \msm$, 
  \begin{equation*}
    \sup \ensemble{\norm{\diff \varphi_s(x)}}{s \in \ccint{0,t}, x \in \msk} < \plusinfty \eqsp.
  \end{equation*}
\end{enumerate}  
\end{assumption}
\begin{lemma}
  \label{lem:stab_c1c}
  Let $(P_t)_{t\geqslant 0}$ be a non explosive PDMP semigroup on $\msm$ with corresponding characteristics $(\varphi,\lambda,Q)$ satisfying \Cref{ass:stability}. 
  Then for all $f \in \mrc^1(\msm)$, $T \in \rset_+$, $P_Tf \in \mrc^1(\msm)$  and for all compact set $\msk \subset \msm$, there exists $C \geq  0$  such that for all $t \in \ccint{0,T}$,
  \begin{equation}
    \label{eq:lem_stab_clc}
  \sup_{x \in \msk}\{ \abs{P_t f}(x) + \norm{\diff (P_tf)(x)}\} \leq C \eqsp.  
  \end{equation}
%   In particular $\mrc^1(\msm)$ is a  core for $(P_t)_{t \geq 0}$. 
% that  and $(x,t)\in\msm\times\rset_+ \mapsto \norm{\na \varphi_t (x)}$ is locally bounded, and that there exist locally bounded functions $C_1:\msm \rightarrow \rset_+$ and $C_2:\rset_+\rightarrow \rset_+$  such that for all $f\in \rmc^1_c(\msm)$, $\lambda Qf\in \rmc^1_c(\msm)$ and for all $x\in\msm$, 
% \[\norm{\na (\lambda Q f)(x)}\ \leqslant  \ C_1(x)\sup\{|f(y)| + \norm{\na f(y)},\ y\in \supp Q(x,\cdot)\}\eqsp,\]
%  and for all $t\geqslant 0$,  $X_s \in \msb(X_0,C_2(t))$ for all $s\in[0,t]$ almost surely. Then, if $f\in \mrc^1_c(\msm)$, $ P_t f\in \mrc^1_c(\msm)$ for all $t \geq 0$. %Therefore, $\mrc^1_c(\msm)$ is a core for $(P_t)_{t \geq 0}$.
 
 
% More precisely, if $f\in \mrc^1_c(\msm)$ and $t\geqslant0$, then there exist $C>0$ and a compact $\msk$ of $\msm$  such that,  for all $s\in [0,t]$, the support of $P_s f$ is included in $\msk$ and  $\norm{\na P_s f}_\infty \leqslant C$.
\end{lemma}
% \begin{remark}
%   Note that in the case where the condition $\inf_{x \in \msm} \lambda(x) >0$ is not satisfied, we can simply consider a modified characteristics $(\varphi,\bar \lambda, \bar Q)$ which defines the same PDMP semigroup $(P_t)_{t \geq 0}$ where $\bar Q$ and $\bar \lambda$ are given for all $x \in \msm$ and $\msa \in \mcb{\msm}$ by
%   \begin{equation*}
%     \bar \lambda(x) = \lambda(x) + \rate \eqsp, \, \bar Q(x,\msa) = \bar \lambda^{-1}(x)\lambda(x) Q(x,\msa) + \parenthese{1-\bar \lambda^{-1}(x)\lambda(x)} \updelta_x(\msa) \eqsp,
%   \end{equation*}
%   for $\rate >0$. Then, if the other conditions of \Cref{lem:stab_c1c} are satisfied, the modified characteristics $(\varphi,\bar \lambda, \bar Q)$ satisfy these conditions as well and $\inf_{x \in \msm} \bar \lambda(x) \geq \rate$. 
% \end{remark}
\begin{proof}
 
For all $x \in \msm$
  denote by $(X_t^x)_{t \geq 0}$ a PDMP starting from $x$ associated
  with the characteristics $(\varphi,\lambda,Q)$ and defined by \Cref{const:1}.  Let
  $(S_n^x)_{n \in \nset}$ be the jump times of $(X_t^x)_{t \geq 0}$
  for all $x \in \msm$ and $(\mcf_t)_{t \geq 0}$ the associated filtration. Let $f\in \mrc^1(\msm) $, $T\geqslant 0$ and a
  compact set $\msk \subset \msm$. For $T =0$, the result is
  straightforward so we consider $T >0$. Let $\tilde \msk$ satisfying for all $n \in \nset$,
$(t_i)_{i \in \{1,\ldots,n+1\}} \in \rset_+^n$,
$\sum_{i=1}^{n+1} t_i \leq T$, \eqref{def:prop_tmsk}.
% $\cup_{i=0}^{n} \msk_i \subset \tilde \msk$,
% $\varphi_{s_i}( \msk_{i-1}) \subset \tilde \msk$, for all
% $i \in \{1,\ldots,n+1\}$ and $s_i \in \ccint{0,t_i}$ setting
% $t_0=0$, where $(\msk_i)_{i \in \{0,\ldots,n\}}$ are given by \eqref{def:msk_i}. 

Since for all $x  \in \msk$, 
  $\PP (X_t^x \in \tilde \msk, \text{ for all } t \in \ccint{0,T}) = 1$,
  for all $t \in \ccint{0,T}$ and $x \in \msm$,
  \begin{equation}
    \label{eq:core_proof_1}
    \abs{P_tf(x)} = \abs{\expe{f(X_t)}} \leq \sup_{y \in \tilde \msk} \abs{f}(y) \eqsp.
  \end{equation}
  
Furthermore,  $(P_t)_{t \geq 0}$
  is assumed to be non explosive. Therefore
  $\sup_{n \in \nset} \S^{x}_n = \plusinfty$ and we can consider the
  following decomposition for all $t \in \ccint{0,T}$ and $x \in \msk$
  \begin{equation}
    \label{eq:decomposition_regular_pDMP}
  P_tf(x)  = \sum_{n=0}^{\plusinfty} \expeMarkov{}{\1_{\coint{S^{x}_n,S^{x}_{n+1}}}(t) f(X^{x}_t)} \eqsp.
\end{equation}
We  show that for all $n \in \nset$,
  \begin{equation}
    \label{eq:def_F_n}
   F_{n,t} : x \mapsto
  \expeMarkov{}{\1_{\cointLigne{S^{x}_n,S^{x}_{n+1}}}(t)
    f(X^{x}_t)}  \eqsp,
  \end{equation}
 is continuously
  differentiable and in addition there exists $C \geq 0$ such that for all
  $n \in \nset$, $t \in \ccint{0,T}$
  \begin{equation}
    \label{eq:estimate_gradient_n}
\sup_{x \in \msk}   \norm{ \diff  F_{n,t} (x)} \leq C^n  /n!\eqsp.%       \expeMarkov{(x,y)}{\1_{\coint{\bS_n^{\epsilon},\bS_n^{\epsilon}}}(t) } \eqsp,
   \end{equation}
   %where $(\bS_n^{\epsilon})_{n \in \nset}$ are the event times of a Poisson process with constant jump rate $\rate$.
   Assume for the moment that this result holds. Then, we have for all $t \in \ccint{0,T}$,
    \begin{equation*}
      \lim_{N \to \plusinfty}   \sum_{n=N}^{\infty} \sup_{x \in \msk}  \norm{ \diff F_{n,t}(x) } = 0 \eqsp. 
    \end{equation*}
    By \eqref{eq:decomposition_regular_pDMP}, it implies that
    $x \mapsto P_T f(x)$ is continuously differentiable. In
    addition, for all compact set $\msk \subset\msm$, there exists $C \geq 0$ such that for all $t \in \ccint{0,T}$, $ \norm{\diff P_tf(x)}_{\msk} \leq C $.
 %    \begin{equation*}
 %        \label{eq:core_proof_0}
 % \norm{\diff P_tf(x)}_{\msk} \leq C \eqsp.
 %    \end{equation*}
This result and \eqref{eq:core_proof_1} imply \eqref{eq:lem_stab_clc}.
  
    We now turn in showing that for all $n \in \nset$, $F_n$ is
    continuously differentiable and \eqref{eq:estimate_gradient_n}
    holds. We first show this result for $n = 0$. In a second time, we
    make an induction on $n \in \nsets$. 

For all $x \in \msk$ and $t \in \ccint{0,T}$, we have
    \begin{equation*}
      F_{0,t}(x) =  f(\phi_t(x)) \exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \eqsp. 
    \end{equation*}
Therefore, for all $x\in \msk$ and $t \in \ccint{0,T}$, we obtain by \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c}
    \begin{multline*}
      \diff F_{0,t}(x) = \defEns{\diff f (\phi_t(x))} \diff (\phi_t)(x) \exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \\
+        f(\phi_t(x))   \parentheseDeux{\int_0 ^t \defEns{\diff  \lambda (\phi_s(x)) \cdot \diff(\phi_s)(x) }\rmd s}\exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \eqsp.
\end{multline*}
Since for all $x \in \msk$ and $t \in \ccint{0,T}$, $\varphi_t(x) \in \tilde \msk$, $f \in \mrc^1(\msm)$ and using \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c}, we get there exists $C_0 \geq 0$ such that for all $t \in \ccint{0,T}$,
\begin{equation*}
\sup_{x \in \msk} [     \abs{F_0(x)}+    \norm{\diff F_0(x)}  ]\leq C_0 \eqsp.
    \end{equation*}
%    where we have used that for all $x \in \msm$, $\lambda(x) \geq \rate$.

We now show the result for $n \in \nsets$. We give first an explicit expression of $F_n$ for all $n \in \nsets$. Indeed, we have conditioning successively on $\mcf_{S_{n+1}^x}, \cdots, \mcf_{S_1^x}$, for all $x \in \msk$ and $t \in \ccint{0,T}$
\begin{multline}
  \label{eq:forme_loimarkov_chain}
  % \expeMarkov{(x,y)}{\1_{\coint{S^{(\epsilon)}_n,S^{(\epsilon)}_{n+1}}}(t) f(X^{(\epsilon)}_t,Y^{(\epsilon)}_t)}
  F_{n,t}(x)  = \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
  \int_0^{t-t_1} \rmd t_2 \exp\parenthese{-\int_0^{t_2} \lambda\defEns{\phi_{s_2}(x_1)} \rmd s_2}  \int_{\msm } \opK(\phi_{t_2}(x_1),\rmd x_2) \\
  \cdots   \int_0^{t-\sum_{i=1}^{n-1}t_i} \rmd t_n \exp\parenthese{-\int_0^{t_n} \lambda\defEns{\phi_{s_n}(x_{n-1})} \rmd s_n} \\
  \int_{\msm } \opK(\phi_{t_n}(x_{n-1}),\rmd x_n) f(\phi_{t-\sum_{i=1}^n t_i} (x_n))   \\  \exp\parenthese{-\int_0^{t-\sum_{i=1}^n t_i} \lambda\defEns{\phi_{s_{n+1}}(x_{n})} \rmd s_{n+1}} \eqsp,
\end{multline}
where $\opK$ is the kernel defined on $(\msm, \mcb{\msm})$  for all $x \in \msm$ and $\msa \in \mcb{\msm}$ by
  \begin{equation*}
    \opK(x,\msa) = \lambda(x) Q(x,\msa)  \eqsp.
  \end{equation*}

%   For the case $n=1$, we get for all $x \in \msk$ and $t \in \ccint{0,T}$,
%   \begin{multline}
%     \label{eq:first_estimate_gradient} 
%     F_{1,t}(x) =
%     \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1}  \lambda\defEns{\phi_{s_1}(x)} \rmd s_1}    \\
%       \times\left\lbrace \int_{\msm}  \lambda\parenthese{\phi_{t_1}(x)} Q(\phi_{t_1}(x),\rmd x_1) f\parenthese{\phi_{t-t_1}(x_1)} \exp\parenthese{-\int_0^{t-t_1} \lambda\defEns{\phi_{s_{2}}(x_1)} \rmd s_{2}} \right \rbrace
%   \eqsp.
% \end{multline}
% Since $f \in \mrc^1(\msm)$ and by \ref{item_1_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
% \begin{equation*}
%   x_1 \mapsto g(t_1,x_1) =  f\parenthese{\phi_{t-t_1}(x_1)} \exp\parenthese{-\int_0^{t-t_1} \lambda\defEns{\phi_{s_{2}}(x_1)} \rmd s_{2}} \eqsp,
% \end{equation*}
% is continuously differentiable for $t \in \ccint{0,T}, t_1 \in \ccint{0,t}$. In addition, for all $t \in \ccint{0,T}, t_1 \in \ccint{0,t}$ and for all $x_1 \in \supp \{Q(\varphi_{t_1}(x),\cdot)\}$, by \eqref{def:prop_tmsk}-\eqref{def:msk_i} $\varphi_{s_1}(x_1) \in\tilde K$ for all $s_1\in\ccint{0,t-t_1}$ and therefore
% \begin{equation*}
%   \abs{g}(t_1,x_1)  + \norm{\diff_x g(t_1,x_1)} < 2 \defEnsLigne{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{\diff \lambda }  \sup_{s \in \ccint{0,T}, y \in  \tmsk} \norm{\diff \varphi_{s}(y)}}\rme^{-\rate(t-t_1)} \eqsp.
% \end{equation*}
% Then by \ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
% $x \mapsto \lambda Qg(t_1,\varphi_{t_1}(x))$ is continuously differentiable for all
% $t \in \ccint{0,T}$, $t_1 \in \ccint{0,t}$ and for all $x \in \msk$,
% \begin{multline*}
%   \abs{\lambda Qg(t_1,\varphi_{t_1}(x))}  + \norm{\diff_x \lambda Qg(t_1,\varphi_{t_1}(x))}\\
%   \leq   4  \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}^2\rme^{-\rate(t-t_1)} \eqsp.
% \end{multline*}
%  In addition, since $\varphi_{t_1}(x) \subset \tilde \msk$, for all $t_1 \in \ccint{0,t}$, $t\in\ccint{0,T}$ and $x\in \msk$, by \ref{item_2_lem:stab_c1c}, we have
% \begin{multline*}
%   \sup_{x \in \msk} [\abs{F_1(x)} + \norm{\diff F_1(x) }] \\
%   \leq   8  \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}^3  t  \rme^{-\rate t} \eqsp.
% \end{multline*}

 We introduce a sequence of operator
$( Q^{(n)})_{n \in \nset^*}$, defined for all
$g : \rset_+ \times \msm \to \rset$, bounded on all compact of
$\ccint{0,T} \times \msm$ and measurable, $t \in \ccint{0,T}$ and
$x \in \msm$ by
  \begin{multline}
\label{eq:def_q_n}
    Q^{(n)} g (t,x) = \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
    \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n  \exp\parenthese{-\int_0^{t_n} \lambda\defEns{\phi_{s_n}(x_{n-1})} \rmd s_n} \\\int_{\msm } \opK(\phi_{t_n}(x_{n-1}),\rmd x_n) g(t-\sum_{i=1}^n t_i ,x_n) \eqsp.
  \end{multline}
  Taking for $g$ the function
  $g_F : (s,y) \mapsto f(\varphi_s(y)) \exp(-\int_0^s \rmd u
  \lambda(\varphi_u(y)))$, we have $F_{n,t} = Q^{(n)} g_F(t,\cdot)$. Since
  $f \in \mrc^1(\msm)$ and by \Cref{ass:stability}-\ref{item_3_lem:stab_c1c}, $g_F$ is
  measurable, for all $s \in \ccint{0,T}$, $y \mapsto g_F(s,y)$ is
  differentiable on $\msm$ and satisfies for all $T' \in \ccint{0,T}$,
  $\msk' \subset \msm$ compact,
  $\sup_{s \in \ccint{0,T'}, y \in \msk'} \{\abs{g_F(s,y)} +
  \norm{\diff_x g_F(s,y)}\} < \plusinfty$. Therefore if we show that for
  all measurable function $g :\rset_+ \times \msm \to \rset_+$ such
  that for all $s \in \ccint{0,T}$, $y \mapsto g(s,y)$ is differentiable
  on $\msm$ satisfying for all $T' \in \ccint{0,T}$, $\msk' \subset \msm$
  compact,
  $\sup_{s \in \ccint{0,T'}, y \in \msk'} \abs{g(s,y)} +
  \norm{\diff_x g(s,y)} < \plusinfty$: 1) for all
  $t \in \ccint{0,T}$ and $x \in \msk$, $x \mapsto Q^{(n)} g(t,x)$ is differentiable at $x$ 2) there exists $C \geq 0$ such that for all $n \in \nsets$,
  $x \in \msk$ and $t \in \ccint{0,T}$,
  \begin{equation}
    \label{eq:objectif_g}
    \abs{Q^{(n)} g(t,x)} + \norm{\diff_x Q^{(n)} g(t,x)} \leq C^n/(n!) \eqsp,
  \end{equation}
then \eqref{eq:estimate_gradient_n} holds which will conclude the proof. Denote by $\mrgD$ the set of function $g$ satisfying the assumptions above. 

  Note the following relation between $Q^{(n-1)}$ and $Q^{(1)}$ which will be essential in our next reasonings: for all
$g : \rset_+ \times \msm \to \rset$, bounded on all compact of
$\rset_+ \times \msm$ and measurable, $t \in \ccint{0,T}$ and
$x \in \msm$ 
  \begin{multline}
\label{eq:q_n_prop_q_1}
    Q^{(n)} g (t,x) = \int_{0}^t \rmd t_1  \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) Q^{n-1}g(t-t_1,x_1) \\
    = Q^{(1)} g_{n-1}(t,x)\eqsp,
  \end{multline}
where $g_{n-1}(s,y) = Q^{n-1}g(s,y)$ for all $s \in \rset_+$ and $y \in \msm$.
  
First, we make an induction on $i \in \{1,\ldots,n\}$ to show that for
all  $i \in \{1,\ldots,n\}$ and
$g \in \mrg$, that $(s,x) \mapsto Q^{(i)} g(s,x) \in \mrgD$. For $i =1$, note that for all $s \in \ccint{0,T}$ and $y \in \msm$,
  \begin{equation}
  \label{eq:def_q_1}
    Q^{(1)}g(s,y) = \int_0^s \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(y)} \rmd s_1}  \int_{\msm } \opK(\phi_{t_1}(y),\rmd y_1) g(s-t_1 ,y_1) \eqsp.
  \end{equation}
  Let $T' \in \ccint{0,T}$, $\msk' \subset \msm$ be compact and $\tilde \msk'$ satisfying \eqref{def:prop_tmsk} associated with
  $\msk'$. Then for all $s \in \ccint{0,T'}$, $t_1\in\ccint{0,s}$, $\varphi_{t_1}(y) \in \tilde \msk '$ for all $y \in \msk'$. Therefore we have 
 by assumption on $g$, \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
  $y \mapsto  \int_{\msm } \opK(\phi_{t_1}(y),\rmd y_1) g(s-t_1 ,y_1)$ for all $s \in \ccint{0,T'}$, $t_1 \in \ccint{0,s}$, is differentiable and there exists $C \geq 0$ such that for all $s \in \ccint{0,T'}$, $t_1 \in \ccint{0,s}$
  \begin{equation*}
    \sup_{y \in \msk'} \defEns{ \abs{\opK g(s-t_1 \cdot)(\phi_{t_1}(y))} + \norm{\diff_x  \opK g(s-t_1 \cdot)(\phi_{t_1}(y))}} < C \eqsp
  \end{equation*}
  By \eqref{eq:def_q_1}, we get then the result for $i=1$. The result for $i \in \{2,\ldots,n\}$ is then a straightforward consequence of \eqref{eq:q_n_prop_q_1} and the case $i=1$.

  We now show that for all $g \in \mrgD$ that  there exists $C \geq 0$ such that for all
  $x \in \msk$ and $t \in \ccint{0,T}$, \eqref{eq:objectif_g}
  holds. % Note that for all $j \in \{1,\ldots,n-1\}$, by \eqref{eq:def_q_n} we have for all
  % $s \in \rset_+$ and $x \in \msm$,
  % \begin{multline*}
  %   Q^n_tg(x) =  \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
  %   \cdots \int_{\msm } \opK(\phi_{t_{j}}(x_{j-1}),\rmd x_j)  Q_{t-\sum_{i=1}^{j} t_i}^{n-j} g(x_j) \eqsp.
  % \end{multline*}
  By an induction on $N \in \{1,\ldots,n\}$, we show that  for all
  $N \in \{1,\ldots,n\}$, for all $t \in \ccint{0,T}$,
  $(t_i)_{i \in \{1,\ldots,n-N\}} \in \rset_+^{n-N}$, $\sum_{j=1}^{n-N} t_j \leq t$
  \begin{multline*}
    \sup_{x_{n-N} \in \msk_{n-N}} \abs{Q^N g\parenthese{t-\sum_{j=1}^{n-N}t_j,x_{n-N}} } + \norm{\diff Q^N g\parenthese{t-\sum_{j=1}^{n-N}t_j,x_{n-N}} } \\
    \leq C^{N}_1 \defEns{\sup_{s \in \ccint{0,T}, y \in \tmsk} \abs{g(s,y)} +\sup_{s \in \ccint{0,T}, y \in \tmsk} \norm{\diff_x g(s,y)} }   \left. \parenthese{t-\sum_{j=1}^{n-N}t_j}^N \middle /(N!) \right .\eqsp,
  \end{multline*}
  where $(\msk_j)_{j \in \{1,\ldots,n-N\}}$ are defined by \eqref{def:msk_i} relatively to $\msk$ and $\tmsk$ and
  \begin{equation*}
    C_1 = \norm{\lambda}_{\infty,\tmsk} + \sup_{s \in \ccint{0,T}} \norm{\diff_x \varphi_s(x)}_{\infty, \tmsk} (T \norm{\diff \lambda}_{\infty,\tmsk} + \norm{\Psi}_{\infty,\tmsk}) \eqsp.
  \end{equation*}

  For $N=1$, the result is straightforward from \eqref{eq:def_q_1} and \Cref{ass:stability}. Now assume that the result holds for $N \in \{1,\ldots,n-1\}$ and let $(t_i)_{i \in \{1,\ldots,n-N-1\}} \in \rset_+^{n-N-1}$.

  Then first by \eqref{eq:q_n_prop_q_1} and \Cref{ass:stability}, we have for all $x \in \msk_{n-N-1}$,
  \begin{equation*}
      Q^{(N)} g (t-\sum_{j=1}^{n-N-1}t_j,x) \leq \norm{\lambda}_{\infty,\tmsk}  \int_{0}^t \rmd t_1  \int_{\msm } \sup\defEns{ Q^{n-1}g(t-t_1,x_1) \, : \, x_1 \in \supp(\opK(\phi_{t_1}(x), x_1)) \eqsp.
      \end{equation*}
      Using the induction hypothesis and \Cref{ass:stability} again, we get 
      
  \begin{equation*}
      Q^{(N)} g (t-\sum_{j=1}^{n-N-1}t_j,x) \leq C_1^N \norm{\lambda}_{\infty,\tmsk}  \parenthese{t-\sum_{j=1}^{n-N-1}t_j}^{N+1} \middle /((N+1)!) \eqsp.
      \end{equation*}

%   Indeed, let
%   $x \in \msm$, $t \in \ccint{0,T}$ and
%   $g : \rset_+ \times \msm \to \rset$, bounded on all compact of
%   $\rset_+ \times \msm$, measurable, $y \mapsto g(s,y)$ is
%   continuously differentiable on $msm$, for all $s \in \rset_+$, Since
%   for all $y \in \msm$,

%   Then, an easy induction implies
%   by \eqref{def:prop_tmsk} that for all $i \in \{2,\ldots,n\}$,
%   $(t_j)_{i \in \{1,\ldots,i-1\}} \in \rset_+^n$,
%   $\sum_{j=1}^{i-1} t_j \leq t$, there exists
%   $(\msk_j)_{j \in \{1,\ldots,i-1\}}$ satisfying \eqref{def:msk_i} and
%   \begin{multline*}
%     \sup_{x_i \in \msk_i}      \abs{Q^{(i)}_{t-\sum_{j=1}^{i-1}t_j} g (x_i) } + \norm{\diff_x Q^{(i)}_{t-\sum_{j=1}^{i-1}t_j} g (x_i)}
%     \leq \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}
%   \end{multline*}
%   Note that using the same reasoning as for $F_1$, we get that for all
%   functions
%   $(u,x) \in \rset_+ \times \msm \mapsto g(u,x) \in \rset$,
%    measurable, continuously differentiable with respect to $x$, for all $u >0$, $x \mapsto Q^{(1)}_u g(x,y)$ is continuously differentiable. In addition, for all   $u \in \ccint{0,t}$, there exists $C \geq 0$ such that 

%   \begin{multline}
%     \label{eq:estimate_nabla_G_1}
% \sup_{x \in \msk}      \abs{Q^{(1)}_t g(x)} + \norm{\nabla Q^{(1)}_t g(x)} \\\leq C  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \defEns{
%       \sup_{\substack{x \in \msk}} \abs{g}(t-t_1,x) +  \sup_{\substack{x \in \msk}} \norm{\diff_{x}g}(t-t_1,x)} \eqsp.
%   \end{multline}

%   By an easy induction using that for all $t \geq 0$,
%   $g : \rset_+ \times \msm \to \rset$, bounded and measurable, $x \in \msm$
%   and $n \in \nsets$, $n >1$,
%   \begin{equation*}
%      Q^{(n)}_t g (x,y) =      Q^{(1)}_t [\tilde{g}_t] (x,y)  \eqsp, \quad \text{with }  \tilde{g} (t_1,w,z) = Q^{(n-1)}_{t_1} g (w,z) \eqsp,
%    \end{equation*}
%    for all $t_1 \in \ccint{0,t}$ and \eqref{eq:estimate_nabla_G_1}, we
%    have that for all functions
%    $(t,x,y) \rset_+ \times \msm \mapsto g(t,x,y) \in \rset$,
%    bounded and measurable, differentiable with respect to the space
%    variables $(x,y)$, for all $t >0$ and $n \in \nsets$,
%    $(x,y) \mapsto Q^{(n)}_t g(x,y)$ is continuously differentiable. In
%    addition, for all $R \geq 0$, $n \in \nsets$ and $T >0$, there
%    exists $C \geq 0$ such that for all $t \in \ccint{0,T}$,
%    $x \in \msm$, $\norm{x} + \norm{y} \leq R$,
%   \begin{multline*}
%     \label{eq:estimate_nabla_G_n}
%      \abs{Q^{(n)}_t g(x,y)} + \norm{ \nabla Q^{(n)}_t g(x,y)} \leq C^n  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n \rme^{-\rate t_n }  \\\defEns{
%        \sup_{\substack{x \in \msm\\ \norm{x} + (1+t) \norm{y} \leq R}} \abs{g}\parenthese{t-\sum_{i=1}^n t_i,x,y} +     \sup_{\substack{x \in \msm\\ \norm{x} + (1+t) \norm{y} \leq R}}  \norm{\nabla_{x,y}g}\parenthese{t-\sum_{i=1}^n t_i,x,y}} \eqsp.
%   \end{multline*}

%   Applying this result to the function
%   \begin{equation*}
%   (t,x,y) \mapsto     f(\phi_{t} (x_n,y_n))     \exp\parenthese{-\int_0^{t} \lambda\defEns{\phi_{s_{n+1}}(x_{n},y_{n})} \rmd s_{n+1}} \eqsp,
%   \end{equation*}
%   and using \eqref{eq:def_F_n}, we get that for all $n \in \nsets$,
%   $F_n$ is continuously differentiable. In addition, using that for
%   all $(z,w) \in \msm$, $\lambda(z,w) \geq \rate$, we
%   get for all $R \geq 0$, $n \in \nsets$ and $T >0$, there exists
%   $C \geq 0$ such that for all $t \in \ccint{0,T}$,
%   $x \in \msm$, $\norm{x} + \norm{y} \leq R$,
%   \begin{align*}
%     \label{eq:estimate_nabla_F_n}
%     &\abs{F_n(x,y)} + \norm{ \nabla F_n(x,y)} \\
%     &\qquad     \qquad  \leq C^n  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n \rme^{-\rate t_n }  \rme^{-(t-\sum_{i=1}^n t_i)\rate} \defEns{ \norm{f}_\infty + \norm{\nabla f}_\infty}  \\
%     &\qquad     \qquad   \leq  C^n \rme^{-t \rate } \int_0^t \rmd t_1  \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n   \defEns{ \norm{f}_\infty + \norm{\nabla f}_\infty}\eqsp,
%   \end{align*}
%   which shows that \eqref{eq:estimate_gradient_n} holds and concludes the proof. 
  

%   For all $s\in[0,t]$, we have by \eqref{item_4_lem:stab_c1c} for all $x \in \msm$,
%   \begin{equation*}
%    P_s f(x) = \int_{\msm} \1_{\msk_{x,t}}(y) f(y) P_s(x,\rmd y)   \eqsp.
%  \end{equation*}
%  Therefore $P_sf(x) = 0$ for all $x \in \msm$, 
%   $P_s f(x) = 0$ for all $x$ with $dist(x,\supp f) > \sup\{C_2(s),\ s\in[0,t]\}$. In particular, $P_t f$ is compactly supported. For any $x_0 \in \msm$, let us prove that $P_t f$ is $\rmc^1$ on $\msb(x_0,1)$. Let $\lambda_* = 1+ \sup\{\lambda(x),\ x\in\msb(x_0,1+C_2(t))\}$, and $(\bar P_t)_{t\geqslant 0}$ be the PDMP semigroup with characteristics $( \varphi,\lambda_*,Q_*)_{i\in \iintLigne{1,n}})$ with for all $x\in\msm$,
% \[Q_*(x,\cdot) \ = \  \frac{1 - (\lambda(x)\wedge \lambda_*)}{\lambda_*} \delta_x(\cdot) +  \frac{\lambda(x)\wedge \lambda_*}{\lambda_*} Q(x,\cdot) \eqsp.\]
% Then, for all $x\in \msb(x_0,1)$, $\bar P_t f(x) = P_t f(x)$.

%  Conditioning by the jump times of the process (which are jump times of an homogeneous Poisson process with intensity $\lambda_*$),
%  \begin{eqnarray*}
%  \bar P_t f(x) & = & \sum_{k\in\nset} \frac{(\lambda_* t)^k}{k!}\int_{\Delta_{k,t}} T_{s_1} Q_* T_{s_2} \dots Q_* T_{s_{k-1}} Q_* T_{s_k} f(x) \rmd s_1,\dots,\rmd s_k
%  \end{eqnarray*}
%  where, for $k\in\nset$, $\Delta_{k,t} = \{s\in \rset_+^k, \sum_{i=1}^k s_i = t\}$ and $T_r f(x) = f( \varphi_r(x))$. For a given $x\in \msb(x_0,1)$, $k\in\nset$ and $s\in \Delta_{k,t}$, let $E_0=\{x\}$, $E_{i} = \cup\{ \supp Q_*( \varphi_{s_i}(y),\cdot),\ y\in E_{i-1}\}$ for $i\in \iintLigne{1,k-1}$ and $E_k = \cup\{ \varphi_{s_k}(y),\ y\in E_{k-1}\}$. By assumption, for almost every $s\in \Delta_{k,t}$, $E_i \subset \msb(x,C_2(t))\subset \msb(x_0,1+C_2(t))$ for all $i\in \iintLigne{0,k}$ (otherwise, this would be in contradiction with the fact that almost surely $X_u \in \msb(X_0,C_2(t))$ for all $u\in[0,t]$). Hence, there exists $C>0$ such that, for all $x\in \msb(x_0,1)$, $k\in\nset$, $i\in \iintLigne{1,k-1}$ and almost every $s\in \Delta_{k,t}$,
%  \[\sup\{|T_{s_i}Q_*f(y)| + \norm{\na T_{s_i}Q_* f(y)},\ y\in E_{i-1}\} \ \leqslant \ C \sup\{|f(y)| + \norm{\na f(y)},\ y\in E_{i}\}\eqsp,\]
%   \[\sup\{|T_{s_k} f(y)| + \norm{\na T_{s_k}  f(y)},\ y\in E_{k-1}\} \ \leqslant \ C \sup\{|f(y)| + \norm{\na f(y)},\ y\in E_{k}\}\eqsp,\]
% and in particular
% \[\norm{\na (T_{s_1} Q_*  \dots  Q_* T_{s_k} f)(x)} \ \leqslant \ C^k ( \|f\|_\infty + \norm{\na f}_\infty) \eqsp.\]
%  Hence, $\bar P_t f$ is $\rmc^1$ on $\msb(x_0,1)$, on which it is equal to $P_t f$, which concludes.
\end{proof}

\begin{remark}
  \Cref{lem:stab_c1c} can be generalized  under the condition that
for some $k \in \nsets$,  the  characteristics $(\varphi,\lambda,Q)$ satisfy
\begin{enumerate}[label = (\roman*)]
\item \label{item_1_lem:stab_c1c_b} the flow  $\varphi$ and the Markov kernel $Q$ are compactly compatible;
\item \label{item_2_lem:stab_c1c_b} $\lambda\in\mrc^{k}(\msm)$ and for all $f \in \mrc^k(\msm)$, $\lambda Qf \in \mrc^k(\msm)$ and there exists a function $\Psi :\msm \to \rset_+$ such that for all compact set $\msk \subset \msm$, $\sup_{y \in \msk} \Psi(y) < \plusinfty$ and for all $x \in \msk$, $i \in\{1,\ldots,k\}$,
  \begin{equation*}
    \label{eq:1}
  \norm{\diff^i (\lambda Qf)(x)} \leq    \sup_{y \in \msk} \{ \Psi(y)\} \sup \ensemble{ \norm{\diff^i f(y)}}{y \in \supp \{Q(x,\cdot)\} \eqsp,i \in\{1,\ldots,k\} };
  \end{equation*}
\item \label{item_3_lem:stab_c1c_b} for all $t \in \rset_+$, we have $x \mapsto \varphi_t(x)$ is $k$-times continuously differentiable  and for all compact $\msk \subset \msm$, 
  \begin{equation*}
    \sup \ensemble{\norm{\diff^i \varphi_s(x)}}{s \in \ccint{0,t}, x \in \msk\eqsp, i \in \{1,\ldots,k\}} < \plusinfty \eqsp.
  \end{equation*}
\end{enumerate}
Then for all function $f \in \mrc^k(\msm)$, and $T \in \rset_+$,
$P_Tf \in \mrc^k(\msm)$. In addition, for all compact set
$\msk \subset\msm$, and $T \in \rset_+$, there exists $C \geq 0$ such
that for all $t \in \ccint{0,T}$,
$\sup_{x \in \msk} \absLigne{P_t f}(x) + \sup_{x \in \msk, i
  \in\{1,\ldots,k\}} \norm{\diff^i P_t f(x)} \leq C$.
\end{remark}


\begin{assumption}
  \label{ass:compact_sup}
    Let $(P_t)_{t \geq 0}$ be a non explosive PDMP semi-group with 
    characteristics $(\varphi,\lambda,Q)$. Assume that for all $T \geq 0$, there exists $M \geq 0$ such that for all $x \in \msm$ and $t \in \ccint{0,T}$, $\supp\{P_t(x,\cdot)\} \subset \cball{x}{M}$.
\end{assumption}
\begin{lemma}
  \label{lem:compact_sup}
  Assume \Cref{ass:compact_sup}.
 Then for all $f \in \rmc_c(\msm)$, $T \in \rset_+$, there exists a bounded set $\msa$ such that  $P_t^{\veps} f (x) = 0$, for all $x \not \in \msa$ and $t \in \ccint{0,T}$.
\end{lemma}
\begin{proof}
Let $f \in \rmc_c(\msm)$, $T \in \rset_+$. Then by assumption, there exist $M_f,M_T \in \rset_+$ such that $\supp(f) \subset \ball{x_0}{M_f}$, $x_0 \in \msm$, and $\supp\{P_t(x,\cdot)\} \subset \cball{x}{M}$ for all $t \in \ccint{0,T}$, $x \in \msm$. Therefore, we get for all  $x \not \in \cball{x_0}{M_T+M_f+1}$, $P_tf(x) = \int_{\msm}\1_{\cball{x}{M_T}\cap \ball{x_0}{M_f}}(y) f(y) P_t(x,\rmd y) = 0$. Indeed by construction $\cball{x}{M_T}\cap \ball{x_0}{M_f} = \emptyset$ since by the triangle inequality,  $\dist(x,y) \leq M_T$ implies that $\dist(x_0,y) \geq M_f+1$. 
\end{proof}


By \Cref{lem:stab_c1c}, \Cref{lem:compact_sup} and \cite[Proposition 3.3, Chapter 1]{ethier:kurtz:1986}, we obtain the following result. 
\begin{corollary}
\label{coro:core_generator}
  Assume \Cref{ass:stability} and \Cref{ass:compact_sup}. Then, $\rmc^1_c(\msm)$ is a core for the (strong) generator of $(P_t)_{t \geq 0}$. 
\end{corollary}


\begin{definition}
  We say that the PDMP semi-group $(P_t)_{t \geq 0}$ with   characteristics $( \varphi,\lambda,Q)$ is smoothly and compactly approximable if
  for all $\varepsilon>0$ there exists  characteristics  $( \varphi,\lambda^\varepsilon,Q^\varepsilon)$ satisfying \Cref{ass:stability}-\Cref{ass:compact_sup} and 
\begin{equation}
\label{eq:def_sm_comp_approx}
  \sup_{\substack{x \in \msm\\ \msa \in \mcbb(\msm)}} \defEns{\lambda^\varepsilon (x) \wedge \lambda (x) \abs{  Q^\varepsilon(x,\msa)  -  Q (x,\msa) } + \abs{\lambda^\varepsilon (x) - \lambda (x)} } \leq \veps \eqsp.
\end{equation}
\end{definition}



\begin{proposition}\label{prop:approx-BPS}
  Let $U\in\rmc^2(\rset^d)$, $\rate>0$ and $\loiy\in\mcp(\msv)$ with $\msv \subset \rset^d$ bounded. Then the associated BPS on $\rset^d \times \msv$, given by \Cref{ex:BPS}, is smoothly and compactly  approximable.
\end{proposition}

\begin{proof}
  Let $(\varphi,\lambda,Q)$ be the  characteristics of the BPS given by \Cref{ex:superposition:bps}. Let $\veps > 0$, $\lambda^{\veps}: \msm \to \rset_+$ and $Q^{\veps}$ be  a Markov kernel on $(\rset^d\times \msv,\mcbb(\rset^d\times \msv))$ defined for all $(x,y)\in \rset^d \times \msv$ and $\msa \in \mcbb(\rset^d)$ by
    \begin{equation*}
    \lambda^{\veps}(x,y) = \lambda_1^{\veps}(x,y) + \lambdab \eqsp, \, \lambda_1^{\veps}(x,y) = (\ps{y}{\nabla U(x)}-\veps)^2_+ / (\veps + (\ps{y}{\nabla U(x)}-\veps)_+) \eqsp,
  \end{equation*}
  \begin{equation*}
    Q^{\veps}((x,y),\msa) =    (1/\lambda^{\veps}(x,y))\defEns{\lambda_1^{\veps} \updelta_{(x,\Refl(x,y))}(\msa) + \rate (\updelta_x \otimes \loiy)(\msa)} \eqsp,
  \end{equation*}
  where $\Refl$ is defined by \eqref{eq:def_refl} for $g = \nabla U$. Then, similarly to the BPS process, $(\varphi,\lambda^{\veps},Q^{\veps})$ defines a non explosive semi-group $(P_t^{\veps})_{t\geq 0}$ on $(\rset^d \times \msv) \times \mcbb (\rset^d \times \msv)$. In addition we have
     \begin{equation}
     \label{eq:bound_distance_lambda_lambda_eps}
    \sup_{x \in \msm } \abs{ \lambda^{(\epsilon)}(x,y) -
    \lambda(x,y) } \leq 2 \epsilon  \eqsp.
   \end{equation}
   Therefore, using \Cref{rem:sync}, we get
   \begin{multline*}
\sup_{\substack{x \in \msm\\ \msa \in \mcbb(\msm)}} \defEns{\lambda^\varepsilon (x) \wedge \lambda (x) \abs{  Q^\varepsilon(x,\msa)  -  Q (x,\msa) } + \abs{\lambda^\varepsilon (x) - \lambda (x)} } \\ \leq 2 \sup_{\substack{x \in \msm\\ \msa \in \mcbb(\msm)}}  \abs{\lambda^\varepsilon (x)   Q^\varepsilon(x,\msa)  -  \lambda (x)  Q (x,\msa) } \leq 4 \veps   \eqsp,
\end{multline*}
which shows \eqref{eq:def_sm_comp_approx}.

Since $\msv$ is assumed to be  bounded, $\msv \subset\cball{0}{M_{\msv}}$, with $M_\msv \in \rset_+$. Therefore by definition,  for all $t \in \rset_+$ and $(x,y) \in \rset^d \times \msv$, we have $P^{\veps}_t((x,y),\cball{x}{t M_\msv} \times \msv) = 1$ and $P^{\veps}_t$ satisfies \Cref{ass:compact_sup}.

Finally, we show that \Cref{ass:stability} is satisfied. \Cref{ass:stability}-\ref{item_3_lem:stab_c1c_b} trivially holds by definition of $\varphi$. 

For all closed ball, $\cball{0}{M} \subset \rset^d$, $M \in \rset_+$, $Q^{\veps}((x,y),\cball{0}{M} \times \msv) = 1$ for all $x \in \cball{0}{M}$. Therefore, for all compact set $\msk \subset \ball{0}{M} \times \msv \subset \rset^d \times \msv$, $M \geq 0$, $T \in \rset_+$, $N \in \nset$, $(t_i)_{i \in \{1,\ldots,N+1\}} \in \rset_+^n$,
$\sum_{i=1}^{N+1} t_i \leq T$, \eqref{def:prop_tmsk} is satisfied for $\tilde{K} = \ball{0}{M+TR} \times \msv$, with  $R = \sup_{y \in \msv} \norm{y}$,
for all $i \in \{1,\ldots,N+1\}$ and $s_i \in \ccint{0,t_i}$ setting
$t_0=0$,  $(\msk_i)_{i \in \{0,\ldots,N\}}$ are given by
\begin{equation*}
  \msk_0 = \ball{0}{M} \times \msv\eqsp, \, \msk_i =  \ball{0}{R_i } \times \msv \eqsp, \, R_i =M+R \sum_{j=0}^i t_j \eqsp,
\end{equation*}
and \eqref{def:msk_i} holds. Thus, $\varphi$ and $Q^{\veps}$ are compactly compatible.

    Then note that for all  $\lambda^{\veps}$ is
  continuously differentiable on $\msm$ since
  $t \mapsto (t-\veps)_+^2/(\veps+(t-\veps)_+)$ is on $\rset$; and its gradient is given for all $x \in \msm$ by
  \begin{equation}
    \label{eq:gradient_lambda_eps}
    \nabla(\lambda^{(\epsilon)})(x,y) =
    \begin{cases}
      \frac{(\ps{y}{\nabla U(x)}-\epsilon)(\ps{y}{\nabla U(x)}+\epsilon)}{\ps{y}{\nabla U(x)}^2} \begin{pmatrix}  \nabla^2 U(x) y , \nabla U(x)
      \end{pmatrix} & \text{ if $\ps{y}{\nabla U(x)} \geq \epsilon$}\\
      0 & \text{ otherwise} \eqsp.
    \end{cases}
  \end{equation}
  In addition, for all continuously differentiable function $f: \rset^d \times \msv \to \rset$,  $(x,y) \in \rset^d \times \msv$, we have
  $    \lambda^{\veps}(x,y)  Q^{\veps}f(x,y) = A_1(x,y) + A_2(x,y)$  where
  \begin{equation*}
    A_1(x,y) = \lambda_1^{\veps}(x,y) f(x,\Refl(x,y)) \eqsp, \, A_2(x,y) =  \rate \int_{\msv} f(x,\tilde y) \loiy(\rmd \tilde y) \eqsp.
  \end{equation*}
  We show that $A_1$ and $A_2$ are continuously differentiable and satisfy for $i=1,2$, for all compact set $\msk \in \rset^d \times \msv$, for all $(x,y) \in \msk$,
  \begin{equation}
    \label{eq:bound_bps_A_1_2} 
    \norm{\diff A_i(x,y)} \leq \sup_{(w,z) \in \msk} \{\Psi_i(w,z)\}\sup\ensemble{\abs{f}(x,\tilde{y}) + \norm{\diff f(x,\tilde{y})}}{y \in \msv}   \eqsp,
  \end{equation}
  where $\Psi_i : \rset^d \times \msv \to \rset_+$, $i=1,2$, are
  bounded on compact sets of $\rset^d \times \msv$. Note that if we
  show \eqref{eq:bound_bps_A_1_2}, since for all
  $(x,y) \in \rset^d \times \msv$,
  $\supp \{Q((x,y),\cdot)\} = \{x\} \times \msv$, this result concludes the proof that \Cref{ass:stability}-\ref{item_2_lem:stab_c1c_b} holds.
  
  First, for all $(x,y) \in \rset^d \times \msv$, $\Refl$ is
  continuously differentiable at $(x,y)$ is
  $\ps{y}{\nabla U(x)} \not =0$. Since $f$, $\lambda_1^{\veps}$ are
  continuously differentiable and $\lambda_1^{\veps}(x,y) = 0$ if
  $\ps{y}{\nabla U(x)} \leq \veps$, $A_1$ is continuously
  differentiable and satisfies for all $(x,y) \in \rset^d \times y$,
  $\ps{y}{\nabla U(x)} \geq \veps$
  \begin{equation}
    \label{eq:bound_bps_A_1}
\norm{\diff A_1(x,y)} \leq  \norm{\diff \lambda_1^{\veps}(x,y)} \abs{f}(x,\Refl(x,y)) + \lambda_1^{\veps}(x,y) (1+\norm{\diff \Refl(x,y)})\norm{\diff f(x,\Refl(x,y))} \eqsp. 
\end{equation}
Regarding $A_2$, we have for all $(x,y) \in \rset^d \times \msv$, since $\diff f$ is bounded on all compact sets of $\rset^d \times \msv$ and the Lebesgue dominated convergence theorem,
\begin{equation*}
\norm{\diff A_2(x,y)} \leq \rate \int_\msv \norm{\diff_x f(x,\tilde y)} \loiy(\tilde y) \leq \rate \sup_{y \in \msv}\norm{\diff f(x,\tilde y)}\eqsp,
\end{equation*}
where $\diff_x$ is the differential operator with respect to the $x$-variable. Combining this result and \eqref{eq:bound_bps_A_1}, we get that \eqref{eq:bound_bps_A_1_2} holds and therefore \Cref{ass:stability}-\ref{item_2_lem:stab_c1c_b} as well.

\end{proof}


\begin{lemma}
  \label{lem:dist_generator}
  Let $(P_t^1)_{t \geq 0}$ and $(P_t^2)_{t \geq 0}$ be  non explosive PDMP semigroups with  characteristics $(\varphi,\lambda^1,Q^1)$ and $(\varphi,\lambda^2,Q^2)$ respectively. Assume that there exists $\eta \geq 0$, such that 
  \begin{equation*}
    \sup_{\substack{x \in \msm \\ \msa \in \mcbb(\msm) }} \abs{\lambda^1(x) Q^1(x,\msa) - \lambda^2(x) Q^2(x,\msa)} \leq \eta \eqsp.
  \end{equation*}
 Then for all  $f \in \rmc^1_c(\msm)$,
  \begin{equation*}
    \sup_{x \in \msm} \abs{\generator f(x) - \generator^{\veps} f(x)} \leq \eta \sup_{x \in \msm}\abs{f}(x) \eqsp,
  \end{equation*}
  where $\generator^1$, $\generator^2$ are the (weak) generator of $(P_t^1)_{t \geq 0}$,   $(P_t^{2})_{t \geq 0}$ respectively.
\end{lemma}

\begin{proof}
  Let $\veps >0$ and $f \in \rmc^1_c(\msm)$. 
  Since $\rmc^1_c(\msm)$ belongs to the domain of $\generator^1$ and $\generator^{2}$, we have for all $x \in \msm$ by \eqref{eq:def_generator} and \cite[Section III.1]{dunford:schwartz:1958} \alain{mettre bon label}
  \begin{multline*}
    \abs{\generator^1f(x) - \generator^2f(x)} = \abs{\lambda^1(x) Q^1f(x)-\lambda^2(x) Q^2f(x)} \\\leq  \sup_{x \in \msm} \{\abs{f}(x) \}\sup_{\msa \in \mcb{\msm}} \abs{\lambda^1(x) Q^1(x,\msa)-\lambda^2(x) Q^2(x,\msa)} \leq \eta \sup_{x \in \msm}\abs{f}(x)  \eqsp, 
  \end{multline*}
  which concludes the proof.
\end{proof}

\begin{proposition}\label{lem:critere-invariant}
  Let $(P_t)_{t \geq 0}$ be a non explosive PDMP semigroup with  characteristics $(\varphi,\lambda,Q)$. Assume that $(P_t)_{t \geq 0}$ is smoothly and compactly approximable and $\int_{\msm} \abs{\lambda} (x) \mu(\rmd x) < \plusinfty$. In addition, assume that the (weak) generator $\generator$ associated with $(P_t)_{t \geq 0}$ satisfies for all $f \in \mrc^1_c(\msm)$,
  \begin{equation}
    \label{eq:critere_inv}
    \int_{\msm} \generator f(x) \mu (\rmd x) = 0 \eqsp.
  \end{equation}
  Then $\mu$ is invariant for $(P_t)_{t \geq 0}$. 
  % Let $\generator$ be the generator of the semigroup $(P_t)_{t\geqslant 0}$ of a homogeneous PDMP with characteristics $( \varphi,(\lambda_i,Q_i)_{i\in \iintLigne{1,n}})$, and let $\mu\in \mcp(\msm)$. Suppose the PDMP is nicely approximable  and $\int_{\msm} \lambda_i \rmd \mu < \infty$ for all $i\in \iintLigne{1,n}$.
%that satisfies
%\begin{eqnarray*}
%\sum_{i=1}^n \int_{\msm} |\lambda_i^\varepsilon - \lambda_i| \rmd \mu & \underset{\varepsilon\rightarrow 0}\longrightarrow & 0\eqsp .
%\end{eqnarray*}
% Suppose moreover that
% \begin{eqnarray*}
% \int_{\msm} \generator f(x) \mu( \rmd x) & = & 0
% \end{eqnarray*}
% for all $f\in \mrc^{1}_c(\msm)$. Then $\mu$ is invariant for $(P_t)_{t\geqslant 0}$.
\end{proposition}

\begin{proof}
Since $\mrc^{1}_c(\msm)$ is dense in $\mrl^\infty(\mu)$, where $\mrl^\infty(\mu)$ is the space of measurable function with bounded essential supremum with respect to $\mu$,  it is sufficient to show that 
\[\int_\msm P_t f (x) \mu(\rmd x) \ = \ \int_\msm   f(x)  \mu(\rmd x) \]
for all $t\geqslant 0$ and $f\in \mrc^{1}_c(\msm)$.
Let $\veps >0$, a PDMP semi-group $(P^{\veps}_s)_{s \geq 0}$ with  characteristics  $(\varphi,\lambda^{\veps}, Q^{\veps})$ satisfying \Cref{ass:stability}-\Cref{ass:compact_sup} and \eqref{eq:def_sm_comp_approx}, and $t \geq 0$ . 
By \Cref{prop:synchrone}, we have for all $x \in \msm$, $\tvnorm{\updelta_x P_t - \updelta_x P^{\veps}_t} \leq 2(1-\rme^{-t \veps})$, therefore we get for all  $f \in \mrc^1_c(\msm)$
\begin{align}
\nonumber
  &   \abs{  \int_{\msm} P_tf(x) \mu(\rmd x)-     \int_{\msm} f(x) \mu(\rmd x)} \leq \abs{\int_{\msm} \defEns{P_t f(x) -P_t^{\veps} f(x)}\mu(\rmd x)} \\
  \nonumber
& \qquad \qquad  \qquad   \qquad \qquad \qquad   \qquad \qquad  +\abs{ \int_{\msm} \{P_t^{\veps} f(x) - f(x) \} \mu(\rmd x)  } \\%[-0.5cm]
  \label{eq:preuve_invariance_bounded_support_1} 
 &      \qquad   \qquad \qquad \qquad   \qquad \qquad  \leq 2(1-
    \rme^{-\veps t}) \sup_{x \in \msm} \abs{f(x)} +\abs{ \int_{\msm} \{ P_t^{\veps} f(x) - f(x) \} \mu(\rmd x)  } \eqsp.
\end{align}

Furthermore, by \Cref{coro:core_generator}, $\mrc^1_c(\msm)$ is a
core for the strong generator associated with $(P_s^{\veps})_{s \geq 0}$. Thus, it belongs to the
domain of the strong generator of $(P_t^{\veps})_{t \geq 0}$ and by Dynkin formula \cite[Proposition 1.5-(c)]{ethier:kurtz:1986}, we get
\begin{equation*}
   \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)=  \int_{\msm} f(x)\mu(\rmd x)- \int_{\msm} \int_0^t \generator^{\veps}P_s^{\veps}f(x) \rmd s\,\mu(\rmd x)\eqsp.
\end{equation*}
Therefore,
\begin{multline}
    \label{eq:preuve_invariance_bounded_support_2}
  \abs{ \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)- \int_{\msm} f(x) \mu(\rmd x) } \\\leq 
  \abs{\int_{\msm} \int_0^t \defEns{\generator^{\veps}-\generator } P_s^{\veps}f(x) \rmd s\mu(\rmd x)} 
 + \abs{\int_{\msm} \int_0^t \generator P_s^{\veps}f(x) \rmd s\, \mu(\rmd x)} \eqsp.
\end{multline}
In addition, by \eqref{eq:lem_stab_clc} in \Cref{lem:stab_c1c}, \Cref{ass:stability}-\ref{item_3_lem:stab_c1c} and \Cref{lem:compact_sup},  $\int_{\msm} \int_0^t \abs{\generator P_s^{\veps}f(x)} \rmd s\mu(\rmd x) < \plusinfty$. Therefore, by  Fubini's theorem and \eqref{eq:critere_inv}, we get  $\int_{\msm} \int_0^t \generator P_s^{\veps}f(x) \rmd s\mu(\rmd x) = 0$. Combining  this result, \eqref{eq:preuve_invariance_bounded_support_2} becomes 
\begin{equation}
    \label{eq:preuve_invariance_bounded_support_2_5}
  \abs{ \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)- \int_{\msm} f(x) \mu(\rmd x) } \leq 
  \abs{\int_{\msm} \int_0^t \defEns{\generator^{\veps}-\generator } P_s^{\veps}f(x) \rmd s\mu(\rmd x)}  \eqsp.
\end{equation}
Note that by \eqref{eq:rem_syn_3}, \eqref{eq:def_sm_comp_approx} and \Cref{lem:dist_generator}, for all  $f \in \mrc^1_c(\msm)$
\begin{equation*}
%  \label{eq:diff_generator_approximation}
\sup_{x \in \msm}\abs{  \generator f(x) -   \generator^{\veps} f(x)} \leq \veps \sup_{x \in \msm} \abs{f(x)} \eqsp. 
\end{equation*}
Using this result in \eqref{eq:preuve_invariance_bounded_support_2_5}, we obtain 
\begin{equation}
\label{eq:preuve_invariance_bounded_support_3}
\abs{ \int_{\msm} P_t^{\veps} f(x)\mu(\rmd x)- \int_{\msm} f(x) \mu(\rmd x) } \leq  \veps t \sup_{\substack{x \in \msm\\
  s \in \ccint{0,t}}} \abs{P_s f(x)} \leq \veps t \sup_{x \in \msm} \abs{f}(x) \eqsp. 
\end{equation}

Plugging 
 \eqref{eq:preuve_invariance_bounded_support_3} in \eqref{eq:preuve_invariance_bounded_support_1}, we finally obtain
\begin{equation*}
   \abs{  \int_{\msm} P_tf(x)\mu(\rmd x)-     \int_{\msm} f(x) \mu(\rmd x)} \leq  (2(1-
    \rme^{-\veps t}) +\veps t  )\sup_{x \in \msm} \abs{f(x)} \eqsp.
\end{equation*}
Taking the limit as $\veps$ goes to $0$ concludes the proof. 
\end{proof}

\begin{proposition}\label{prop:invarince-BPS}
  Let $U\in\rmc^2(\rset^d)$, $\rate>0$ and $\loiy\in\mcp(\msv)$ with
  $\msv \subset \rset^d$, and let $(P_t)_{t\geqslant 0}$ be the
  corresponding BPS Markov semi-group, given by \Cref{ex:BPS}. Assume
  that $\loiy$ is rotation invariant,~\ie~for all
  $O \in \rset^{d\times d}$, $O^{\transpose}O = \Id$,
  $\loiy(O \msa) = \loiy(\msa)$, for all $\msa \in\mcbb(\msv)$. In addition, suppose that
\[\int_{\rset^d} ( 1+\norm{\na U(x)} ) e^{-U(x)}\rmd x \ < \ \infty \eqsp,\quad \int_\msv \norm{y} \loiy(\rmd y)\ < \ \infty \eqsp.\]
Then $\tpi = \pi \otimes \loiy$ is invariant for $(P_t)_{t\geqslant 0}$, where $\pi$ is the probability measure on $(\rset^d,\mcbb(\rset^d))$ with density with respect to the Lebesgue measure proportional to $x \mapsto \rme^{-U(x)}$.  
\end{proposition}

\begin{proof}
  Consider first the case where $\msv$ is bounded. Then, by \Cref{prop:approx-BPS}, $(P_t)_{t \geq 0}$ is smoothly and compactly approximable and the other assumptions of \Cref{lem:critere-invariant} are easily checked.  In particular, for all $f\in\mrc^{1}_c(\rset^d\times\msv) $, 
$   \int \generator f(x)  \pi(\rmd x) = 0$
  follows from an integration by parts and because $\msv$ and $\loiy$ is rotation invariant, see e.g. \cite{MonmarcheRTP} for more details.


Consider the conditional distribution associated with $\loiy$ defined for all $\msa \in \mcb{\msv}$, 
\begin{equation}
  \label{eq:loiy_R}
  \mu^{R}(\msa) = \mu(\ball{0}{R}\cap \msa) / \mu(\ball{0}{R}) \eqsp,
\end{equation}
for $R$ large enough such that $\mu(\ball{0}{R}) \not = 0$.  Consider
a BPS semi-group $(P_t^R)_{t \geq 0}$ associated with $U$ and $\mu^R$,
\ie~with  characteristics $(\varphi,\lambda,Q^R)$ with $\varphi$ given by \eqref{eq:transport_libre}, $\lambda$ by \eqref{eq:def_lambda_total_bps} and
$Q^R$ is defined for all $(x,v) \in \rset^d \times \msv$, $\msa \in \mcbb( \rset^d \times \msv)$ by
\begin{equation*}
    Q^R((x,y),\msa)  =  \lambda^{-1}(x,y)\defEns{\ps{\nabla U(x)}{y} \updelta_{(x,\Refl(x,y))}(\msa) + \rate (\updelta_x \otimes \loiy^R)(\msa)} \eqsp. 
\end{equation*}
Note that since $\msv \cap \ball{0}{R}$ is bounded,  $\tilde{\pi}^{R} = \pi \otimes \loiy^R$ is an invariant measure  for $(P_t^R)_{t \geq 0}$. Therefore for
any $f : \rset^{d} \times \msv \to \rset$, bounded and measurable, $t \geq 0$, we
have for all $R \geq 0$ large enough,
\begin{align}
  \nonumber
  & \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}(x,y) - \int_{\rset^{d} \times \msv} f(x,y) \rmd \tilde{\pi}(x,y)} \\
    \nonumber
  &  \qquad \qquad \leq \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}(x,y) - \int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}^{R}(x,y) } \\
    \nonumber
  & \qquad\qquad\qquad+  \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}^{R}(x,y) - \int_{\rset^{d} \times \msv} P_t^{R} f(x,y) \rmd \tilde{\pi}^{R}(x,y) } \\
    \nonumber
  & \qquad\qquad\qquad+ \abs{\int_{\rset^{d} \times \msv}  f(x,y) \rmd \tilde{\pi}^{R}(x,y) - \int_{\rset^{d} \times \msv} f(x,y) \rmd \tilde{\pi}(x,y) } \\
  % \label{eq:invariance_non_bornee_1}
  \nonumber
  & \qquad\qquad \leq 2 \sup_{\rset^d \times \msv}\abs{f}  \mu\parenthese{\rset^{d} \setminus \ball{0}{R}} +   \abs{\int_{\rset^{d} \times \msv} P_t f(x,y) \rmd \tilde{\pi}^{R}(x,y) - \int_{\rset^{d} \times \msv} P_t^{R} f(x,y) \rmd \tilde{\pi}^{R}(x,y) } \eqsp.
\end{align}
Since $\lim_{R \to \plusinfty} \mu\parentheseLigne{\rset^{d} \setminus \ball{0}{R}} = 0$, it
remains to show that the last term in the right-hand side goes to $0$
as $R \to \plusinfty$ and the proof will be finished. Besides, note
that this result holds if for $t >0$, we  show that for all
$(x,y) \in \rset^{d} \times \msv$,
\begin{equation}
  \label{eq:invariance_non_bornee_2}
\lim_{R \to \plusinfty}   \tvnorm{ \updelta_{(x,y)} P_t  -  \updelta_{(x,y)} P_t^R } = 0 \eqsp.
\end{equation}
But by \Cref{prop:synchrone} and definition of  characteristics of $(P_s)_{s \geq 0}$ and $(P_s^R)_{s \geq 0}$, we get for all $t \geq 0$, $(x,y) \in \rset^d \times \msv$, 
\begin{equation*}
  \tvnorm{ \updelta_{(x,y)} P_t  -  \updelta_{(x,y)} P_t^R }  \leq 2 (1-\exp(-\rate \mu(\msv \setminus \ball{0}{R}))) \eqsp,
\end{equation*}
which shows that \eqref{eq:invariance_non_bornee_2} holds. 
\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> regularityD.tex <==
\section{Regularity estimates for PDMP semigroups}
\label{sec:stab_c1c}


For our next result, we need the following definition.
\begin{definition}
  \label{def:compact_comp}
We say that a
differential flow $\varphi$ on $\msm$ and a Markov kernel $Q$ are
compactly compatible if for all compact set $\msk \subset \msm$ and $T \geq 0$,
there exists a compact set $\tilde \msk \subset \msm$ satisfying for
all $n \in \nsets$, $(t_i)_{i \in \iint{1,n}} \in \rset_+^n$,
$\sum_{i=1}^{n} t_i \leq T$,
there exists a sequence $(\msk_i)_{i \in \iint{1,n}}$ of
compact sets of $\msm$ such that setting $\msk_0 = \msk$,
\begin{enumerate}[label=(\roman*)]
  \item \label{def:compact_comp_item_1} for all $i \in \iint{1,n}$, $\msk_i$ only depends on $(t_j)_{j \in \iint{1,i}}$ and $\cup_{i=0}^{n} \msk_i \subset \tilde \msk$;
  \item \label{def:compact_comp_item_2} for all $i \in \iint{0,n-1}$, $s_{i+1} \in \ccint{0,t_{i+1}}$ and $s_{n+1} \in \ccintLigne{0,T-\sum_{j=1}^n t_j}$,
    \begin{equation*}
%  \label{def:msk_i}
 \bigcup_{x \in \msk_i} \supp \{ Q(\varphi_{t_{i+1}}(x),\cdot) \} \subset
\msk_{i+1} \eqsp, \qquad \varphi_{s_{i+1}}( \msk_{i}) \subset \tilde \msk  \eqsp, \qquad  \varphi_{s_{n+1}}( \msk_{n}) \subset \tilde \msk
\end{equation*}

\end{enumerate}
\end{definition}

Note that by definition, if $\varphi$ and $Q$ are compactly compatible
and the PDMP semigroup with  characteristics $(\varphi, \lambda,Q)$ is
non explosive, for all $T \geq 0$ and all
compact set $\msk \subset \msm$, there exists a compact set
$\tilde \msk \subset \msm$, such that
$\PP (X_t \in \tilde{\msk}, \text{ for all $t \in \ccint{0,T}$} ) =1$,
where $(X_t)_{t \geq 0}$ is a PDMP process with  characteristics $(\varphi, \lambda,Q)$ and starting from $X_0 \in \msk$.

\begin{assumption}
  \label{ass:stability}
The  characteristics $(\varphi,\lambda,Q)$ satisfy
\begin{enumerate}[label = (\roman*)]
\item \label{item_1_lem:stab_c1c} the flow  $\varphi$ and the Markov kernel $Q$ are compactly compatible;
\item \label{item_2_lem:stab_c1c} $\lambda\in\mrc^{1}(\msm)$ and for
  all $f \in \mrc^1(\msm)$, $\lambda Qf \in \mrc^1(\msm)$ and there
  exists a function $\Psi :\msm \to \rset_+$ such that for all compact set $\msk \subset \msm$, $\sup_{y \in \msk} \Psi(y) < \plusinfty$ and for all 
  $x \in \msk$,
  \begin{equation*}
    \label{eq:1}
 \norm{\diff (\lambda Qf)(x)} \leq   \sup_{y \in \msk}\{ \Psi(y) \} \sup \ensemble{\abs{f(y)} + \norm{\diff f(y)}}{y \in \supp \{Q(x,\cdot)\}};
  \end{equation*}
\item \label{item_3_lem:stab_c1c} for all compact $\msk \subset \msm$, 
  \begin{equation*}
    \sup \ensemble{\norm{\diff \varphi_s(x)}}{s \in \ccint{0,t}, x \in \msk} < \plusinfty \eqsp.
  \end{equation*}
\end{enumerate}  
\end{assumption}
\begin{lemma}
  \label{lem:stab_c1c}
  Let $(P_t)_{t\geqslant 0}$ be a non explosive PDMP semigroup on $\msm$ with corresponding characteristics $(\varphi,\lambda,Q)$ satisfying \Cref{ass:stability}. 
  Then for all $f \in \mrc^1(\msm)$, $T \in \rset_+$, $P_Tf \in \mrc^1(\msm)$  and for all compact set $\msk \subset \msm$, there exists $C \geq  0$  such that for all $t \in \ccint{0,T}$,
  \begin{equation}
    \label{eq:lem_stab_clc}
  \sup_{x \in \msk}\{ \abs{P_t f}(x) + \norm{\diff (P_tf)(x)}\} \leq C \eqsp.  
  \end{equation}
%   In particular $\mrc^1(\msm)$ is a  core for $(P_t)_{t \geq 0}$. 
% that  and $(x,t)\in\msm\times\rset_+ \mapsto \norm{\na \varphi_t (x)}$ is locally bounded, and that there exist locally bounded functions $C_1:\msm \rightarrow \rset_+$ and $C_2:\rset_+\rightarrow \rset_+$  such that for all $f\in \rmc^1_c(\msm)$, $\lambda Qf\in \rmc^1_c(\msm)$ and for all $x\in\msm$, 
% \[\norm{\na (\lambda Q f)(x)}\ \leqslant  \ C_1(x)\sup\{|f(y)| + \norm{\na f(y)},\ y\in \supp Q(x,\cdot)\}\eqsp,\]
%  and for all $t\geqslant 0$,  $X_s \in \msb(X_0,C_2(t))$ for all $s\in[0,t]$ almost surely. Then, if $f\in \mrc^1_c(\msm)$, $ P_t f\in \mrc^1_c(\msm)$ for all $t \geq 0$. %Therefore, $\mrc^1_c(\msm)$ is a core for $(P_t)_{t \geq 0}$.
 
 
% More precisely, if $f\in \mrc^1_c(\msm)$ and $t\geqslant0$, then there exist $C>0$ and a compact $\msk$ of $\msm$  such that,  for all $s\in [0,t]$, the support of $P_s f$ is included in $\msk$ and  $\norm{\na P_s f}_\infty \leqslant C$.
\end{lemma}
% \begin{remark}
%   Note that in the case where the condition $\inf_{x \in \msm} \lambda(x) >0$ is not satisfied, we can simply consider a modified characteristics $(\varphi,\bar \lambda, \bar Q)$ which defines the same PDMP semigroup $(P_t)_{t \geq 0}$ where $\bar Q$ and $\bar \lambda$ are given for all $x \in \msm$ and $\msa \in \mcb{\msm}$ by
%   \begin{equation*}
%     \bar \lambda(x) = \lambda(x) + \rate \eqsp, \, \bar Q(x,\msa) = \bar \lambda^{-1}(x)\lambda(x) Q(x,\msa) + \parenthese{1-\bar \lambda^{-1}(x)\lambda(x)} \updelta_x(\msa) \eqsp,
%   \end{equation*}
%   for $\rate >0$. Then, if the other conditions of \Cref{lem:stab_c1c} are satisfied, the modified characteristics $(\varphi,\bar \lambda, \bar Q)$ satisfy these conditions as well and $\inf_{x \in \msm} \bar \lambda(x) \geq \rate$. 
% \end{remark}
\begin{proof}
 
For all $x \in \msm$
  denote by $(X_t^x)_{t \geq 0}$ a PDMP starting from $x$ associated
  with the characteristics $(\varphi,\lambda,Q)$ and defined by \Cref{const:1}.  Let
  $(S_n^x)_{n \in \nset}$ be the jump times of $(X_t^x)_{t \geq 0}$
  for all $x \in \msm$ and $(\mcf_t)_{t \geq 0}$ the associated filtration. Let $f\in \mrc^1(\msm) $, $T\geqslant 0$ and a
  compact set $\msk \subset \msm$. For $T =0$, the result is
  straightforward so we consider $T >0$. Let $\tilde \msk$ satisfying for all $n \in \nset$,
$(t_i)_{i \in \iint{1,n+1}} \in \rset_+^n$,
$\sum_{i=1}^{n+1} t_i \leq T$,  \ref{def:compact_comp_item_1}-\ref{def:compact_comp_item_2} in \Cref{def:compact_comp}.
% $\cup_{i=0}^{n} \msk_i \subset \tilde \msk$,
% $\varphi_{s_i}( \msk_{i-1}) \subset \tilde \msk$, for all
% $i \in \iint{1,n+1}$ and $s_i \in \ccint{0,t_i}$ setting
% $t_0=0$, where $(\msk_i)_{i \in \{0,\ldots,n\}}$ are given by \eqref{def:msk_i}. 

Since for all $x  \in \msk$, 
  $\PP (X_t^x \in \tilde \msk, \text{ for all } t \in \ccint{0,T}) = 1$,
  for all $t \in \ccint{0,T}$ and $x \in \msm$,
  \begin{equation}
    \label{eq:core_proof_1}
    \abs{P_tf(x)} = \abs{\expe{f(X_t)}} \leq \sup_{y \in \tilde \msk} \abs{f}(y) \eqsp.
  \end{equation}
  
Furthermore,  $(P_t)_{t \geq 0}$
  is assumed to be non explosive. Therefore
  $\sup_{n \in \nset} \S^{x}_n = \plusinfty$ and we can consider the
  following decomposition for all $t \in \ccint{0,T}$ and $x \in \msk$
  \begin{equation}
    \label{eq:decomposition_regular_pDMP}
  P_tf(x)  = \sum_{n=0}^{\plusinfty} \expeMarkov{}{\1_{\coint{S^{x}_n,S^{x}_{n+1}}}(t) f(X^{x}_t)} \eqsp.
\end{equation}
We  show that for all $n \in \nset$,
  \begin{equation}
    \label{eq:def_F_n}
   F_{n,t} : x \mapsto
  \expeMarkov{}{\1_{\cointLigne{S^{x}_n,S^{x}_{n+1}}}(t)
    f(X^{x}_t)}  \eqsp,
  \end{equation}
 is continuously
  differentiable and in addition there exists $C \geq 0$ such that for all
  $n \in \nset$, $t \in \ccint{0,T}$
  \begin{equation}
    \label{eq:estimate_gradient_n}
\sup_{x \in \msk}   \norm{ \diff  F_{n,t} (x)} \leq C^n  /n!\eqsp.%       \expeMarkov{(x,y)}{\1_{\coint{\bS_n^{\epsilon},\bS_n^{\epsilon}}}(t) } \eqsp,
   \end{equation}
   %where $(\bS_n^{\epsilon})_{n \in \nset}$ are the event times of a Poisson process with constant jump rate $\rate$.
   Assume for the moment that this result holds. Then, we have for all $t \in \ccint{0,T}$,
    \begin{equation*}
      \lim_{N \to \plusinfty}   \sum_{n=N}^{\infty} \sup_{x \in \msk}  \norm{ \diff F_{n,t}(x) } = 0 \eqsp. 
    \end{equation*}
    By \eqref{eq:decomposition_regular_pDMP}, it implies that
    $x \mapsto P_T f(x)$ is continuously differentiable. In
    addition, for all compact set $\msk \subset\msm$, there exists $C \geq 0$ such that for all $t \in \ccint{0,T}$, $ \norm{\diff P_tf(x)}_{\msk} \leq C $.
 %    \begin{equation*}
 %        \label{eq:core_proof_0}
 % \norm{\diff P_tf(x)}_{\msk} \leq C \eqsp.
 %    \end{equation*}
This result and \eqref{eq:core_proof_1} imply \eqref{eq:lem_stab_clc}.
  
    We now turn in showing that for all $n \in \nset$, $F_n$ is
    continuously differentiable and \eqref{eq:estimate_gradient_n}
    holds. We first show this result for $n = 0$. In a second time, we
    make an induction on $n \in \nsets$. 

For all $x \in \msk$ and $t \in \ccint{0,T}$, we have
    \begin{equation*}
      F_{0,t}(x) =  f(\phi_t(x)) \exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \eqsp. 
    \end{equation*}
Therefore, for all $x\in \msk$ and $t \in \ccint{0,T}$, we obtain by \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c}
    \begin{multline*}
      \diff F_{0,t}(x) = \defEns{\diff f (\phi_t(x))} \diff (\phi_t)(x) \exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \\
+        f(\phi_t(x))   \parentheseDeux{\int_0 ^t \defEns{\diff  \lambda (\phi_s(x)) \cdot \diff(\phi_s)(x) }\rmd s}\exp \parenthese{- \int_0 ^t \lambda(\phi_s(x)) \rmd s} \eqsp.
\end{multline*}
Since for all $x \in \msk$ and $t \in \ccint{0,T}$, $\varphi_t(x) \in \tilde \msk$, $f \in \mrc^1(\msm)$ and using \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c}, we get there exists $C_0 \geq 0$ such that for all $t \in \ccint{0,T}$,
\begin{equation}
  \label{eq:bound_F_0}
\sup_{x \in \msk} [     \abs{F_0(x)}+    \norm{\diff F_0(x)}  ]\leq C_0 \eqsp.
    \end{equation}
%    where we have used that for all $x \in \msm$, $\lambda(x) \geq \rate$.

We now show the result for $n \in \nsets$. We give first an explicit expression of $F_n$ for all $n \in \nsets$. Indeed, we have conditioning successively on $\mcf_{S_{n+1}^x}, \cdots, \mcf_{S_1^x}$, for all $x \in \msk$ and $t \in \ccint{0,T}$
\begin{multline}
  \label{eq:forme_loimarkov_chain}
  % \expeMarkov{(x,y)}{\1_{\coint{S^{(\epsilon)}_n,S^{(\epsilon)}_{n+1}}}(t) f(X^{(\epsilon)}_t,Y^{(\epsilon)}_t)}
  F_{n,t}(x)  = \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
  \int_0^{t-t_1} \rmd t_2 \exp\parenthese{-\int_0^{t_2} \lambda\defEns{\phi_{s_2}(x_1)} \rmd s_2}  \int_{\msm } \opK(\phi_{t_2}(x_1),\rmd x_2) \\
  \cdots   \int_0^{t-\sum_{i=1}^{n-1}t_i} \rmd t_n \exp\parenthese{-\int_0^{t_n} \lambda\defEns{\phi_{s_n}(x_{n-1})} \rmd s_n} \\
  \int_{\msm } \opK(\phi_{t_n}(x_{n-1}),\rmd x_n) f(\phi_{t-\sum_{i=1}^n t_i} (x_n))   \\  \exp\parenthese{-\int_0^{t-\sum_{i=1}^n t_i} \lambda\defEns{\phi_{s_{n+1}}(x_{n})} \rmd s_{n+1}} \eqsp,
\end{multline}
where $\opK$ is the kernel defined on $(\msm, \mcb{\msm})$  for all $x \in \msm$ and $\msa \in \mcb{\msm}$ by
  \begin{equation*}
    \opK(x,\msa) = \lambda(x) Q(x,\msa)  \eqsp.
  \end{equation*}

%   For the case $n=1$, we get for all $x \in \msk$ and $t \in \ccint{0,T}$,
%   \begin{multline}
%     \label{eq:first_estimate_gradient} 
%     F_{1,t}(x) =
%     \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1}  \lambda\defEns{\phi_{s_1}(x)} \rmd s_1}    \\
%       \times\left\lbrace \int_{\msm}  \lambda\parenthese{\phi_{t_1}(x)} Q(\phi_{t_1}(x),\rmd x_1) f\parenthese{\phi_{t-t_1}(x_1)} \exp\parenthese{-\int_0^{t-t_1} \lambda\defEns{\phi_{s_{2}}(x_1)} \rmd s_{2}} \right \rbrace
%   \eqsp.
% \end{multline}
% Since $f \in \mrc^1(\msm)$ and by \ref{item_1_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
% \begin{equation*}
%   x_1 \mapsto g(t_1,x_1) =  f\parenthese{\phi_{t-t_1}(x_1)} \exp\parenthese{-\int_0^{t-t_1} \lambda\defEns{\phi_{s_{2}}(x_1)} \rmd s_{2}} \eqsp,
% \end{equation*}
% is continuously differentiable for $t \in \ccint{0,T}, t_1 \in \ccint{0,t}$. In addition, for all $t \in \ccint{0,T}, t_1 \in \ccint{0,t}$ and for all $x_1 \in \supp \{Q(\varphi_{t_1}(x),\cdot)\}$, by \eqref{def:prop_tmsk}-\eqref{def:msk_i} $\varphi_{s_1}(x_1) \in\tilde K$ for all $s_1\in\ccint{0,t-t_1}$ and therefore
% \begin{equation*}
%   \abs{g}(t_1,x_1)  + \norm{\diff_x g(t_1,x_1)} < 2 \defEnsLigne{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{\diff \lambda }  \sup_{s \in \ccint{0,T}, y \in  \tmsk} \norm{\diff \varphi_{s}(y)}}\rme^{-\rate(t-t_1)} \eqsp.
% \end{equation*}
% Then by \ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
% $x \mapsto \lambda Qg(t_1,\varphi_{t_1}(x))$ is continuously differentiable for all
% $t \in \ccint{0,T}$, $t_1 \in \ccint{0,t}$ and for all $x \in \msk$,
% \begin{multline*}
%   \abs{\lambda Qg(t_1,\varphi_{t_1}(x))}  + \norm{\diff_x \lambda Qg(t_1,\varphi_{t_1}(x))}\\
%   \leq   4  \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}^2\rme^{-\rate(t-t_1)} \eqsp.
% \end{multline*}
%  In addition, since $\varphi_{t_1}(x) \subset \tilde \msk$, for all $t_1 \in \ccint{0,t}$, $t\in\ccint{0,T}$ and $x\in \msk$, by \ref{item_2_lem:stab_c1c}, we have
% \begin{multline*}
%   \sup_{x \in \msk} [\abs{F_1(x)} + \norm{\diff F_1(x) }] \\
%   \leq   8  \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}^3  t  \rme^{-\rate t} \eqsp.
% \end{multline*}

 We introduce a sequence of operator
$( Q^{(n)})_{n \in \nset^*}$, defined for all
$g : \rset_+ \times \msm \to \rset$, bounded on all compact of
$\ccint{0,T} \times \msm$ and measurable, $t \in \ccint{0,T}$ and
$x \in \msm$ by
  \begin{multline}
\label{eq:def_q_n}
    Q^{(n)} g (t,x) = \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
    \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n  \exp\parenthese{-\int_0^{t_n} \lambda\defEns{\phi_{s_n}(x_{n-1})} \rmd s_n} \\\int_{\msm } \opK(\phi_{t_n}(x_{n-1}),\rmd x_n) g(t-\sum_{i=1}^n t_i ,x_n) \eqsp.
  \end{multline}
  Taking for $g$ the function
  $g_F : (s,y) \mapsto f(\varphi_s(y)) \exp(-\int_0^s \rmd u
  \lambda(\varphi_u(y)))$, we have $F_{n,t} = Q^{(n)} g_F(t,\cdot)$. Since
  $f \in \mrc^1(\msm)$ and by \Cref{ass:stability}-\ref{item_3_lem:stab_c1c}, $g_F$ is
  measurable, for all $s \in \ccint{0,T}$, $y \mapsto g_F(s,y)$ is continuously
  differentiable on $\msm$ and satisfies for all $T' \in \ccint{0,T}$,
  $\msk' \subset \msm$ compact,
  $\sup_{s \in \ccint{0,T'}, y \in \msk'} \{\abs{g_F(s,y)} +
  \norm{\diff_x g_F(s,y)}\} < \plusinfty$. Therefore if we show that for
  all measurable function $g :\rset_+ \times \msm \to \rset_+$ such
  that for all $s \in \ccint{0,T}$, $y \mapsto g(s,y)$ is continuously differentiable
  on $\msm$ satisfying for all $T' \in \ccint{0,T}$, $\msk' \subset \msm$
  compact,
  $\sup_{s \in \ccint{0,T'}, y \in \msk'} \abs{g(s,y)} +
  \norm{\diff_x g(s,y)} < \plusinfty$: 1) for all
  $t \in \ccint{0,T}$ and $x \in \msk$, $x \mapsto Q^{(n)} g(t,x)$ is differentiable at $x$ 2) there exists $C \geq 0$ such that for all $n \in \nsets$,
  $x \in \msk$ and $t \in \ccint{0,T}$,
  \begin{equation}
    \label{eq:objectif_g}
    \abs{Q^{(n)} g(t,x)} + \norm{\diff_x Q^{(n)} g(t,x)} \leq C^n/(n!) \eqsp,
  \end{equation}
Note that this result and \eqref{eq:bound_F_0} show that \eqref{eq:estimate_gradient_n} holds and the proof is finished. Denote by $\mrgD$ the set of function $g$ satisfying the assumptions above. 

  Note the following relation between $Q^{(n-1)}$ and $Q^{(1)}$ which will be essential in our next reasonings: for all
$g : \rset_+ \times \msm \to \rset$, bounded on all compact of
$\rset_+ \times \msm$ and measurable, $t \in \ccint{0,T}$ and
$x \in \msm$ 
  \begin{multline}
\label{eq:q_n_prop_q_1}
    Q^{(n)} g (t,x) = \int_{0}^t \rmd t_1  \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) Q^{n-1}g(t-t_1,x_1) \\
    = Q^{(1)} [Q^{(n-1)}g](t,x)\eqsp.
  \end{multline}
  
  First, we make an induction on $i \in \iint{1,n}$ to show that
  for all $i \in \iint{1,n}$ and $g \in \mrg$, that
  $(s,x) \mapsto Q^{(i)} g(s,x) \in \mrgD$, which will show that for
  all $t \in \ccint{0,T}$,  $y\mapsto Q^ng(t,y)$
  is continuously differentiable. For $i =1$, note that for all
  $s \in \ccint{0,T}$ and $y \in \msm$,
  \begin{equation}
  \label{eq:def_q_1}
    Q^{(1)}g(s,y) = \int_0^s \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(y)} \rmd s_1}  \int_{\msm } \opK(\phi_{t_1}(y),\rmd y_1) g(s-t_1 ,y_1) \eqsp.
  \end{equation}
  Let $T' \in \ccint{0,T}$, $\msk' \subset \msm$ be compact and $\tilde \msk'$ given by \Cref{def:compact_comp} associated with
  $\msk'$ and $T'$. Then for all $s \in \ccint{0,T'}$, $t_1\in\ccint{0,s}$, $\varphi_{t_1}(y) \in \tilde \msk '$ for all $y \in \msk'$. Therefore we have 
 by assumption on $g$, \Cref{ass:stability}-\ref{item_2_lem:stab_c1c}-\ref{item_3_lem:stab_c1c},
  $y \mapsto  \int_{\msm } \opK(\phi_{t_1}(y),\rmd y_1) g(s-t_1 ,y_1)$ for all $s \in \ccint{0,T'}$, $t_1 \in \ccint{0,s}$, is differentiable and there exists $C \geq 0$ such that for all $s \in \ccint{0,T'}$, $t_1 \in \ccint{0,s}$
  \begin{equation*}
    \sup_{y \in \msk'} \defEns{ \abs{\opK g(s-t_1 \cdot)(\phi_{t_1}(y))} + \norm{\diff_x  \opK g(s-t_1 \cdot)(\phi_{t_1}(y))}} < C \eqsp
  \end{equation*}
  By \eqref{eq:def_q_1}, we get then the result for $i=1$. The result for $i \in \iint{2,n}$ is then a straightforward consequence of \eqref{eq:q_n_prop_q_1} and the case $i=1$.

  We now show that for all $g \in \mrgD$ that  there exists $C \geq 0$ such that for all
  $x \in \msk$ and $t \in \ccint{0,T}$, \eqref{eq:objectif_g}
  holds. % Note that for all $j \in \iint{1,n-1}$, by \eqref{eq:def_q_n} we have for all
  % $s \in \rset_+$ and $x \in \msm$,
  % \begin{multline*}
  %   Q^n_tg(x) =  \int_0^t \rmd t_1 \exp\parenthese{-\int_0^{t_1} \lambda\defEns{\phi_{s_1}(x)} \rmd s_1} \int_{\msm } \opK(\phi_{t_1}(x),\rmd x_1) \\
  %   \cdots \int_{\msm } \opK(\phi_{t_{j}}(x_{j-1}),\rmd x_j)  Q_{t-\sum_{i=1}^{j} t_i}^{n-j} g(x_j) \eqsp.
  % \end{multline*}
  By an induction on $N \in \iint{1,n}$, we show that for all $t \in \ccint{0,T}$,
  $(t_i)_{i \in \iint{1,n-N}} \in \rset_+^{n-N}$, $\sum_{j=1}^{n-N} t_j \leq t$, there exists $(\msk_{i})_{i \in \iint{0,n-N}}$ satisfying
  \ref{def:compact_comp_item_1}-\ref{def:compact_comp_item_2} in \Cref{def:compact_comp} with respect to $\msk$, $T$, $\tmsk$, $(t_i)_{i \in \iint{1,n-N}}$  and the following bound holds
  \begin{multline}
    \label{eq:stab_cont_rec}
    \sup_{x_{n-N} \in \msk_{n-N}} \abs{Q^N g\parenthese{t-\sum_{j=1}^{n-N}t_j,x_{n-N}} } + \norm{\diff Q^N g\parenthese{t-\sum_{j=1}^{n-N}t_j,x_{n-N}} } \\
    \leq C^{N}_1 \defEns{\sup_{s \in \ccint{0,T}, y \in \tmsk} \abs{g(s,y)} +\sup_{s \in \ccint{0,T}, y \in \tmsk} \norm{\diff_x g(s,y)} }   \left. \parenthese{t-\sum_{j=1}^{n-N}t_j}^N \middle /(N!) \right .\eqsp,
  \end{multline}
  where 
  \begin{equation}
    \label{eq:def_C_1C_2}
    C_1 = \norm{\lambda}_{\infty,\tmsk} + C_2 \eqsp, \qquad C_2 = \sup_{s \in \ccint{0,T}} \norm{\diff_x \varphi_s(x)}_{\infty, \tmsk} (T \norm{\diff \lambda}_{\infty,\tmsk} + \norm{\Psi}_{\infty,\tmsk}) \eqsp.
  \end{equation}
Then, the result for $N=n$ will conclude the proof.
  
  For $N=1$, let $t \in \ccint{0,T}$,
  $(t_i)_{i \in \iint{1,n-1}} \in \rset_+^{n-1}$, $\sum_{j=1}^{n-1} t_j \leq t$. Note that for all $y \in \msm$, setting $u_{n-1} = \sum_{i=1}^{n-1} t_i$,
    \begin{equation*}
%  \label{eq:def_q_1}
    Q^{(1)}g\parenthese{t-u_{n-1},y} = \int_0^{t - u_{n-1}} \rmd t_{n} \exp\parenthese{-\int_0^{t_n} \lambda\defEns{\phi_{s_n}(y)} \rmd s_n}  \int_{\msm } \opK(\phi_{t_n}(y),\rmd y_n) g(t-u_{n-1}-t_n ,y_n) \eqsp.
  \end{equation*}
For all $t_n \in \rset_+$, such that
  $\sum_{i=1}^n t_i < t$, by \Cref{ass:stability}-\ref{item_1_lem:stab_c1c}, there exists $(\msk_i)_{i \in \iint{0,n}}$ satisfying \ref{def:compact_comp_item_1}-\ref{def:compact_comp_item_2} in \Cref{def:compact_comp}. In particular, $(\msk_i)_{i \in \iint{0,n-1}}$ only depends on  $(t_i)_{i \in \iint{1,n-1}}$.  Then, using \Cref{ass:stability}, we get for all 
  $x_{n-1} \in \msk_{n-1}$,
\begin{align*}
&  \abs{ Q^{(1)}g\parenthese{t-u_{n-1},x_{n-1}}} \\
& \qquad \leq \norm{\lambda}_{\infty,\tmsk}  \int_0^{t - u_{n-1}} \rmd t_{n}    \sup\defEns{\abs{g}(t-u_{n-1}-t_n ,y_n)\, : \, y_n \in \supp\{ Q(\phi_{t_n}(x_{n-1}),\rmd y_n)\}} \\
                                          & \qquad  \leq  \norm{\lambda}_{\infty,\tmsk}  \int_0^{t - u_{n-1}} \rmd t_{n}    \sup\defEns{\abs{g}(t-u_{n-1}-t_n ,y_n)\, : \, y_n \in \msk_n} \eqsp,
\end{align*}
and
\begin{align*}
&   \norm{\nabla_x  Q^{(1)}g\parenthese{t-u_{n-1},x_{n-1}}} \\
  \qquad &\leq C_2 \int_0^{t - u_{n-1}} \rmd t_{n}    \sup\defEns{\abs{g}(t-u_{n-1}-t_n ,y_n) \, : \, y_n \in \supp\{ Q(\phi_{t_n}(x_{n-1}),\rmd y_n)\}}\\
& +  C_2 \int_0^{t - u_{n-1}} \rmd t_{n}    \sup\defEns{\norm{\nabla_x g (t-u_{n-1}-t_n ,y_n)} \, : \, y_n \in \supp\{ Q(\phi_{t_n}(x_{n-1}),\rmd y_n)\}}\\
&\leq C_2 \int_0^{t - u_{n-1}} \rmd t_{n}    \sup\defEns{\abs{g}(t-u_{n-1}-t_n ,y_n^1)+ \norm{\nabla_x g (t-u_{n-1}-t_n ,y_n^2)} \, : \, y_n^1,y_n^2 \in \msk_n} 
  \eqsp,
\end{align*}
where $C_2$ is given by \eqref{eq:def_C_1C_2}. Combining these two results and using that $\msk_n \subset \tmsk$ for all $t_n$, $\sum_{i=1}^n t_i < t$ give~\eqref{eq:stab_cont_rec} for $N=1$.

Now assume that the result holds for $N \in \iint{1,n-1}$ and let $(t_i)_{i \in \iint{1,n-N-1}} \in \rset_+^{n-N-1}$. By induction hypothesis, for all $t_{n-N} \in \rset_+$, such that
  $\sum_{i=1}^{n-N} t_i < t$, there exists  $(\msk_{i})_{i \in \iint{0,n-N}}$ satisfying
  \ref{def:compact_comp_item_1}-\ref{def:compact_comp_item_2} in \Cref{def:compact_comp} with respect to $\msk$, $T$, $\tmsk$, $(t_i)_{i \in \iint{1,n-N}}$.  Then, using \Cref{ass:stability} and \eqref{eq:q_n_prop_q_1}, we get for all 
  $x_{n-N-1} \in \msk_{n-N-1}$, setting $u_{n-N-1} =\sum_{i=1}^{n-N-1} t_i $ and $\msa_{n-N} = \supp\{ Q(\phi_{t_{n-N}}(x_{n-N-1}),\rmd y_{n-N})\}$
\begin{align*}
&  \abs{ Q^{(N)}g\parenthese{t-u_{n-N-1},x_{n-N-1}}} \\
& \qquad \leq \norm{\lambda}_{\infty,\tmsk}  \int_0^{t - u_{n-N-1}} \rmd t_{n-N}    \sup\defEns{\abs{Q^{(N-1)} g}(t-u_{n-N-1}-t_{n-N} ,y_{n-N})\, : \, y_{n-N} \in \msa_{n-N}} \\
                                          & \qquad  \leq  \norm{\lambda}_{\infty,\tmsk}  \int_0^{t - u_{n-N-1}} \rmd t_{n-N}    \sup\defEns{\abs{Q^{(N-1)}g}(t-u_{n-N-1}-t_{n-N} ,y_{n-N})\, : \, y_{n-N} \in \msk_{n-N}} \eqsp,
\end{align*}
and
\begin{align*}
&   \norm{\nabla_x  Q^{(N)}g\parenthese{t-u_{n-N-1},x_{n-N-1}}} \\
  \qquad &\leq C_2 \int_0^{t - u_{n-N-1}} \rmd t_{n-N}    \sup\defEns{\abs{Q^{(N-1)} g}(t-u_{n-N-1}-t_{n-N} ,y_{n-N}) \, : \, y_{n-N} \in \msa_{n-N}}\\
& +  C_2 \int_0^{t - u_{n-N-1}} \rmd t_{n-N}    \sup\defEns{\norm{\nabla_x Q^{(N-1)} g (t-u_{n-N-1}-t_{n-N} ,y_{n-N})} \, : \, y_{n-N} \in \msa_{n-N}}\\
  \qquad &\leq C_2 \int_0^{t - u_{n-N-1}} \rmd t_{n-N}    \sup\defEns{\abs{Q^{(N-1)}g}(t-u_{n-N-1}-t_{n-N} ,y_{n-N}) \, : \, y_{n-N} \in \msk_{n-N}}\\
& +  C_2 \int_0^{t - u_{n-N-1}} \rmd t_{n-N}    \sup\defEns{\norm{\nabla_x Q^{(N-1)} g (t-u_{n-N-1}-t_{n-N} ,y_{n-N})} \, : \, y_{n-N} \in \msk_{n-N}}
  \eqsp,
\end{align*}
where $C_2$ is given by \eqref{eq:def_C_1C_2}. Combining these two results using  $\msk_{n-N} \subset \tmsk$ for all $t_{n-N}$, $\sum_{i=1}^{n-N} t_i < t$ and the induction hypothesis conclude the proof of \eqref{eq:stab_cont_rec}.

%   Indeed, let
%   $x \in \msm$, $t \in \ccint{0,T}$ and
%   $g : \rset_+ \times \msm \to \rset$, bounded on all compact of
%   $\rset_+ \times \msm$, measurable, $y \mapsto g(s,y)$ is
%   continuously differentiable on $msm$, for all $s \in \rset_+$, Since
%   for all $y \in \msm$,

%   Then, an easy induction implies
%   by \eqref{def:prop_tmsk} that for all $i \in \{2,\ldots,n\}$,
%   $(t_j)_{i \in \{1,\ldots,i-1\}} \in \rset_+^n$,
%   $\sum_{j=1}^{i-1} t_j \leq t$, there exists
%   $(\msk_j)_{j \in \{1,\ldots,i-1\}}$ satisfying \eqref{def:msk_i} and
%   \begin{multline*}
%     \sup_{x_i \in \msk_i}      \abs{Q^{(i)}_{t-\sum_{j=1}^{i-1}t_j} g (x_i) } + \norm{\diff_x Q^{(i)}_{t-\sum_{j=1}^{i-1}t_j} g (x_i)}
%     \leq \defEns{\sup_{\tmsk} \abs{f} + \sup_{ \tmsk} \norm{\diff f} + \sup_{ \tmsk} \norm{ \lambda } + \sup_{ \tmsk} \norm{\diff \lambda }\parenthese{1+  \sup_{s \in \ccint{0,T}, y \in   \tmsk} \norm{\diff \varphi_{s}(y)}}}
%   \end{multline*}
%   Note that using the same reasoning as for $F_1$, we get that for all
%   functions
%   $(u,x) \in \rset_+ \times \msm \mapsto g(u,x) \in \rset$,
%    measurable, continuously differentiable with respect to $x$, for all $u >0$, $x \mapsto Q^{(1)}_u g(x,y)$ is continuously differentiable. In addition, for all   $u \in \ccint{0,t}$, there exists $C \geq 0$ such that 

%   \begin{multline}
%     \label{eq:estimate_nabla_G_1}
% \sup_{x \in \msk}      \abs{Q^{(1)}_t g(x)} + \norm{\nabla Q^{(1)}_t g(x)} \\\leq C  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \defEns{
%       \sup_{\substack{x \in \msk}} \abs{g}(t-t_1,x) +  \sup_{\substack{x \in \msk}} \norm{\diff_{x}g}(t-t_1,x)} \eqsp.
%   \end{multline}

%   By an easy induction using that for all $t \geq 0$,
%   $g : \rset_+ \times \msm \to \rset$, bounded and measurable, $x \in \msm$
%   and $n \in \nsets$, $n >1$,
%   \begin{equation*}
%      Q^{(n)}_t g (x,y) =      Q^{(1)}_t [\tilde{g}_t] (x,y)  \eqsp, \quad \text{with }  \tilde{g} (t_1,w,z) = Q^{(n-1)}_{t_1} g (w,z) \eqsp,
%    \end{equation*}
%    for all $t_1 \in \ccint{0,t}$ and \eqref{eq:estimate_nabla_G_1}, we
%    have that for all functions
%    $(t,x,y) \rset_+ \times \msm \mapsto g(t,x,y) \in \rset$,
%    bounded and measurable, differentiable with respect to the space
%    variables $(x,y)$, for all $t >0$ and $n \in \nsets$,
%    $(x,y) \mapsto Q^{(n)}_t g(x,y)$ is continuously differentiable. In
%    addition, for all $R \geq 0$, $n \in \nsets$ and $T >0$, there
%    exists $C \geq 0$ such that for all $t \in \ccint{0,T}$,
%    $x \in \msm$, $\norm{x} + \norm{y} \leq R$,
%   \begin{multline*}
%     \label{eq:estimate_nabla_G_n}
%      \abs{Q^{(n)}_t g(x,y)} + \norm{ \nabla Q^{(n)}_t g(x,y)} \leq C^n  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n \rme^{-\rate t_n }  \\\defEns{
%        \sup_{\substack{x \in \msm\\ \norm{x} + (1+t) \norm{y} \leq R}} \abs{g}\parenthese{t-\sum_{i=1}^n t_i,x,y} +     \sup_{\substack{x \in \msm\\ \norm{x} + (1+t) \norm{y} \leq R}}  \norm{\nabla_{x,y}g}\parenthese{t-\sum_{i=1}^n t_i,x,y}} \eqsp.
%   \end{multline*}

%   Applying this result to the function
%   \begin{equation*}
%   (t,x,y) \mapsto     f(\phi_{t} (x_n,y_n))     \exp\parenthese{-\int_0^{t} \lambda\defEns{\phi_{s_{n+1}}(x_{n},y_{n})} \rmd s_{n+1}} \eqsp,
%   \end{equation*}
%   and using \eqref{eq:def_F_n}, we get that for all $n \in \nsets$,
%   $F_n$ is continuously differentiable. In addition, using that for
%   all $(z,w) \in \msm$, $\lambda(z,w) \geq \rate$, we
%   get for all $R \geq 0$, $n \in \nsets$ and $T >0$, there exists
%   $C \geq 0$ such that for all $t \in \ccint{0,T}$,
%   $x \in \msm$, $\norm{x} + \norm{y} \leq R$,
%   \begin{align*}
%     \label{eq:estimate_nabla_F_n}
%     &\abs{F_n(x,y)} + \norm{ \nabla F_n(x,y)} \\
%     &\qquad     \qquad  \leq C^n  \int_0^t \rmd t_1 \rme^{- \rate t_1 } \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n \rme^{-\rate t_n }  \rme^{-(t-\sum_{i=1}^n t_i)\rate} \defEns{ \norm{f}_\infty + \norm{\nabla f}_\infty}  \\
%     &\qquad     \qquad   \leq  C^n \rme^{-t \rate } \int_0^t \rmd t_1  \cdots \int_0^{t-\sum_{i=1}^{n-1} t_i} \rmd t_n   \defEns{ \norm{f}_\infty + \norm{\nabla f}_\infty}\eqsp,
%   \end{align*}
%   which shows that \eqref{eq:estimate_gradient_n} holds and concludes the proof. 
  

%   For all $s\in[0,t]$, we have by \eqref{item_4_lem:stab_c1c} for all $x \in \msm$,
%   \begin{equation*}
%    P_s f(x) = \int_{\msm} \1_{\msk_{x,t}}(y) f(y) P_s(x,\rmd y)   \eqsp.
%  \end{equation*}
%  Therefore $P_sf(x) = 0$ for all $x \in \msm$, 
%   $P_s f(x) = 0$ for all $x$ with $dist(x,\supp f) > \sup\{C_2(s),\ s\in[0,t]\}$. In particular, $P_t f$ is compactly supported. For any $x_0 \in \msm$, let us prove that $P_t f$ is $\rmc^1$ on $\msb(x_0,1)$. Let $\lambda_* = 1+ \sup\{\lambda(x),\ x\in\msb(x_0,1+C_2(t))\}$, and $(\bar P_t)_{t\geqslant 0}$ be the PDMP semigroup with characteristics $( \varphi,\lambda_*,Q_*)_{i\in \iintLigne{1,n}})$ with for all $x\in\msm$,
% \[Q_*(x,\cdot) \ = \  \frac{1 - (\lambda(x)\wedge \lambda_*)}{\lambda_*} \delta_x(\cdot) +  \frac{\lambda(x)\wedge \lambda_*}{\lambda_*} Q(x,\cdot) \eqsp.\]
% Then, for all $x\in \msb(x_0,1)$, $\bar P_t f(x) = P_t f(x)$.

%  Conditioning by the jump times of the process (which are jump times of an homogeneous Poisson process with intensity $\lambda_*$),
%  \begin{eqnarray*}
%  \bar P_t f(x) & = & \sum_{k\in\nset} \frac{(\lambda_* t)^k}{k!}\int_{\Delta_{k,t}} T_{s_1} Q_* T_{s_2} \dots Q_* T_{s_{k-1}} Q_* T_{s_k} f(x) \rmd s_1,\dots,\rmd s_k
%  \end{eqnarray*}
%  where, for $k\in\nset$, $\Delta_{k,t} = \{s\in \rset_+^k, \sum_{i=1}^k s_i = t\}$ and $T_r f(x) = f( \varphi_r(x))$. For a given $x\in \msb(x_0,1)$, $k\in\nset$ and $s\in \Delta_{k,t}$, let $E_0=\{x\}$, $E_{i} = \cup\{ \supp Q_*( \varphi_{s_i}(y),\cdot),\ y\in E_{i-1}\}$ for $i\in \iintLigne{1,k-1}$ and $E_k = \cup\{ \varphi_{s_k}(y),\ y\in E_{k-1}\}$. By assumption, for almost every $s\in \Delta_{k,t}$, $E_i \subset \msb(x,C_2(t))\subset \msb(x_0,1+C_2(t))$ for all $i\in \iintLigne{0,k}$ (otherwise, this would be in contradiction with the fact that almost surely $X_u \in \msb(X_0,C_2(t))$ for all $u\in[0,t]$). Hence, there exists $C>0$ such that, for all $x\in \msb(x_0,1)$, $k\in\nset$, $i\in \iintLigne{1,k-1}$ and almost every $s\in \Delta_{k,t}$,
%  \[\sup\{|T_{s_i}Q_*f(y)| + \norm{\na T_{s_i}Q_* f(y)},\ y\in E_{i-1}\} \ \leqslant \ C \sup\{|f(y)| + \norm{\na f(y)},\ y\in E_{i}\}\eqsp,\]
%   \[\sup\{|T_{s_k} f(y)| + \norm{\na T_{s_k}  f(y)},\ y\in E_{k-1}\} \ \leqslant \ C \sup\{|f(y)| + \norm{\na f(y)},\ y\in E_{k}\}\eqsp,\]
% and in particular
% \[\norm{\na (T_{s_1} Q_*  \dots  Q_* T_{s_k} f)(x)} \ \leqslant \ C^k ( \|f\|_\infty + \norm{\na f}_\infty) \eqsp.\]
%  Hence, $\bar P_t f$ is $\rmc^1$ on $\msb(x_0,1)$, on which it is equal to $P_t f$, which concludes.
\end{proof}

\begin{remark}
  \Cref{lem:stab_c1c} can be generalized  under the condition that
for some $k \in \nsets$,  the  characteristics $(\varphi,\lambda,Q)$ satisfy
\begin{enumerate}[label = (\roman*)]
\item \label{item_1_lem:stab_c1c_b} the flow  $\varphi$ and the Markov kernel $Q$ are compactly compatible;
\item \label{item_2_lem:stab_c1c_b} $\lambda\in\mrc^{k}(\msm)$ and for all $f \in \mrc^k(\msm)$, $\lambda Qf \in \mrc^k(\msm)$ and there exists a function $\Psi :\msm \to \rset_+$ such that for all compact set $\msk \subset \msm$, $\sup_{y \in \msk} \Psi(y) < \plusinfty$ and for all $x \in \msk$, $i \in\iint{1,k}$,
  \begin{equation*}
    \label{eq:1}
  \norm{\diffD^i (\lambda Qf)(x)} \leq    \sup_{y \in \msk} \{ \Psi(y)\} \sup \ensemble{ \norm{\diffD^i f(y)}}{y \in \supp \{Q(x,\cdot)\} \eqsp,i \in\iint{1,k} };
  \end{equation*}
\item \label{item_3_lem:stab_c1c_b} for all $t \in \rset_+$, we have $x \mapsto \varphi_t(x)$ is $k$-times continuously differentiable  and for all compact $\msk \subset \msm$, 
  \begin{equation*}
    \sup \ensemble{\norm{\diffD^i \varphi_s(x)}}{s \in \ccint{0,t}, x \in \msk\eqsp, i \in \iint{1,k}} < \plusinfty \eqsp.
  \end{equation*}
\end{enumerate}
Then for all function $f \in \mrc^k(\msm)$, and $T \in \rset_+$,
$P_Tf \in \mrc^k(\msm)$. In addition, for all compact set
$\msk \subset\msm$, and $T \in \rset_+$, there exists $C \geq 0$ such
that for all $t \in \ccint{0,T}$,
$\sup_{x \in \msk} \absLigne{P_t f}(x) + \sup_{x \in \msk, i
  \in\iint{1,k}} \norm{\diffD^i P_t f(x)} \leq C$.
\end{remark}



Combining \Cref{lem:compact_sup}-\Cref{propo:c_1_c_sgenerator}-\Cref{lem:stab_c1c} and \cite[Proposition 3.3, Chapter 1]{ethier:kurtz:1986}, we get the following result.
\begin{corollary}
\label{coro:core_generator}
Let characteristics $(\varphi,\lambda,Q)$ satisfying \Cref{ass:compact_sup}-\Cref{ass:stability} and $(t,x) \mapsto \varphi_t(x) \in \rmc^1(\msm)$. Then, $\rmc^1_c(\msm)$ is a core for the strong generator of $(P_t)_{t \geq 0}$. 
\end{corollary}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

